Search for magnetically-induced signatures in the arrival directions of ultra-high-energy cosmic rays measured at the Pierre Auger Observatory

We search for signals of magnetically-induced effects in the arrival directions of ultra-high-energy cosmic rays detected at the Pierre Auger Observatory. We apply two different methods. One is a search for sets of events that show a correlation between their arrival direction and the inverse of their energy, which would be expected if they come from the same point-like source, they have the same electric charge and their deflection is relatively small and coherent. We refer to these sets of events as "multiplets". The second method, called "thrust", is a principal axis analysis aimed to detect the elongated patterns in a region of interest. We study the sensitivity of both methods using a benchmark simulation and we apply them to data in two different searches. The first search is done assuming as source candidates a list of nearby active galactic nuclei and starburst galaxies. The second is an all-sky blind search. We report the results and we find no statistically significant features. We discuss the compatibility of these results with the indications on the mass composition inferred from data of the Pierre Auger Observatory.

==> 2020-04-author_list-ZIP/aastex_authorlist.tex <==
% created on 2020-04-02

\author{
A.~Aab\altaffilmark{75},
P.~Abreu\altaffilmark{67},
M.~Aglietta\altaffilmark{50,49},
J.M.~Albury\altaffilmark{12},
I.~Allekotte\altaffilmark{1},
A.~Almela\altaffilmark{8,11},
J.~Alvarez Castillo\altaffilmark{63},
J.~Alvarez-Mu\~niz\altaffilmark{74},
R.~Alves Batista\altaffilmark{75},
G.A.~Anastasi\altaffilmark{58,49},
L.~Anchordoqui\altaffilmark{82},
B.~Andrada\altaffilmark{8},
S.~Andringa\altaffilmark{67},
C.~Aramo\altaffilmark{47},
P.R.~Ara\'ujo Ferreira\altaffilmark{39},
H.~Asorey\altaffilmark{8},
P.~Assis\altaffilmark{67},
G.~Avila\altaffilmark{9,10},
A.M.~Badescu\altaffilmark{70},
A.~Bakalova\altaffilmark{30},
A.~Balaceanu\altaffilmark{68},
F.~Barbato\altaffilmark{56,47},
R.J.~Barreira Luz\altaffilmark{67},
K.H.~Becker\altaffilmark{35},
J.A.~Bellido\altaffilmark{12},
C.~Berat\altaffilmark{34},
M.E.~Bertaina\altaffilmark{58,49},
X.~Bertou\altaffilmark{1},
P.L.~Biermann\altaffilmark{1001},
T.~Bister\altaffilmark{39},
J.~Biteau\altaffilmark{32},
A.~Blanco\altaffilmark{67},
J.~Blazek\altaffilmark{30},
C.~Bleve\altaffilmark{34},
M.~Boh\'a\v{c}ov\'a\altaffilmark{30},
D.~Boncioli\altaffilmark{53,43},
C.~Bonifazi\altaffilmark{24},
L.~Bonneau Arbeletche\altaffilmark{19},
N.~Borodai\altaffilmark{64},
A.M.~Botti\altaffilmark{8},
J.~Brack\altaffilmark{1004},
T.~Bretz\altaffilmark{39},
F.L.~Briechle\altaffilmark{39},
P.~Buchholz\altaffilmark{41},
A.~Bueno\altaffilmark{73},
S.~Buitink\altaffilmark{14},
M.~Buscemi\altaffilmark{54,44},
K.S.~Caballero-Mora\altaffilmark{62},
L.~Caccianiga\altaffilmark{55,46},
L.~Calcagni\altaffilmark{4},
A.~Cancio\altaffilmark{11,8},
F.~Canfora\altaffilmark{75,77},
I.~Caracas\altaffilmark{35},
J.M.~Carceller\altaffilmark{73},
R.~Caruso\altaffilmark{54,44},
A.~Castellina\altaffilmark{50,49},
F.~Catalani\altaffilmark{17},
G.~Cataldi\altaffilmark{45},
L.~Cazon\altaffilmark{67},
M.~Cerda\altaffilmark{9},
J.A.~Chinellato\altaffilmark{20},
K.~Choi\altaffilmark{74},
J.~Chudoba\altaffilmark{30},
L.~Chytka\altaffilmark{31},
R.W.~Clay\altaffilmark{12},
A.C.~Cobos Cerutti\altaffilmark{7},
R.~Colalillo\altaffilmark{56,47},
A.~Coleman\altaffilmark{88},
M.R.~Coluccia\altaffilmark{52,45},
R.~Concei\c{c}\~ao\altaffilmark{67},
A.~Condorelli\altaffilmark{42,43},
G.~Consolati\altaffilmark{46,51},
F.~Contreras\altaffilmark{9,10},
F.~Convenga\altaffilmark{52,45},
C.E.~Covault\altaffilmark{80,1007},
S.~Dasso\altaffilmark{5,3},
K.~Daumiller\altaffilmark{37},
B.R.~Dawson\altaffilmark{12},
J.A.~Day\altaffilmark{12},
R.M.~de Almeida\altaffilmark{26},
J.~de Jes\'us\altaffilmark{8,37},
S.J.~de Jong\altaffilmark{75,77},
G.~De Mauro\altaffilmark{75,77},
J.R.T.~de Mello Neto\altaffilmark{24,25},
I.~De Mitri\altaffilmark{42,43},
J.~de Oliveira\altaffilmark{26},
D.~de Oliveira Franco\altaffilmark{20},
V.~de Souza\altaffilmark{18},
J.~Debatin\altaffilmark{36},
M.~del R\'\i{}o\altaffilmark{10},
O.~Deligny\altaffilmark{32},
N.~Dhital\altaffilmark{64},
A.~Di Matteo\altaffilmark{49},
M.L.~D\'\i{}az Castro\altaffilmark{20},
C.~Dobrigkeit\altaffilmark{20},
J.C.~D'Olivo\altaffilmark{63},
Q.~Dorosti\altaffilmark{41},
R.C.~dos Anjos\altaffilmark{23},
M.T.~Dova\altaffilmark{4},
J.~Ebr\altaffilmark{30},
R.~Engel\altaffilmark{36,37},
I.~Epicoco\altaffilmark{52,45},
M.~Erdmann\altaffilmark{39},
C.O.~Escobar\altaffilmark{1002},
A.~Etchegoyen\altaffilmark{8,11},
H.~Falcke\altaffilmark{75,78,77},
J.~Farmer\altaffilmark{87},
G.~Farrar\altaffilmark{85},
A.C.~Fauth\altaffilmark{20},
N.~Fazzini\altaffilmark{1002},
F.~Feldbusch\altaffilmark{38},
F.~Fenu\altaffilmark{58,49},
B.~Fick\altaffilmark{84},
J.M.~Figueira\altaffilmark{8},
A.~Filip\v{c}i\v{c}\altaffilmark{72,71},
T.~Fodran\altaffilmark{75},
M.M.~Freire\altaffilmark{6},
T.~Fujii\altaffilmark{87,1005},
A.~Fuster\altaffilmark{8,11},
C.~Galea\altaffilmark{75},
C.~Galelli\altaffilmark{55,46},
B.~Garc\'\i{}a\altaffilmark{7},
A.L.~Garcia Vegas\altaffilmark{39},
H.~Gemmeke\altaffilmark{38},
F.~Gesualdi\altaffilmark{8,37},
A.~Gherghel-Lascu\altaffilmark{68},
P.L.~Ghia\altaffilmark{32},
U.~Giaccari\altaffilmark{75},
M.~Giammarchi\altaffilmark{46},
M.~Giller\altaffilmark{65},
J.~Glombitza\altaffilmark{39},
F.~Gobbi\altaffilmark{9},
G.~Golup\altaffilmark{1},
M.~G\'omez Berisso\altaffilmark{1},
P.F.~G\'omez Vitale\altaffilmark{9,10},
J.P.~Gongora\altaffilmark{9},
N.~Gonz\'alez\altaffilmark{8},
I.~Goos\altaffilmark{1,37},
D.~G\'ora\altaffilmark{64},
A.~Gorgi\altaffilmark{50,49},
M.~Gottowik\altaffilmark{35},
T.D.~Grubb\altaffilmark{12},
F.~Guarino\altaffilmark{56,47},
G.P.~Guedes\altaffilmark{21},
E.~Guido\altaffilmark{49,58},
S.~Hahn\altaffilmark{37,8},
R.~Halliday\altaffilmark{80},
M.R.~Hampel\altaffilmark{8},
P.~Hansen\altaffilmark{4},
D.~Harari\altaffilmark{1},
V.M.~Harvey\altaffilmark{12},
A.~Haungs\altaffilmark{37},
T.~Hebbeker\altaffilmark{39},
D.~Heck\altaffilmark{37},
G.C.~Hill\altaffilmark{12},
C.~Hojvat\altaffilmark{1002},
J.R.~H\"orandel\altaffilmark{75,77},
P.~Horvath\altaffilmark{31},
M.~Hrabovsk\'y\altaffilmark{31},
T.~Huege\altaffilmark{37,14},
J.~Hulsman\altaffilmark{8,37},
A.~Insolia\altaffilmark{54,44},
P.G.~Isar\altaffilmark{69},
J.A.~Johnsen\altaffilmark{81},
J.~Jurysek\altaffilmark{30},
A.~K\"a\"ap\"a\altaffilmark{35},
K.H.~Kampert\altaffilmark{35},
B.~Keilhauer\altaffilmark{37},
J.~Kemp\altaffilmark{39},
H.O.~Klages\altaffilmark{37},
M.~Kleifges\altaffilmark{38},
J.~Kleinfeller\altaffilmark{9},
M.~K\"opke\altaffilmark{36},
G.~Kukec Mezek\altaffilmark{71},
B.L.~Lago\altaffilmark{16},
D.~LaHurd\altaffilmark{80},
R.G.~Lang\altaffilmark{18},
M.A.~Leigui de Oliveira\altaffilmark{22},
V.~Lenok\altaffilmark{37},
A.~Letessier-Selvon\altaffilmark{33},
I.~Lhenry-Yvon\altaffilmark{32},
D.~Lo Presti\altaffilmark{54,44},
L.~Lopes\altaffilmark{67},
R.~L\'opez\altaffilmark{59},
R.~Lorek\altaffilmark{80},
Q.~Luce\altaffilmark{36},
A.~Lucero\altaffilmark{8},
A.~Machado Payeras\altaffilmark{20},
M.~Malacari\altaffilmark{87},
G.~Mancarella\altaffilmark{52,45},
D.~Mandat\altaffilmark{30},
B.C.~Manning\altaffilmark{12},
J.~Manshanden\altaffilmark{40},
P.~Mantsch\altaffilmark{1002},
S.~Marafico\altaffilmark{32},
A.G.~Mariazzi\altaffilmark{4},
I.C.~Mari\c{s}\altaffilmark{13},
G.~Marsella\altaffilmark{52,45},
D.~Martello\altaffilmark{52,45},
H.~Martinez\altaffilmark{18},
O.~Mart\'\i{}nez Bravo\altaffilmark{59},
M.~Mastrodicasa\altaffilmark{53,43},
H.J.~Mathes\altaffilmark{37},
J.~Matthews\altaffilmark{83},
G.~Matthiae\altaffilmark{57,48},
E.~Mayotte\altaffilmark{35},
P.O.~Mazur\altaffilmark{1002},
G.~Medina-Tanco\altaffilmark{63},
D.~Melo\altaffilmark{8},
A.~Menshikov\altaffilmark{38},
K.-D.~Merenda\altaffilmark{81},
S.~Michal\altaffilmark{31},
M.I.~Micheletti\altaffilmark{6},
L.~Miramonti\altaffilmark{55,46},
D.~Mockler\altaffilmark{13},
S.~Mollerach\altaffilmark{1},
F.~Montanet\altaffilmark{34},
C.~Morello\altaffilmark{50,49},
M.~Mostaf\'a\altaffilmark{86},
A.L.~M\"uller\altaffilmark{8,37},
M.A.~Muller\altaffilmark{20,1003,24},
K.~Mulrey\altaffilmark{14},
R.~Mussa\altaffilmark{49},
M.~Muzio\altaffilmark{85},
W.M.~Namasaka\altaffilmark{35},
L.~Nellen\altaffilmark{63},
M.~Niculescu-Oglinzanu\altaffilmark{68},
M.~Niechciol\altaffilmark{41},
D.~Nitz\altaffilmark{84,1006},
D.~Nosek\altaffilmark{29},
V.~Novotny\altaffilmark{29},
L.~No\v{z}ka\altaffilmark{31},
A Nucita\altaffilmark{52,45},
L.A.~N\'u\~nez\altaffilmark{28},
M.~Palatka\altaffilmark{30},
J.~Pallotta\altaffilmark{2},
M.P.~Panetta\altaffilmark{52,45},
P.~Papenbreer\altaffilmark{35},
G.~Parente\altaffilmark{74},
A.~Parra\altaffilmark{59},
M.~Pech\altaffilmark{30},
F.~Pedreira\altaffilmark{74},
J.~P\c{e}kala\altaffilmark{64},
R.~Pelayo\altaffilmark{61},
J.~Pe\~na-Rodriguez\altaffilmark{28},
J.~Perez Armand\altaffilmark{19},
M.~Perlin\altaffilmark{8,37},
L.~Perrone\altaffilmark{52,45},
C.~Peters\altaffilmark{39},
S.~Petrera\altaffilmark{42,43},
T.~Pierog\altaffilmark{37},
M.~Pimenta\altaffilmark{67},
V.~Pirronello\altaffilmark{54,44},
M.~Platino\altaffilmark{8},
B.~Pont\altaffilmark{75},
M.~Pothast\altaffilmark{77,75},
P.~Privitera\altaffilmark{87},
M.~Prouza\altaffilmark{30},
A.~Puyleart\altaffilmark{84},
S.~Querchfeld\altaffilmark{35},
J.~Rautenberg\altaffilmark{35},
D.~Ravignani\altaffilmark{8},
M.~Reininghaus\altaffilmark{37,8},
J.~Ridky\altaffilmark{30},
F.~Riehn\altaffilmark{67},
M.~Risse\altaffilmark{41},
P.~Ristori\altaffilmark{2},
V.~Rizi\altaffilmark{53,43},
W.~Rodrigues de Carvalho\altaffilmark{19},
J.~Rodriguez Rojo\altaffilmark{9},
M.J.~Roncoroni\altaffilmark{8},
M.~Roth\altaffilmark{37},
E.~Roulet\altaffilmark{1},
A.C.~Rovero\altaffilmark{5},
P.~Ruehl\altaffilmark{41},
S.J.~Saffi\altaffilmark{12},
A.~Saftoiu\altaffilmark{68},
F.~Salamida\altaffilmark{53,43},
H.~Salazar\altaffilmark{59},
G.~Salina\altaffilmark{48},
J.D.~Sanabria Gomez\altaffilmark{28},
F.~S\'anchez\altaffilmark{8},
E.M.~Santos\altaffilmark{19},
E.~Santos\altaffilmark{30},
F.~Sarazin\altaffilmark{81},
R.~Sarmento\altaffilmark{67},
C.~Sarmiento-Cano\altaffilmark{8},
R.~Sato\altaffilmark{9},
P.~Savina\altaffilmark{52,45,32},
C.~Sch\"afer\altaffilmark{37},
V.~Scherini\altaffilmark{45},
H.~Schieler\altaffilmark{37},
M.~Schimassek\altaffilmark{36,8},
M.~Schimp\altaffilmark{35},
F.~Schl\"uter\altaffilmark{37,8},
D.~Schmidt\altaffilmark{36},
O.~Scholten\altaffilmark{76,14},
P.~Schov\'anek\altaffilmark{30},
F.G.~Schr\"oder\altaffilmark{88,37},
S.~Schr\"oder\altaffilmark{35},
S.J.~Sciutto\altaffilmark{4},
M.~Scornavacche\altaffilmark{8,37},
R.C.~Shellard\altaffilmark{15},
G.~Sigl\altaffilmark{40},
G.~Silli\altaffilmark{8,37},
O.~Sima\altaffilmark{68,1007},
R.~\v{S}m\'\i{}da\altaffilmark{87},
P.~Sommers\altaffilmark{86},
J.F.~Soriano\altaffilmark{82},
J.~Souchard\altaffilmark{34},
R.~Squartini\altaffilmark{9},
M.~Stadelmaier\altaffilmark{37,8},
D.~Stanca\altaffilmark{68},
S.~Stani\v{c}\altaffilmark{71},
J.~Stasielak\altaffilmark{64},
P.~Stassi\altaffilmark{34},
A.~Streich\altaffilmark{36,8},
M.~Su\'arez-Dur\'an\altaffilmark{28},
T.~Sudholz\altaffilmark{12},
T.~Suomij\"arvi\altaffilmark{32},
A.D.~Supanitsky\altaffilmark{8},
J.~\v{S}up\'\i{}k\altaffilmark{31},
Z.~Szadkowski\altaffilmark{66},
A.~Taboada\altaffilmark{36},
A.~Tapia\altaffilmark{27},
C.~Timmermans\altaffilmark{77,75},
P.~Tobiska\altaffilmark{30},
C.J.~Todero Peixoto\altaffilmark{17},
B.~Tom\'e\altaffilmark{67},
G.~Torralba Elipe\altaffilmark{74},
A.~Travaini\altaffilmark{9},
P.~Travnicek\altaffilmark{30},
C.~Trimarelli\altaffilmark{53,43},
M.~Trini\altaffilmark{71},
M.~Tueros\altaffilmark{4},
R.~Ulrich\altaffilmark{37},
M.~Unger\altaffilmark{37},
M.~Urban\altaffilmark{39},
L.~Vaclavek\altaffilmark{31},
M.~Vacula\altaffilmark{31},
J.F.~Vald\'es Galicia\altaffilmark{63},
I.~Vali\~no\altaffilmark{42,43},
L.~Valore\altaffilmark{56,47},
A.~van Vliet\altaffilmark{75},
E.~Varela\altaffilmark{59},
B.~Vargas C\'ardenas\altaffilmark{63},
A.~V\'asquez-Ram\'\i{}rez\altaffilmark{28},
D.~Veberi\v{c}\altaffilmark{37},
C.~Ventura\altaffilmark{25},
I.D.~Vergara Quispe\altaffilmark{4},
V.~Verzi\altaffilmark{48},
J.~Vicha\altaffilmark{30},
L.~Villase\~nor\altaffilmark{59},
J.~Vink\altaffilmark{79},
S.~Vorobiov\altaffilmark{71},
H.~Wahlberg\altaffilmark{4},
A.A.~Watson\altaffilmark{1000},
M.~Weber\altaffilmark{38},
A.~Weindl\altaffilmark{37},
L.~Wiencke\altaffilmark{81},
H.~Wilczy\'nski\altaffilmark{64},
T.~Winchen\altaffilmark{14},
M.~Wirtz\altaffilmark{39},
D.~Wittkowski\altaffilmark{35},
B.~Wundheiler\altaffilmark{8},
A.~Yushkov\altaffilmark{30},
O.~Zapparrata\altaffilmark{13},
E.~Zas\altaffilmark{74},
D.~Zavrtanik\altaffilmark{71,72},
M.~Zavrtanik\altaffilmark{72,71},
L.~Zehrer\altaffilmark{71},
A.~Zepeda\altaffilmark{60},
M.~Ziolkowski\altaffilmark{41},
F.~Zuccarello\altaffilmark{54,44}
}

\fullcollaborationName{The Pierre Auger Collaboration}

\altaffiltext{1}{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}
\altaffiltext{2}{Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina}
\altaffiltext{3}{Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina}
\altaffiltext{4}{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}
\altaffiltext{5}{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}
\altaffiltext{6}{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}
\altaffiltext{7}{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}
\altaffiltext{8}{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\altaffiltext{9}{Observatorio Pierre Auger, Malarg\"ue, Argentina}
\altaffiltext{10}{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}
\altaffiltext{11}{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}
\altaffiltext{12}{University of Adelaide, Adelaide, S.A., Australia}
\altaffiltext{13}{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}
\altaffiltext{14}{Vrije Universiteit Brussels, Brussels, Belgium}
\altaffiltext{15}{Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil}
\altaffiltext{16}{Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil}
\altaffiltext{17}{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}
\altaffiltext{18}{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}
\altaffiltext{19}{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}
\altaffiltext{20}{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}
\altaffiltext{21}{Universidade Estadual de Feira de Santana, Feira de Santana, Brazil}
\altaffiltext{22}{Universidade Federal do ABC, Santo Andr\'e, SP, Brazil}
\altaffiltext{23}{Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil}
\altaffiltext{24}{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}
\altaffiltext{25}{Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil}
\altaffiltext{26}{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}
\altaffiltext{27}{Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia}
\altaffiltext{28}{Universidad Industrial de Santander, Bucaramanga, Colombia}
\altaffiltext{29}{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}
\altaffiltext{30}{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}
\altaffiltext{31}{Palacky University, RCPTM, Olomouc, Czech Republic}
\altaffiltext{32}{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}
\altaffiltext{33}{Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Universit\'es Paris 6 et Paris 7, CNRS-IN2P3, Paris, France}
\altaffiltext{34}{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}
\altaffiltext{35}{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}
\altaffiltext{36}{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}
\altaffiltext{37}{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\altaffiltext{38}{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}
\altaffiltext{39}{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}
\altaffiltext{40}{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}
\altaffiltext{41}{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}
\altaffiltext{42}{Gran Sasso Science Institute, L'Aquila, Italy}
\altaffiltext{43}{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}
\altaffiltext{44}{INFN, Sezione di Catania, Catania, Italy}
\altaffiltext{45}{INFN, Sezione di Lecce, Lecce, Italy}
\altaffiltext{46}{INFN, Sezione di Milano, Milano, Italy}
\altaffiltext{47}{INFN, Sezione di Napoli, Napoli, Italy}
\altaffiltext{48}{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}
\altaffiltext{49}{INFN, Sezione di Torino, Torino, Italy}
\altaffiltext{50}{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\altaffiltext{51}{Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy}
\altaffiltext{52}{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\altaffiltext{53}{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\altaffiltext{54}{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\altaffiltext{55}{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\altaffiltext{56}{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\altaffiltext{57}{Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy}
\altaffiltext{58}{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\altaffiltext{59}{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}
\altaffiltext{60}{Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico, D.F., M\'exico}
\altaffiltext{61}{Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico}
\altaffiltext{62}{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}
\altaffiltext{63}{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}
\altaffiltext{64}{Institute of Nuclear Physics PAN, Krakow, Poland}
\altaffiltext{65}{University of \L{}\'od\'z, Faculty of Astrophysics, \L{}\'od\'z, Poland}
\altaffiltext{66}{University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland}
\altaffiltext{67}{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}
\altaffiltext{68}{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}
\altaffiltext{69}{Institute of Space Science, Bucharest-Magurele, Romania}
\altaffiltext{70}{University Politehnica of Bucharest, Bucharest, Romania}
\altaffiltext{71}{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}
\altaffiltext{72}{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\altaffiltext{73}{Universidad de Granada and C.A.F.P.E., Granada, Spain}
\altaffiltext{74}{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}
\altaffiltext{75}{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\altaffiltext{76}{KVI -- Center for Advanced Radiation Technology, University of Groningen, Groningen, The Netherlands}
\altaffiltext{77}{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\altaffiltext{78}{Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands}
\altaffiltext{79}{Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands}
\altaffiltext{80}{Case Western Reserve University, Cleveland, OH, USA}
\altaffiltext{81}{Colorado School of Mines, Golden, CO, USA}
\altaffiltext{82}{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}
\altaffiltext{83}{Louisiana State University, Baton Rouge, LA, USA}
\altaffiltext{84}{Michigan Technological University, Houghton, MI, USA}
\altaffiltext{85}{New York University, New York, NY, USA}
\altaffiltext{86}{Pennsylvania State University, University Park, PA, USA}
\altaffiltext{87}{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}
\altaffiltext{88}{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}
\altaffiltext{}{-----}
\altaffiltext{1000}{School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom}
\altaffiltext{1001}{Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany}
\altaffiltext{1002}{Fermi National Accelerator Laboratory, USA}
\altaffiltext{1003}{also at Universidade Federal de Alfenas, Po\c{c}os de Caldas, Brazil}
\altaffiltext{1004}{Colorado State University, Fort Collins, CO, USA}
\altaffiltext{1005}{now at Hakubi Center for Advanced Research and Graduate School of Science, Kyoto University, Kyoto, Japan}
\altaffiltext{1006}{also at Karlsruhe Institute of Technology, Karlsruhe, Germany}
\altaffiltext{1007}{also at Radboud Universtiy Nijmegen, Nijmegen, The Netherlands}


==> 2020-04-author_list-ZIP/acknowledgments.tex <==
% created on 2020-04-02

\section*{Acknowledgments}

\begin{sloppypar}
The successful installation, commissioning, and operation of the Pierre
Auger Observatory would not have been possible without the strong
commitment and effort from the technical and administrative staff in
Malarg\"ue. We are very grateful to the following agencies and
organizations for financial support:
\end{sloppypar}

\begin{sloppypar}
Argentina -- Comisi\'on Nacional de Energ\'\i{}a At\'omica; Agencia Nacional de
Promoci\'on Cient\'\i{}fica y Tecnol\'ogica (ANPCyT); Consejo Nacional de
Investigaciones Cient\'\i{}ficas y T\'ecnicas (CONICET); Gobierno de la
Provincia de Mendoza; Municipalidad de Malarg\"ue; NDM Holdings and Valle
Las Le\~nas; in gratitude for their continuing cooperation over land
access; Australia -- the Australian Research Council; Brazil -- Conselho
Nacional de Desenvolvimento Cient\'\i{}fico e Tecnol\'ogico (CNPq);
Financiadora de Estudos e Projetos (FINEP); Funda\c{c}\~ao de Amparo \`a
Pesquisa do Estado de Rio de Janeiro (FAPERJ); S\~ao Paulo Research
Foundation (FAPESP) Grants No.~2019/10151-2, No.~2010/07359-6 and
No.~1999/05404-3; Minist\'erio da Ci\^encia, Tecnologia, Inova\c{c}\~oes e
Comunica\c{c}\~oes (MCTIC); Czech Republic -- Grant No.~MSMT CR LTT18004,
LM2015038, LM2018102, CZ.02.1.01/0.0/0.0/16{\textunderscore}013/0001402,
CZ.02.1.01/0.0/0.0/18{\textunderscore}046/0016010 and
CZ.02.1.01/0.0/0.0/17{\textunderscore}049/0008422; France -- Centre de Calcul
IN2P3/CNRS; Centre National de la Recherche Scientifique (CNRS); Conseil
R\'egional Ile-de-France; D\'epartement Physique Nucl\'eaire et Corpusculaire
(PNC-IN2P3/CNRS); D\'epartement Sciences de l'Univers (SDU-INSU/CNRS);
Institut Lagrange de Paris (ILP) Grant No.~LABEX ANR-10-LABX-63 within
the Investissements d'Avenir Programme Grant No.~ANR-11-IDEX-0004-02;
Germany -- Bundesministerium f\"ur Bildung und Forschung (BMBF); Deutsche
Forschungsgemeinschaft (DFG); Finanzministerium Baden-W\"urttemberg;
Helmholtz Alliance for Astroparticle Physics (HAP);
Helmholtz-Gemeinschaft Deutscher Forschungszentren (HGF); Ministerium
f\"ur Innovation, Wissenschaft und Forschung des Landes
Nordrhein-Westfalen; Ministerium f\"ur Wissenschaft, Forschung und Kunst
des Landes Baden-W\"urttemberg; Italy -- Istituto Nazionale di Fisica
Nucleare (INFN); Istituto Nazionale di Astrofisica (INAF); Ministero
dell'Istruzione, dell'Universit\'a e della Ricerca (MIUR); CETEMPS Center
of Excellence; Ministero degli Affari Esteri (MAE); M\'exico -- Consejo
Nacional de Ciencia y Tecnolog\'\i{}a (CONACYT) No.~167733; Universidad
Nacional Aut\'onoma de M\'exico (UNAM); PAPIIT DGAPA-UNAM; The Netherlands
-- Ministry of Education, Culture and Science; Netherlands Organisation
for Scientific Research (NWO); Dutch national e-infrastructure with the
support of SURF Cooperative; Poland -Ministry of Science and Higher
Education, grant No.~DIR/WK/2018/11; National Science Centre, Grants
No.~2013/08/M/ST9/00322, No.~2016/23/B/ST9/01635 and No.~HARMONIA
5--2013/10/M/ST9/00062, UMO-2016/22/M/ST9/00198; Portugal -- Portuguese
national funds and FEDER funds within Programa Operacional Factores de
Competitividade through Funda\c{c}\~ao para a Ci\^encia e a Tecnologia
(COMPETE); Romania -- Romanian Ministry of Education and Research, the
Program Nucleu within MCI (PN19150201/16N/2019 and PN19060102) and
project PN-III-P1-1.2-PCCDI-2017-0839/19PCCDI/2018 within PNCDI III;
Slovenia -- Slovenian Research Agency, grants P1-0031, P1-0385, I0-0033,
N1-0111; Spain -- Ministerio de Econom\'\i{}a, Industria y Competitividad
(FPA2017-85114-P and FPA2017-85197-P), Xunta de Galicia (ED431C
2017/07), Junta de Andaluc\'\i{}a (SOMM17/6104/UGR), Feder Funds, RENATA Red
Nacional Tem\'atica de Astropart\'\i{}culas (FPA2015-68783-REDT) and Mar\'\i{}a de
Maeztu Unit of Excellence (MDM-2016-0692); USA -- Department of Energy,
Contracts No.~DE-AC02-07CH11359, No.~DE-FR02-04ER41300,
No.~DE-FG02-99ER41107 and No.~DE-SC0011689; National Science Foundation,
Grant No.~0450696; The Grainger Foundation; Marie Curie-IRSES/EPLANET;
European Particle Physics Latin American Network; and UNESCO.
\end{sloppypar}


==> 2020-04-author_list-ZIP/elsarticle_authorlist.tex <==
% created on 2020-04-02

\author[75]{A.~Aab}
\author[67]{P.~Abreu}
\author[50,49]{M.~Aglietta}
\author[12]{J.M.~Albury}
\author[1]{I.~Allekotte}
\author[8,11]{A.~Almela}
\author[63]{J.~Alvarez Castillo}
\author[74]{J.~Alvarez-Mu\~niz}
\author[75]{R.~Alves Batista}
\author[58,49]{G.A.~Anastasi}
\author[82]{L.~Anchordoqui}
\author[8]{B.~Andrada}
\author[67]{S.~Andringa}
\author[47]{C.~Aramo}
\author[39]{P.R.~Ara\'ujo Ferreira}
\author[8]{H.~Asorey}
\author[67]{P.~Assis}
\author[9,10]{G.~Avila}
\author[70]{A.M.~Badescu}
\author[30]{A.~Bakalova}
\author[68]{A.~Balaceanu}
\author[56,47]{F.~Barbato}
\author[67]{R.J.~Barreira Luz}
\author[35]{K.H.~Becker}
\author[12]{J.A.~Bellido}
\author[34]{C.~Berat}
\author[58,49]{M.E.~Bertaina}
\author[1]{X.~Bertou}
\author[b]{P.L.~Biermann}
\author[39]{T.~Bister}
\author[32]{J.~Biteau}
\author[67]{A.~Blanco}
\author[30]{J.~Blazek}
\author[34]{C.~Bleve}
\author[30]{M.~Boh\'a\v{c}ov\'a}
\author[53,43]{D.~Boncioli}
\author[24]{C.~Bonifazi}
\author[19]{L.~Bonneau Arbeletche}
\author[64]{N.~Borodai}
\author[8]{A.M.~Botti}
\author[e]{J.~Brack}
\author[39]{T.~Bretz}
\author[39]{F.L.~Briechle}
\author[41]{P.~Buchholz}
\author[73]{A.~Bueno}
\author[14]{S.~Buitink}
\author[54,44]{M.~Buscemi}
\author[62]{K.S.~Caballero-Mora}
\author[55,46]{L.~Caccianiga}
\author[4]{L.~Calcagni}
\author[11,8]{A.~Cancio}
\author[75,77]{F.~Canfora}
\author[35]{I.~Caracas}
\author[73]{J.M.~Carceller}
\author[54,44]{R.~Caruso}
\author[50,49]{A.~Castellina}
\author[17]{F.~Catalani}
\author[45]{G.~Cataldi}
\author[67]{L.~Cazon}
\author[9]{M.~Cerda}
\author[20]{J.A.~Chinellato}
\author[74]{K.~Choi}
\author[30]{J.~Chudoba}
\author[31]{L.~Chytka}
\author[12]{R.W.~Clay}
\author[7]{A.C.~Cobos Cerutti}
\author[56,47]{R.~Colalillo}
\author[88]{A.~Coleman}
\author[52,45]{M.R.~Coluccia}
\author[67]{R.~Concei\c{c}\~ao}
\author[42,43]{A.~Condorelli}
\author[46,51]{G.~Consolati}
\author[9,10]{F.~Contreras}
\author[52,45]{F.~Convenga}
\author[80,h]{C.E.~Covault}
\author[5,3]{S.~Dasso}
\author[37]{K.~Daumiller}
\author[12]{B.R.~Dawson}
\author[12]{J.A.~Day}
\author[26]{R.M.~de Almeida}
\author[8,37]{J.~de Jes\'us}
\author[75,77]{S.J.~de Jong}
\author[75,77]{G.~De Mauro}
\author[24,25]{J.R.T.~de Mello Neto}
\author[42,43]{I.~De Mitri}
\author[26]{J.~de Oliveira}
\author[20]{D.~de Oliveira Franco}
\author[18]{V.~de Souza}
\author[36]{J.~Debatin}
\author[10]{M.~del R\'\i{}o}
\author[32]{O.~Deligny}
\author[64]{N.~Dhital}
\author[49]{A.~Di Matteo}
\author[20]{M.L.~D\'\i{}az Castro}
\author[20]{C.~Dobrigkeit}
\author[63]{J.C.~D'Olivo}
\author[41]{Q.~Dorosti}
\author[23]{R.C.~dos Anjos}
\author[4]{M.T.~Dova}
\author[30]{J.~Ebr}
\author[36,37]{R.~Engel}
\author[52,45]{I.~Epicoco}
\author[39]{M.~Erdmann}
\author[c]{C.O.~Escobar}
\author[8,11]{A.~Etchegoyen}
\author[75,78,77]{H.~Falcke}
\author[87]{J.~Farmer}
\author[85]{G.~Farrar}
\author[20]{A.C.~Fauth}
\author[c]{N.~Fazzini}
\author[38]{F.~Feldbusch}
\author[58,49]{F.~Fenu}
\author[84]{B.~Fick}
\author[8]{J.M.~Figueira}
\author[72,71]{A.~Filip\v{c}i\v{c}}
\author[75]{T.~Fodran}
\author[6]{M.M.~Freire}
\author[87,f]{T.~Fujii}
\author[8,11]{A.~Fuster}
\author[75]{C.~Galea}
\author[55,46]{C.~Galelli}
\author[7]{B.~Garc\'\i{}a}
\author[39]{A.L.~Garcia Vegas}
\author[38]{H.~Gemmeke}
\author[8,37]{F.~Gesualdi}
\author[68]{A.~Gherghel-Lascu}
\author[32]{P.L.~Ghia}
\author[75]{U.~Giaccari}
\author[46]{M.~Giammarchi}
\author[65]{M.~Giller}
\author[39]{J.~Glombitza}
\author[9]{F.~Gobbi}
\author[1]{G.~Golup}
\author[1]{M.~G\'omez Berisso}
\author[9,10]{P.F.~G\'omez Vitale}
\author[9]{J.P.~Gongora}
\author[8]{N.~Gonz\'alez}
\author[1,37]{I.~Goos}
\author[64]{D.~G\'ora}
\author[50,49]{A.~Gorgi}
\author[35]{M.~Gottowik}
\author[12]{T.D.~Grubb}
\author[56,47]{F.~Guarino}
\author[21]{G.P.~Guedes}
\author[49,58]{E.~Guido}
\author[37,8]{S.~Hahn}
\author[80]{R.~Halliday}
\author[8]{M.R.~Hampel}
\author[4]{P.~Hansen}
\author[1]{D.~Harari}
\author[12]{V.M.~Harvey}
\author[37]{A.~Haungs}
\author[39]{T.~Hebbeker}
\author[37]{D.~Heck}
\author[12]{G.C.~Hill}
\author[c]{C.~Hojvat}
\author[75,77]{J.R.~H\"orandel}
\author[31]{P.~Horvath}
\author[31]{M.~Hrabovsk\'y}
\author[37,14]{T.~Huege}
\author[8,37]{J.~Hulsman}
\author[54,44]{A.~Insolia}
\author[69]{P.G.~Isar}
\author[81]{J.A.~Johnsen}
\author[30]{J.~Jurysek}
\author[35]{A.~K\"a\"ap\"a}
\author[35]{K.H.~Kampert}
\author[37]{B.~Keilhauer}
\author[39]{J.~Kemp}
\author[37]{H.O.~Klages}
\author[38]{M.~Kleifges}
\author[9]{J.~Kleinfeller}
\author[36]{M.~K\"opke}
\author[71]{G.~Kukec Mezek}
\author[16]{B.L.~Lago}
\author[80]{D.~LaHurd}
\author[18]{R.G.~Lang}
\author[22]{M.A.~Leigui de Oliveira}
\author[37]{V.~Lenok}
\author[33]{A.~Letessier-Selvon}
\author[32]{I.~Lhenry-Yvon}
\author[54,44]{D.~Lo Presti}
\author[67]{L.~Lopes}
\author[59]{R.~L\'opez}
\author[80]{R.~Lorek}
\author[36]{Q.~Luce}
\author[8]{A.~Lucero}
\author[20]{A.~Machado Payeras}
\author[87]{M.~Malacari}
\author[52,45]{G.~Mancarella}
\author[30]{D.~Mandat}
\author[12]{B.C.~Manning}
\author[40]{J.~Manshanden}
\author[c]{P.~Mantsch}
\author[32]{S.~Marafico}
\author[4]{A.G.~Mariazzi}
\author[13]{I.C.~Mari\c{s}}
\author[52,45]{G.~Marsella}
\author[52,45]{D.~Martello}
\author[18]{H.~Martinez}
\author[59]{O.~Mart\'\i{}nez Bravo}
\author[53,43]{M.~Mastrodicasa}
\author[37]{H.J.~Mathes}
\author[83]{J.~Matthews}
\author[57,48]{G.~Matthiae}
\author[35]{E.~Mayotte}
\author[c]{P.O.~Mazur}
\author[63]{G.~Medina-Tanco}
\author[8]{D.~Melo}
\author[38]{A.~Menshikov}
\author[81]{K.-D.~Merenda}
\author[31]{S.~Michal}
\author[6]{M.I.~Micheletti}
\author[55,46]{L.~Miramonti}
\author[13]{D.~Mockler}
\author[1]{S.~Mollerach}
\author[34]{F.~Montanet}
\author[50,49]{C.~Morello}
\author[86]{M.~Mostaf\'a}
\author[8,37]{A.L.~M\"uller}
\author[20,d,24]{M.A.~Muller}
\author[14]{K.~Mulrey}
\author[49]{R.~Mussa}
\author[85]{M.~Muzio}
\author[35]{W.M.~Namasaka}
\author[63]{L.~Nellen}
\author[68]{M.~Niculescu-Oglinzanu}
\author[41]{M.~Niechciol}
\author[84,g]{D.~Nitz}
\author[29]{D.~Nosek}
\author[29]{V.~Novotny}
\author[31]{L.~No\v{z}ka}
\author[52,45]{A Nucita}
\author[28]{L.A.~N\'u\~nez}
\author[30]{M.~Palatka}
\author[2]{J.~Pallotta}
\author[52,45]{M.P.~Panetta}
\author[35]{P.~Papenbreer}
\author[74]{G.~Parente}
\author[59]{A.~Parra}
\author[30]{M.~Pech}
\author[74]{F.~Pedreira}
\author[64]{J.~P\c{e}kala}
\author[61]{R.~Pelayo}
\author[28]{J.~Pe\~na-Rodriguez}
\author[19]{J.~Perez Armand}
\author[8,37]{M.~Perlin}
\author[52,45]{L.~Perrone}
\author[39]{C.~Peters}
\author[42,43]{S.~Petrera}
\author[37]{T.~Pierog}
\author[67]{M.~Pimenta}
\author[54,44]{V.~Pirronello}
\author[8]{M.~Platino}
\author[75]{B.~Pont}
\author[77,75]{M.~Pothast}
\author[87]{P.~Privitera}
\author[30]{M.~Prouza}
\author[84]{A.~Puyleart}
\author[35]{S.~Querchfeld}
\author[35]{J.~Rautenberg}
\author[8]{D.~Ravignani}
\author[37,8]{M.~Reininghaus}
\author[30]{J.~Ridky}
\author[67]{F.~Riehn}
\author[41]{M.~Risse}
\author[2]{P.~Ristori}
\author[53,43]{V.~Rizi}
\author[19]{W.~Rodrigues de Carvalho}
\author[9]{J.~Rodriguez Rojo}
\author[8]{M.J.~Roncoroni}
\author[37]{M.~Roth}
\author[1]{E.~Roulet}
\author[5]{A.C.~Rovero}
\author[41]{P.~Ruehl}
\author[12]{S.J.~Saffi}
\author[68]{A.~Saftoiu}
\author[53,43]{F.~Salamida}
\author[59]{H.~Salazar}
\author[48]{G.~Salina}
\author[28]{J.D.~Sanabria Gomez}
\author[8]{F.~S\'anchez}
\author[19]{E.M.~Santos}
\author[30]{E.~Santos}
\author[81]{F.~Sarazin}
\author[67]{R.~Sarmento}
\author[8]{C.~Sarmiento-Cano}
\author[9]{R.~Sato}
\author[52,45,32]{P.~Savina}
\author[37]{C.~Sch\"afer}
\author[45]{V.~Scherini}
\author[37]{H.~Schieler}
\author[36,8]{M.~Schimassek}
\author[35]{M.~Schimp}
\author[37,8]{F.~Schl\"uter}
\author[36]{D.~Schmidt}
\author[76,14]{O.~Scholten}
\author[30]{P.~Schov\'anek}
\author[88,37]{F.G.~Schr\"oder}
\author[35]{S.~Schr\"oder}
\author[4]{S.J.~Sciutto}
\author[8,37]{M.~Scornavacche}
\author[15]{R.C.~Shellard}
\author[40]{G.~Sigl}
\author[8,37]{G.~Silli}
\author[68,h]{O.~Sima}
\author[87]{R.~\v{S}m\'\i{}da}
\author[86]{P.~Sommers}
\author[82]{J.F.~Soriano}
\author[34]{J.~Souchard}
\author[9]{R.~Squartini}
\author[37,8]{M.~Stadelmaier}
\author[68]{D.~Stanca}
\author[71]{S.~Stani\v{c}}
\author[64]{J.~Stasielak}
\author[34]{P.~Stassi}
\author[36,8]{A.~Streich}
\author[28]{M.~Su\'arez-Dur\'an}
\author[12]{T.~Sudholz}
\author[32]{T.~Suomij\"arvi}
\author[8]{A.D.~Supanitsky}
\author[31]{J.~\v{S}up\'\i{}k}
\author[66]{Z.~Szadkowski}
\author[36]{A.~Taboada}
\author[27]{A.~Tapia}
\author[77,75]{C.~Timmermans}
\author[30]{P.~Tobiska}
\author[17]{C.J.~Todero Peixoto}
\author[67]{B.~Tom\'e}
\author[74]{G.~Torralba Elipe}
\author[9]{A.~Travaini}
\author[30]{P.~Travnicek}
\author[53,43]{C.~Trimarelli}
\author[71]{M.~Trini}
\author[4]{M.~Tueros}
\author[37]{R.~Ulrich}
\author[37]{M.~Unger}
\author[39]{M.~Urban}
\author[31]{L.~Vaclavek}
\author[31]{M.~Vacula}
\author[63]{J.F.~Vald\'es Galicia}
\author[42,43]{I.~Vali\~no}
\author[56,47]{L.~Valore}
\author[75]{A.~van Vliet}
\author[59]{E.~Varela}
\author[63]{B.~Vargas C\'ardenas}
\author[28]{A.~V\'asquez-Ram\'\i{}rez}
\author[37]{D.~Veberi\v{c}}
\author[25]{C.~Ventura}
\author[4]{I.D.~Vergara Quispe}
\author[48]{V.~Verzi}
\author[30]{J.~Vicha}
\author[59]{L.~Villase\~nor}
\author[79]{J.~Vink}
\author[71]{S.~Vorobiov}
\author[4]{H.~Wahlberg}
\author[a]{A.A.~Watson}
\author[38]{M.~Weber}
\author[37]{A.~Weindl}
\author[81]{L.~Wiencke}
\author[64]{H.~Wilczy\'nski}
\author[14]{T.~Winchen}
\author[39]{M.~Wirtz}
\author[35]{D.~Wittkowski}
\author[8]{B.~Wundheiler}
\author[30]{A.~Yushkov}
\author[13]{O.~Zapparrata}
\author[74]{E.~Zas}
\author[71,72]{D.~Zavrtanik}
\author[72,71]{M.~Zavrtanik}
\author[71]{L.~Zehrer}
\author[60]{A.~Zepeda}
\author[41]{M.~Ziolkowski}
\author[54,44]{F.~Zuccarello}

\address[1]{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}
\address[2]{Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina}
\address[3]{Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina}
\address[4]{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}
\address[5]{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}
\address[6]{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}
\address[7]{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}
\address[8]{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\address[9]{Observatorio Pierre Auger, Malarg\"ue, Argentina}
\address[10]{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}
\address[11]{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}
\address[12]{University of Adelaide, Adelaide, S.A., Australia}
\address[13]{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}
\address[14]{Vrije Universiteit Brussels, Brussels, Belgium}
\address[15]{Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil}
\address[16]{Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil}
\address[17]{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}
\address[18]{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}
\address[19]{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}
\address[20]{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}
\address[21]{Universidade Estadual de Feira de Santana, Feira de Santana, Brazil}
\address[22]{Universidade Federal do ABC, Santo Andr\'e, SP, Brazil}
\address[23]{Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil}
\address[24]{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}
\address[25]{Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil}
\address[26]{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}
\address[27]{Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia}
\address[28]{Universidad Industrial de Santander, Bucaramanga, Colombia}
\address[29]{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}
\address[30]{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}
\address[31]{Palacky University, RCPTM, Olomouc, Czech Republic}
\address[32]{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}
\address[33]{Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Universit\'es Paris 6 et Paris 7, CNRS-IN2P3, Paris, France}
\address[34]{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}
\address[35]{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}
\address[36]{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}
\address[37]{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\address[38]{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}
\address[39]{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}
\address[40]{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}
\address[41]{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}
\address[42]{Gran Sasso Science Institute, L'Aquila, Italy}
\address[43]{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}
\address[44]{INFN, Sezione di Catania, Catania, Italy}
\address[45]{INFN, Sezione di Lecce, Lecce, Italy}
\address[46]{INFN, Sezione di Milano, Milano, Italy}
\address[47]{INFN, Sezione di Napoli, Napoli, Italy}
\address[48]{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}
\address[49]{INFN, Sezione di Torino, Torino, Italy}
\address[50]{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\address[51]{Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy}
\address[52]{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\address[53]{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\address[54]{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\address[55]{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\address[56]{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\address[57]{Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy}
\address[58]{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\address[59]{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}
\address[60]{Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico, D.F., M\'exico}
\address[61]{Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico}
\address[62]{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}
\address[63]{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}
\address[64]{Institute of Nuclear Physics PAN, Krakow, Poland}
\address[65]{University of \L{}\'od\'z, Faculty of Astrophysics, \L{}\'od\'z, Poland}
\address[66]{University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland}
\address[67]{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}
\address[68]{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}
\address[69]{Institute of Space Science, Bucharest-Magurele, Romania}
\address[70]{University Politehnica of Bucharest, Bucharest, Romania}
\address[71]{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}
\address[72]{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\address[73]{Universidad de Granada and C.A.F.P.E., Granada, Spain}
\address[74]{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}
\address[75]{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\address[76]{KVI -- Center for Advanced Radiation Technology, University of Groningen, Groningen, The Netherlands}
\address[77]{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\address[78]{Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands}
\address[79]{Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands}
\address[80]{Case Western Reserve University, Cleveland, OH, USA}
\address[81]{Colorado School of Mines, Golden, CO, USA}
\address[82]{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}
\address[83]{Louisiana State University, Baton Rouge, LA, USA}
\address[84]{Michigan Technological University, Houghton, MI, USA}
\address[85]{New York University, New York, NY, USA}
\address[86]{Pennsylvania State University, University Park, PA, USA}
\address[87]{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}
\address[88]{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}
\address[a]{School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom}
\address[b]{Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany}
\address[c]{Fermi National Accelerator Laboratory, USA}
\address[d]{also at Universidade Federal de Alfenas, Po\c{c}os de Caldas, Brazil}
\address[e]{Colorado State University, Fort Collins, CO, USA}
\address[f]{now at Hakubi Center for Advanced Research and Graduate School of Science, Kyoto University, Kyoto, Japan}
\address[g]{also at Karlsruhe Institute of Technology, Karlsruhe, Germany}
\address[h]{also at Radboud Universtiy Nijmegen, Nijmegen, The Netherlands}


==> 2020-04-author_list-ZIP/jcappub_authorlist.tex <==
% created on 2020-04-02

\author[75]{A.~Aab,}
\author[67]{P.~Abreu,}
\author[50,49]{M.~Aglietta,}
\author[12]{J.M.~Albury,}
\author[1]{I.~Allekotte,}
\author[8,11]{A.~Almela,}
\author[63]{J.~Alvarez Castillo,}
\author[74]{J.~Alvarez-Mu\~niz,}
\author[75]{R.~Alves Batista,}
\author[58,49]{G.A.~Anastasi,}
\author[82]{L.~Anchordoqui,}
\author[8]{B.~Andrada,}
\author[67]{S.~Andringa,}
\author[47]{C.~Aramo,}
\author[39]{P.R.~Ara\'ujo Ferreira,}
\author[8]{H.~Asorey,}
\author[67]{P.~Assis,}
\author[9,10]{G.~Avila,}
\author[70]{A.M.~Badescu,}
\author[30]{A.~Bakalova,}
\author[68]{A.~Balaceanu,}
\author[56,47]{F.~Barbato,}
\author[67]{R.J.~Barreira Luz,}
\author[35]{K.H.~Becker,}
\author[12]{J.A.~Bellido,}
\author[34]{C.~Berat,}
\author[58,49]{M.E.~Bertaina,}
\author[1]{X.~Bertou,}
\author[b]{P.L.~Biermann,}
\author[39]{T.~Bister,}
\author[32]{J.~Biteau,}
\author[67]{A.~Blanco,}
\author[30]{J.~Blazek,}
\author[34]{C.~Bleve,}
\author[30]{M.~Boh\'a\v{c}ov\'a,}
\author[53,43]{D.~Boncioli,}
\author[24]{C.~Bonifazi,}
\author[19]{L.~Bonneau Arbeletche,}
\author[64]{N.~Borodai,}
\author[8]{A.M.~Botti,}
\author[e]{J.~Brack,}
\author[39]{T.~Bretz,}
\author[39]{F.L.~Briechle,}
\author[41]{P.~Buchholz,}
\author[73]{A.~Bueno,}
\author[14]{S.~Buitink,}
\author[54,44]{M.~Buscemi,}
\author[62]{K.S.~Caballero-Mora,}
\author[55,46]{L.~Caccianiga,}
\author[4]{L.~Calcagni,}
\author[11,8]{A.~Cancio,}
\author[75,77]{F.~Canfora,}
\author[35]{I.~Caracas,}
\author[73]{J.M.~Carceller,}
\author[54,44]{R.~Caruso,}
\author[50,49]{A.~Castellina,}
\author[17]{F.~Catalani,}
\author[45]{G.~Cataldi,}
\author[67]{L.~Cazon,}
\author[9]{M.~Cerda,}
\author[20]{J.A.~Chinellato,}
\author[74]{K.~Choi,}
\author[30]{J.~Chudoba,}
\author[31]{L.~Chytka,}
\author[12]{R.W.~Clay,}
\author[7]{A.C.~Cobos Cerutti,}
\author[56,47]{R.~Colalillo,}
\author[88]{A.~Coleman,}
\author[52,45]{M.R.~Coluccia,}
\author[67]{R.~Concei\c{c}\~ao,}
\author[42,43]{A.~Condorelli,}
\author[46,51]{G.~Consolati,}
\author[9,10]{F.~Contreras,}
\author[52,45]{F.~Convenga,}
\author[80,h]{C.E.~Covault,}
\author[5,3]{S.~Dasso,}
\author[37]{K.~Daumiller,}
\author[12]{B.R.~Dawson,}
\author[12]{J.A.~Day,}
\author[26]{R.M.~de Almeida,}
\author[8,37]{J.~de Jes\'us,}
\author[75,77]{S.J.~de Jong,}
\author[75,77]{G.~De Mauro,}
\author[24,25]{J.R.T.~de Mello Neto,}
\author[42,43]{I.~De Mitri,}
\author[26]{J.~de Oliveira,}
\author[20]{D.~de Oliveira Franco,}
\author[18]{V.~de Souza,}
\author[36]{J.~Debatin,}
\author[10]{M.~del R\'\i{}o,}
\author[32]{O.~Deligny,}
\author[64]{N.~Dhital,}
\author[49]{A.~Di Matteo,}
\author[20]{M.L.~D\'\i{}az Castro,}
\author[20]{C.~Dobrigkeit,}
\author[63]{J.C.~D'Olivo,}
\author[41]{Q.~Dorosti,}
\author[23]{R.C.~dos Anjos,}
\author[4]{M.T.~Dova,}
\author[30]{J.~Ebr,}
\author[36,37]{R.~Engel,}
\author[52,45]{I.~Epicoco,}
\author[39]{M.~Erdmann,}
\author[c]{C.O.~Escobar,}
\author[8,11]{A.~Etchegoyen,}
\author[75,78,77]{H.~Falcke,}
\author[87]{J.~Farmer,}
\author[85]{G.~Farrar,}
\author[20]{A.C.~Fauth,}
\author[c]{N.~Fazzini,}
\author[38]{F.~Feldbusch,}
\author[58,49]{F.~Fenu,}
\author[84]{B.~Fick,}
\author[8]{J.M.~Figueira,}
\author[72,71]{A.~Filip\v{c}i\v{c},}
\author[75]{T.~Fodran,}
\author[6]{M.M.~Freire,}
\author[87,f]{T.~Fujii,}
\author[8,11]{A.~Fuster,}
\author[75]{C.~Galea,}
\author[55,46]{C.~Galelli,}
\author[7]{B.~Garc\'\i{}a,}
\author[39]{A.L.~Garcia Vegas,}
\author[38]{H.~Gemmeke,}
\author[8,37]{F.~Gesualdi,}
\author[68]{A.~Gherghel-Lascu,}
\author[32]{P.L.~Ghia,}
\author[75]{U.~Giaccari,}
\author[46]{M.~Giammarchi,}
\author[65]{M.~Giller,}
\author[39]{J.~Glombitza,}
\author[9]{F.~Gobbi,}
\author[1]{G.~Golup,}
\author[1]{M.~G\'omez Berisso,}
\author[9,10]{P.F.~G\'omez Vitale,}
\author[9]{J.P.~Gongora,}
\author[8]{N.~Gonz\'alez,}
\author[1,37]{I.~Goos,}
\author[64]{D.~G\'ora,}
\author[50,49]{A.~Gorgi,}
\author[35]{M.~Gottowik,}
\author[12]{T.D.~Grubb,}
\author[56,47]{F.~Guarino,}
\author[21]{G.P.~Guedes,}
\author[49,58]{E.~Guido,}
\author[37,8]{S.~Hahn,}
\author[80]{R.~Halliday,}
\author[8]{M.R.~Hampel,}
\author[4]{P.~Hansen,}
\author[1]{D.~Harari,}
\author[12]{V.M.~Harvey,}
\author[37]{A.~Haungs,}
\author[39]{T.~Hebbeker,}
\author[37]{D.~Heck,}
\author[12]{G.C.~Hill,}
\author[c]{C.~Hojvat,}
\author[75,77]{J.R.~H\"orandel,}
\author[31]{P.~Horvath,}
\author[31]{M.~Hrabovsk\'y,}
\author[37,14]{T.~Huege,}
\author[8,37]{J.~Hulsman,}
\author[54,44]{A.~Insolia,}
\author[69]{P.G.~Isar,}
\author[81]{J.A.~Johnsen,}
\author[30]{J.~Jurysek,}
\author[35]{A.~K\"a\"ap\"a,}
\author[35]{K.H.~Kampert,}
\author[37]{B.~Keilhauer,}
\author[39]{J.~Kemp,}
\author[37]{H.O.~Klages,}
\author[38]{M.~Kleifges,}
\author[9]{J.~Kleinfeller,}
\author[36]{M.~K\"opke,}
\author[71]{G.~Kukec Mezek,}
\author[16]{B.L.~Lago,}
\author[80]{D.~LaHurd,}
\author[18]{R.G.~Lang,}
\author[22]{M.A.~Leigui de Oliveira,}
\author[37]{V.~Lenok,}
\author[33]{A.~Letessier-Selvon,}
\author[32]{I.~Lhenry-Yvon,}
\author[54,44]{D.~Lo Presti,}
\author[67]{L.~Lopes,}
\author[59]{R.~L\'opez,}
\author[80]{R.~Lorek,}
\author[36]{Q.~Luce,}
\author[8]{A.~Lucero,}
\author[20]{A.~Machado Payeras,}
\author[87]{M.~Malacari,}
\author[52,45]{G.~Mancarella,}
\author[30]{D.~Mandat,}
\author[12]{B.C.~Manning,}
\author[40]{J.~Manshanden,}
\author[c]{P.~Mantsch,}
\author[32]{S.~Marafico,}
\author[4]{A.G.~Mariazzi,}
\author[13]{I.C.~Mari\c{s},}
\author[52,45]{G.~Marsella,}
\author[52,45]{D.~Martello,}
\author[18]{H.~Martinez,}
\author[59]{O.~Mart\'\i{}nez Bravo,}
\author[53,43]{M.~Mastrodicasa,}
\author[37]{H.J.~Mathes,}
\author[83]{J.~Matthews,}
\author[57,48]{G.~Matthiae,}
\author[35]{E.~Mayotte,}
\author[c]{P.O.~Mazur,}
\author[63]{G.~Medina-Tanco,}
\author[8]{D.~Melo,}
\author[38]{A.~Menshikov,}
\author[81]{K.-D.~Merenda,}
\author[31]{S.~Michal,}
\author[6]{M.I.~Micheletti,}
\author[55,46]{L.~Miramonti,}
\author[13]{D.~Mockler,}
\author[1]{S.~Mollerach,}
\author[34]{F.~Montanet,}
\author[50,49]{C.~Morello,}
\author[86]{M.~Mostaf\'a,}
\author[8,37]{A.L.~M\"uller,}
\author[20,d,24]{M.A.~Muller,}
\author[14]{K.~Mulrey,}
\author[49]{R.~Mussa,}
\author[85]{M.~Muzio,}
\author[35]{W.M.~Namasaka,}
\author[63]{L.~Nellen,}
\author[68]{M.~Niculescu-Oglinzanu,}
\author[41]{M.~Niechciol,}
\author[84,g]{D.~Nitz,}
\author[29]{D.~Nosek,}
\author[29]{V.~Novotny,}
\author[31]{L.~No\v{z}ka,}
\author[52,45]{A Nucita,}
\author[28]{L.A.~N\'u\~nez,}
\author[30]{M.~Palatka,}
\author[2]{J.~Pallotta,}
\author[52,45]{M.P.~Panetta,}
\author[35]{P.~Papenbreer,}
\author[74]{G.~Parente,}
\author[59]{A.~Parra,}
\author[30]{M.~Pech,}
\author[74]{F.~Pedreira,}
\author[64]{J.~P\c{e}kala,}
\author[61]{R.~Pelayo,}
\author[28]{J.~Pe\~na-Rodriguez,}
\author[19]{J.~Perez Armand,}
\author[8,37]{M.~Perlin,}
\author[52,45]{L.~Perrone,}
\author[39]{C.~Peters,}
\author[42,43]{S.~Petrera,}
\author[37]{T.~Pierog,}
\author[67]{M.~Pimenta,}
\author[54,44]{V.~Pirronello,}
\author[8]{M.~Platino,}
\author[75]{B.~Pont,}
\author[77,75]{M.~Pothast,}
\author[87]{P.~Privitera,}
\author[30]{M.~Prouza,}
\author[84]{A.~Puyleart,}
\author[35]{S.~Querchfeld,}
\author[35]{J.~Rautenberg,}
\author[8]{D.~Ravignani,}
\author[37,8]{M.~Reininghaus,}
\author[30]{J.~Ridky,}
\author[67]{F.~Riehn,}
\author[41]{M.~Risse,}
\author[2]{P.~Ristori,}
\author[53,43]{V.~Rizi,}
\author[19]{W.~Rodrigues de Carvalho,}
\author[9]{J.~Rodriguez Rojo,}
\author[8]{M.J.~Roncoroni,}
\author[37]{M.~Roth,}
\author[1]{E.~Roulet,}
\author[5]{A.C.~Rovero,}
\author[41]{P.~Ruehl,}
\author[12]{S.J.~Saffi,}
\author[68]{A.~Saftoiu,}
\author[53,43]{F.~Salamida,}
\author[59]{H.~Salazar,}
\author[48]{G.~Salina,}
\author[28]{J.D.~Sanabria Gomez,}
\author[8]{F.~S\'anchez,}
\author[19]{E.M.~Santos,}
\author[30]{E.~Santos,}
\author[81]{F.~Sarazin,}
\author[67]{R.~Sarmento,}
\author[8]{C.~Sarmiento-Cano,}
\author[9]{R.~Sato,}
\author[52,45,32]{P.~Savina,}
\author[37]{C.~Sch\"afer,}
\author[45]{V.~Scherini,}
\author[37]{H.~Schieler,}
\author[36,8]{M.~Schimassek,}
\author[35]{M.~Schimp,}
\author[37,8]{F.~Schl\"uter,}
\author[36]{D.~Schmidt,}
\author[76,14]{O.~Scholten,}
\author[30]{P.~Schov\'anek,}
\author[88,37]{F.G.~Schr\"oder,}
\author[35]{S.~Schr\"oder,}
\author[4]{S.J.~Sciutto,}
\author[8,37]{M.~Scornavacche,}
\author[15]{R.C.~Shellard,}
\author[40]{G.~Sigl,}
\author[8,37]{G.~Silli,}
\author[68,h]{O.~Sima,}
\author[87]{R.~\v{S}m\'\i{}da,}
\author[86]{P.~Sommers,}
\author[82]{J.F.~Soriano,}
\author[34]{J.~Souchard,}
\author[9]{R.~Squartini,}
\author[37,8]{M.~Stadelmaier,}
\author[68]{D.~Stanca,}
\author[71]{S.~Stani\v{c},}
\author[64]{J.~Stasielak,}
\author[34]{P.~Stassi,}
\author[36,8]{A.~Streich,}
\author[28]{M.~Su\'arez-Dur\'an,}
\author[12]{T.~Sudholz,}
\author[32]{T.~Suomij\"arvi,}
\author[8]{A.D.~Supanitsky,}
\author[31]{J.~\v{S}up\'\i{}k,}
\author[66]{Z.~Szadkowski,}
\author[36]{A.~Taboada,}
\author[27]{A.~Tapia,}
\author[77,75]{C.~Timmermans,}
\author[30]{P.~Tobiska,}
\author[17]{C.J.~Todero Peixoto,}
\author[67]{B.~Tom\'e,}
\author[74]{G.~Torralba Elipe,}
\author[9]{A.~Travaini,}
\author[30]{P.~Travnicek,}
\author[53,43]{C.~Trimarelli,}
\author[71]{M.~Trini,}
\author[4]{M.~Tueros,}
\author[37]{R.~Ulrich,}
\author[37]{M.~Unger,}
\author[39]{M.~Urban,}
\author[31]{L.~Vaclavek,}
\author[31]{M.~Vacula,}
\author[63]{J.F.~Vald\'es Galicia,}
\author[42,43]{I.~Vali\~no,}
\author[56,47]{L.~Valore,}
\author[75]{A.~van Vliet,}
\author[59]{E.~Varela,}
\author[63]{B.~Vargas C\'ardenas,}
\author[28]{A.~V\'asquez-Ram\'\i{}rez,}
\author[37]{D.~Veberi\v{c},}
\author[25]{C.~Ventura,}
\author[4]{I.D.~Vergara Quispe,}
\author[48]{V.~Verzi,}
\author[30]{J.~Vicha,}
\author[59]{L.~Villase\~nor,}
\author[79]{J.~Vink,}
\author[71]{S.~Vorobiov,}
\author[4]{H.~Wahlberg,}
\author[a]{A.A.~Watson,}
\author[38]{M.~Weber,}
\author[37]{A.~Weindl,}
\author[81]{L.~Wiencke,}
\author[64]{H.~Wilczy\'nski,}
\author[14]{T.~Winchen,}
\author[39]{M.~Wirtz,}
\author[35]{D.~Wittkowski,}
\author[8]{B.~Wundheiler,}
\author[30]{A.~Yushkov,}
\author[13]{O.~Zapparrata,}
\author[74]{E.~Zas,}
\author[71,72]{D.~Zavrtanik,}
\author[72,71]{M.~Zavrtanik,}
\author[71]{L.~Zehrer,}
\author[60]{A.~Zepeda,}
\author[41]{M.~Ziolkowski,}
\author[54,44]{and F.~Zuccarello}

\affiliation[1]{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}
\affiliation[2]{Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina}
\affiliation[3]{Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina}
\affiliation[4]{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}
\affiliation[5]{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}
\affiliation[6]{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}
\affiliation[7]{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}
\affiliation[8]{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation[9]{Observatorio Pierre Auger, Malarg\"ue, Argentina}
\affiliation[10]{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}
\affiliation[11]{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}
\affiliation[12]{University of Adelaide, Adelaide, S.A., Australia}
\affiliation[13]{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}
\affiliation[14]{Vrije Universiteit Brussels, Brussels, Belgium}
\affiliation[15]{Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil}
\affiliation[16]{Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil}
\affiliation[17]{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}
\affiliation[18]{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}
\affiliation[19]{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}
\affiliation[20]{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}
\affiliation[21]{Universidade Estadual de Feira de Santana, Feira de Santana, Brazil}
\affiliation[22]{Universidade Federal do ABC, Santo Andr\'e, SP, Brazil}
\affiliation[23]{Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil}
\affiliation[24]{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}
\affiliation[25]{Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil}
\affiliation[26]{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}
\affiliation[27]{Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia}
\affiliation[28]{Universidad Industrial de Santander, Bucaramanga, Colombia}
\affiliation[29]{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}
\affiliation[30]{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}
\affiliation[31]{Palacky University, RCPTM, Olomouc, Czech Republic}
\affiliation[32]{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}
\affiliation[33]{Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Universit\'es Paris 6 et Paris 7, CNRS-IN2P3, Paris, France}
\affiliation[34]{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}
\affiliation[35]{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}
\affiliation[36]{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}
\affiliation[37]{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\affiliation[38]{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}
\affiliation[39]{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}
\affiliation[40]{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}
\affiliation[41]{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}
\affiliation[42]{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation[43]{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}
\affiliation[44]{INFN, Sezione di Catania, Catania, Italy}
\affiliation[45]{INFN, Sezione di Lecce, Lecce, Italy}
\affiliation[46]{INFN, Sezione di Milano, Milano, Italy}
\affiliation[47]{INFN, Sezione di Napoli, Napoli, Italy}
\affiliation[48]{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}
\affiliation[49]{INFN, Sezione di Torino, Torino, Italy}
\affiliation[50]{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation[51]{Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy}
\affiliation[52]{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation[53]{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation[54]{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation[55]{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation[56]{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation[57]{Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy}
\affiliation[58]{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation[59]{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}
\affiliation[60]{Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico, D.F., M\'exico}
\affiliation[61]{Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico}
\affiliation[62]{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}
\affiliation[63]{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}
\affiliation[64]{Institute of Nuclear Physics PAN, Krakow, Poland}
\affiliation[65]{University of \L{}\'od\'z, Faculty of Astrophysics, \L{}\'od\'z, Poland}
\affiliation[66]{University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland}
\affiliation[67]{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}
\affiliation[68]{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}
\affiliation[69]{Institute of Space Science, Bucharest-Magurele, Romania}
\affiliation[70]{University Politehnica of Bucharest, Bucharest, Romania}
\affiliation[71]{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}
\affiliation[72]{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\affiliation[73]{Universidad de Granada and C.A.F.P.E., Granada, Spain}
\affiliation[74]{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}
\affiliation[75]{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation[76]{KVI -- Center for Advanced Radiation Technology, University of Groningen, Groningen, The Netherlands}
\affiliation[77]{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\affiliation[78]{Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands}
\affiliation[79]{Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands}
\affiliation[80]{Case Western Reserve University, Cleveland, OH, USA}
\affiliation[81]{Colorado School of Mines, Golden, CO, USA}
\affiliation[82]{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}
\affiliation[83]{Louisiana State University, Baton Rouge, LA, USA}
\affiliation[84]{Michigan Technological University, Houghton, MI, USA}
\affiliation[85]{New York University, New York, NY, USA}
\affiliation[86]{Pennsylvania State University, University Park, PA, USA}
\affiliation[87]{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}
\affiliation[88]{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}
\affiliation[]{-----}
\affiliation[a]{School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom}
\affiliation[b]{Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany}
\affiliation[c]{Fermi National Accelerator Laboratory, USA}
\affiliation[d]{also at Universidade Federal de Alfenas, Po\c{c}os de Caldas, Brazil}
\affiliation[e]{Colorado State University, Fort Collins, CO, USA}
\affiliation[f]{now at Hakubi Center for Advanced Research and Graduate School of Science, Kyoto University, Kyoto, Japan}
\affiliation[g]{also at Karlsruhe Institute of Technology, Karlsruhe, Germany}
\affiliation[h]{also at Radboud Universtiy Nijmegen, Nijmegen, The Netherlands}


==> 2020-04-author_list-ZIP/jhep_authorlist.tex <==
% created on 2020-04-02

\author{
A.~Aab$^{75}$,
P.~Abreu$^{67}$,
M.~Aglietta$^{50,49}$,
J.M.~Albury$^{12}$,
I.~Allekotte$^{1}$,
A.~Almela$^{8,11}$,
J.~Alvarez Castillo$^{63}$,
J.~Alvarez-Mu\~niz$^{74}$,
R.~Alves Batista$^{75}$,
G.A.~Anastasi$^{58,49}$,
L.~Anchordoqui$^{82}$,
B.~Andrada$^{8}$,
S.~Andringa$^{67}$,
C.~Aramo$^{47}$,
P.R.~Ara\'ujo Ferreira$^{39}$,
H.~Asorey$^{8}$,
P.~Assis$^{67}$,
G.~Avila$^{9,10}$,
A.M.~Badescu$^{70}$,
A.~Bakalova$^{30}$,
A.~Balaceanu$^{68}$,
F.~Barbato$^{56,47}$,
R.J.~Barreira Luz$^{67}$,
K.H.~Becker$^{35}$,
J.A.~Bellido$^{12}$,
C.~Berat$^{34}$,
M.E.~Bertaina$^{58,49}$,
X.~Bertou$^{1}$,
P.L.~Biermann$^{b}$,
T.~Bister$^{39}$,
J.~Biteau$^{32}$,
A.~Blanco$^{67}$,
J.~Blazek$^{30}$,
C.~Bleve$^{34}$,
M.~Boh\'a\v{c}ov\'a$^{30}$,
D.~Boncioli$^{53,43}$,
C.~Bonifazi$^{24}$,
L.~Bonneau Arbeletche$^{19}$,
N.~Borodai$^{64}$,
A.M.~Botti$^{8}$,
J.~Brack$^{e}$,
T.~Bretz$^{39}$,
F.L.~Briechle$^{39}$,
P.~Buchholz$^{41}$,
A.~Bueno$^{73}$,
S.~Buitink$^{14}$,
M.~Buscemi$^{54,44}$,
K.S.~Caballero-Mora$^{62}$,
L.~Caccianiga$^{55,46}$,
L.~Calcagni$^{4}$,
A.~Cancio$^{11,8}$,
F.~Canfora$^{75,77}$,
I.~Caracas$^{35}$,
J.M.~Carceller$^{73}$,
R.~Caruso$^{54,44}$,
A.~Castellina$^{50,49}$,
F.~Catalani$^{17}$,
G.~Cataldi$^{45}$,
L.~Cazon$^{67}$,
M.~Cerda$^{9}$,
J.A.~Chinellato$^{20}$,
K.~Choi$^{74}$,
J.~Chudoba$^{30}$,
L.~Chytka$^{31}$,
R.W.~Clay$^{12}$,
A.C.~Cobos Cerutti$^{7}$,
R.~Colalillo$^{56,47}$,
A.~Coleman$^{88}$,
M.R.~Coluccia$^{52,45}$,
R.~Concei\c{c}\~ao$^{67}$,
A.~Condorelli$^{42,43}$,
G.~Consolati$^{46,51}$,
F.~Contreras$^{9,10}$,
F.~Convenga$^{52,45}$,
C.E.~Covault$^{80,h}$,
S.~Dasso$^{5,3}$,
K.~Daumiller$^{37}$,
B.R.~Dawson$^{12}$,
J.A.~Day$^{12}$,
R.M.~de Almeida$^{26}$,
J.~de Jes\'us$^{8,37}$,
S.J.~de Jong$^{75,77}$,
G.~De Mauro$^{75,77}$,
J.R.T.~de Mello Neto$^{24,25}$,
I.~De Mitri$^{42,43}$,
J.~de Oliveira$^{26}$,
D.~de Oliveira Franco$^{20}$,
V.~de Souza$^{18}$,
J.~Debatin$^{36}$,
M.~del R\'\i{}o$^{10}$,
O.~Deligny$^{32}$,
N.~Dhital$^{64}$,
A.~Di Matteo$^{49}$,
M.L.~D\'\i{}az Castro$^{20}$,
C.~Dobrigkeit$^{20}$,
J.C.~D'Olivo$^{63}$,
Q.~Dorosti$^{41}$,
R.C.~dos Anjos$^{23}$,
M.T.~Dova$^{4}$,
J.~Ebr$^{30}$,
R.~Engel$^{36,37}$,
I.~Epicoco$^{52,45}$,
M.~Erdmann$^{39}$,
C.O.~Escobar$^{c}$,
A.~Etchegoyen$^{8,11}$,
H.~Falcke$^{75,78,77}$,
J.~Farmer$^{87}$,
G.~Farrar$^{85}$,
A.C.~Fauth$^{20}$,
N.~Fazzini$^{c}$,
F.~Feldbusch$^{38}$,
F.~Fenu$^{58,49}$,
B.~Fick$^{84}$,
J.M.~Figueira$^{8}$,
A.~Filip\v{c}i\v{c}$^{72,71}$,
T.~Fodran$^{75}$,
M.M.~Freire$^{6}$,
T.~Fujii$^{87,f}$,
A.~Fuster$^{8,11}$,
C.~Galea$^{75}$,
C.~Galelli$^{55,46}$,
B.~Garc\'\i{}a$^{7}$,
A.L.~Garcia Vegas$^{39}$,
H.~Gemmeke$^{38}$,
F.~Gesualdi$^{8,37}$,
A.~Gherghel-Lascu$^{68}$,
P.L.~Ghia$^{32}$,
U.~Giaccari$^{75}$,
M.~Giammarchi$^{46}$,
M.~Giller$^{65}$,
J.~Glombitza$^{39}$,
F.~Gobbi$^{9}$,
G.~Golup$^{1}$,
M.~G\'omez Berisso$^{1}$,
P.F.~G\'omez Vitale$^{9,10}$,
J.P.~Gongora$^{9}$,
N.~Gonz\'alez$^{8}$,
I.~Goos$^{1,37}$,
D.~G\'ora$^{64}$,
A.~Gorgi$^{50,49}$,
M.~Gottowik$^{35}$,
T.D.~Grubb$^{12}$,
F.~Guarino$^{56,47}$,
G.P.~Guedes$^{21}$,
E.~Guido$^{49,58}$,
S.~Hahn$^{37,8}$,
R.~Halliday$^{80}$,
M.R.~Hampel$^{8}$,
P.~Hansen$^{4}$,
D.~Harari$^{1}$,
V.M.~Harvey$^{12}$,
A.~Haungs$^{37}$,
T.~Hebbeker$^{39}$,
D.~Heck$^{37}$,
G.C.~Hill$^{12}$,
C.~Hojvat$^{c}$,
J.R.~H\"orandel$^{75,77}$,
P.~Horvath$^{31}$,
M.~Hrabovsk\'y$^{31}$,
T.~Huege$^{37,14}$,
J.~Hulsman$^{8,37}$,
A.~Insolia$^{54,44}$,
P.G.~Isar$^{69}$,
J.A.~Johnsen$^{81}$,
J.~Jurysek$^{30}$,
A.~K\"a\"ap\"a$^{35}$,
K.H.~Kampert$^{35}$,
B.~Keilhauer$^{37}$,
J.~Kemp$^{39}$,
H.O.~Klages$^{37}$,
M.~Kleifges$^{38}$,
J.~Kleinfeller$^{9}$,
M.~K\"opke$^{36}$,
G.~Kukec Mezek$^{71}$,
B.L.~Lago$^{16}$,
D.~LaHurd$^{80}$,
R.G.~Lang$^{18}$,
M.A.~Leigui de Oliveira$^{22}$,
V.~Lenok$^{37}$,
A.~Letessier-Selvon$^{33}$,
I.~Lhenry-Yvon$^{32}$,
D.~Lo Presti$^{54,44}$,
L.~Lopes$^{67}$,
R.~L\'opez$^{59}$,
R.~Lorek$^{80}$,
Q.~Luce$^{36}$,
A.~Lucero$^{8}$,
A.~Machado Payeras$^{20}$,
M.~Malacari$^{87}$,
G.~Mancarella$^{52,45}$,
D.~Mandat$^{30}$,
B.C.~Manning$^{12}$,
J.~Manshanden$^{40}$,
P.~Mantsch$^{c}$,
S.~Marafico$^{32}$,
A.G.~Mariazzi$^{4}$,
I.C.~Mari\c{s}$^{13}$,
G.~Marsella$^{52,45}$,
D.~Martello$^{52,45}$,
H.~Martinez$^{18}$,
O.~Mart\'\i{}nez Bravo$^{59}$,
M.~Mastrodicasa$^{53,43}$,
H.J.~Mathes$^{37}$,
J.~Matthews$^{83}$,
G.~Matthiae$^{57,48}$,
E.~Mayotte$^{35}$,
P.O.~Mazur$^{c}$,
G.~Medina-Tanco$^{63}$,
D.~Melo$^{8}$,
A.~Menshikov$^{38}$,
K.-D.~Merenda$^{81}$,
S.~Michal$^{31}$,
M.I.~Micheletti$^{6}$,
L.~Miramonti$^{55,46}$,
D.~Mockler$^{13}$,
S.~Mollerach$^{1}$,
F.~Montanet$^{34}$,
C.~Morello$^{50,49}$,
M.~Mostaf\'a$^{86}$,
A.L.~M\"uller$^{8,37}$,
M.A.~Muller$^{20,d,24}$,
K.~Mulrey$^{14}$,
R.~Mussa$^{49}$,
M.~Muzio$^{85}$,
W.M.~Namasaka$^{35}$,
L.~Nellen$^{63}$,
M.~Niculescu-Oglinzanu$^{68}$,
M.~Niechciol$^{41}$,
D.~Nitz$^{84,g}$,
D.~Nosek$^{29}$,
V.~Novotny$^{29}$,
L.~No\v{z}ka$^{31}$,
A Nucita$^{52,45}$,
L.A.~N\'u\~nez$^{28}$,
M.~Palatka$^{30}$,
J.~Pallotta$^{2}$,
M.P.~Panetta$^{52,45}$,
P.~Papenbreer$^{35}$,
G.~Parente$^{74}$,
A.~Parra$^{59}$,
M.~Pech$^{30}$,
F.~Pedreira$^{74}$,
J.~P\c{e}kala$^{64}$,
R.~Pelayo$^{61}$,
J.~Pe\~na-Rodriguez$^{28}$,
J.~Perez Armand$^{19}$,
M.~Perlin$^{8,37}$,
L.~Perrone$^{52,45}$,
C.~Peters$^{39}$,
S.~Petrera$^{42,43}$,
T.~Pierog$^{37}$,
M.~Pimenta$^{67}$,
V.~Pirronello$^{54,44}$,
M.~Platino$^{8}$,
B.~Pont$^{75}$,
M.~Pothast$^{77,75}$,
P.~Privitera$^{87}$,
M.~Prouza$^{30}$,
A.~Puyleart$^{84}$,
S.~Querchfeld$^{35}$,
J.~Rautenberg$^{35}$,
D.~Ravignani$^{8}$,
M.~Reininghaus$^{37,8}$,
J.~Ridky$^{30}$,
F.~Riehn$^{67}$,
M.~Risse$^{41}$,
P.~Ristori$^{2}$,
V.~Rizi$^{53,43}$,
W.~Rodrigues de Carvalho$^{19}$,
J.~Rodriguez Rojo$^{9}$,
M.J.~Roncoroni$^{8}$,
M.~Roth$^{37}$,
E.~Roulet$^{1}$,
A.C.~Rovero$^{5}$,
P.~Ruehl$^{41}$,
S.J.~Saffi$^{12}$,
A.~Saftoiu$^{68}$,
F.~Salamida$^{53,43}$,
H.~Salazar$^{59}$,
G.~Salina$^{48}$,
J.D.~Sanabria Gomez$^{28}$,
F.~S\'anchez$^{8}$,
E.M.~Santos$^{19}$,
E.~Santos$^{30}$,
F.~Sarazin$^{81}$,
R.~Sarmento$^{67}$,
C.~Sarmiento-Cano$^{8}$,
R.~Sato$^{9}$,
P.~Savina$^{52,45,32}$,
C.~Sch\"afer$^{37}$,
V.~Scherini$^{45}$,
H.~Schieler$^{37}$,
M.~Schimassek$^{36,8}$,
M.~Schimp$^{35}$,
F.~Schl\"uter$^{37,8}$,
D.~Schmidt$^{36}$,
O.~Scholten$^{76,14}$,
P.~Schov\'anek$^{30}$,
F.G.~Schr\"oder$^{88,37}$,
S.~Schr\"oder$^{35}$,
S.J.~Sciutto$^{4}$,
M.~Scornavacche$^{8,37}$,
R.C.~Shellard$^{15}$,
G.~Sigl$^{40}$,
G.~Silli$^{8,37}$,
O.~Sima$^{68,h}$,
R.~\v{S}m\'\i{}da$^{87}$,
P.~Sommers$^{86}$,
J.F.~Soriano$^{82}$,
J.~Souchard$^{34}$,
R.~Squartini$^{9}$,
M.~Stadelmaier$^{37,8}$,
D.~Stanca$^{68}$,
S.~Stani\v{c}$^{71}$,
J.~Stasielak$^{64}$,
P.~Stassi$^{34}$,
A.~Streich$^{36,8}$,
M.~Su\'arez-Dur\'an$^{28}$,
T.~Sudholz$^{12}$,
T.~Suomij\"arvi$^{32}$,
A.D.~Supanitsky$^{8}$,
J.~\v{S}up\'\i{}k$^{31}$,
Z.~Szadkowski$^{66}$,
A.~Taboada$^{36}$,
A.~Tapia$^{27}$,
C.~Timmermans$^{77,75}$,
P.~Tobiska$^{30}$,
C.J.~Todero Peixoto$^{17}$,
B.~Tom\'e$^{67}$,
G.~Torralba Elipe$^{74}$,
A.~Travaini$^{9}$,
P.~Travnicek$^{30}$,
C.~Trimarelli$^{53,43}$,
M.~Trini$^{71}$,
M.~Tueros$^{4}$,
R.~Ulrich$^{37}$,
M.~Unger$^{37}$,
M.~Urban$^{39}$,
L.~Vaclavek$^{31}$,
M.~Vacula$^{31}$,
J.F.~Vald\'es Galicia$^{63}$,
I.~Vali\~no$^{42,43}$,
L.~Valore$^{56,47}$,
A.~van Vliet$^{75}$,
E.~Varela$^{59}$,
B.~Vargas C\'ardenas$^{63}$,
A.~V\'asquez-Ram\'\i{}rez$^{28}$,
D.~Veberi\v{c}$^{37}$,
C.~Ventura$^{25}$,
I.D.~Vergara Quispe$^{4}$,
V.~Verzi$^{48}$,
J.~Vicha$^{30}$,
L.~Villase\~nor$^{59}$,
J.~Vink$^{79}$,
S.~Vorobiov$^{71}$,
H.~Wahlberg$^{4}$,
A.A.~Watson$^{a}$,
M.~Weber$^{38}$,
A.~Weindl$^{37}$,
L.~Wiencke$^{81}$,
H.~Wilczy\'nski$^{64}$,
T.~Winchen$^{14}$,
M.~Wirtz$^{39}$,
D.~Wittkowski$^{35}$,
B.~Wundheiler$^{8}$,
A.~Yushkov$^{30}$,
O.~Zapparrata$^{13}$,
E.~Zas$^{74}$,
D.~Zavrtanik$^{71,72}$,
M.~Zavrtanik$^{72,71}$,
L.~Zehrer$^{71}$,
A.~Zepeda$^{60}$,
M.~Ziolkowski$^{41}$,
F.~Zuccarello$^{54,44}$
\\
\llap{$^{1}$} Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina\\
\llap{$^{2}$} Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina\\
\llap{$^{3}$} Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina\\
\llap{$^{4}$} IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina\\
\llap{$^{5}$} Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina\\
\llap{$^{6}$} Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina\\
\llap{$^{7}$} Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina\\
\llap{$^{8}$} Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina\\
\llap{$^{9}$} Observatorio Pierre Auger, Malarg\"ue, Argentina\\
\llap{$^{10}$} Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina\\
\llap{$^{11}$} Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina\\
\llap{$^{12}$} University of Adelaide, Adelaide, S.A., Australia\\
\llap{$^{13}$} Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium\\
\llap{$^{14}$} Vrije Universiteit Brussels, Brussels, Belgium\\
\llap{$^{15}$} Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil\\
\llap{$^{16}$} Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil\\
\llap{$^{17}$} Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil\\
\llap{$^{18}$} Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil\\
\llap{$^{19}$} Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil\\
\llap{$^{20}$} Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil\\
\llap{$^{21}$} Universidade Estadual de Feira de Santana, Feira de Santana, Brazil\\
\llap{$^{22}$} Universidade Federal do ABC, Santo Andr\'e, SP, Brazil\\
\llap{$^{23}$} Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil\\
\llap{$^{24}$} Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil\\
\llap{$^{25}$} Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil\\
\llap{$^{26}$} Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil\\
\llap{$^{27}$} Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia\\
\llap{$^{28}$} Universidad Industrial de Santander, Bucaramanga, Colombia\\
\llap{$^{29}$} Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic\\
\llap{$^{30}$} Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic\\
\llap{$^{31}$} Palacky University, RCPTM, Olomouc, Czech Republic\\
\llap{$^{32}$} Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France\\
\llap{$^{33}$} Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Universit\'es Paris 6 et Paris 7, CNRS-IN2P3, Paris, France\\
\llap{$^{34}$} Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France\\
\llap{$^{35}$} Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany\\
\llap{$^{36}$} Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany\\
\llap{$^{37}$} Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany\\
\llap{$^{38}$} Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany\\
\llap{$^{39}$} RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany\\
\llap{$^{40}$} Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany\\
\llap{$^{41}$} Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany\\
\llap{$^{42}$} Gran Sasso Science Institute, L'Aquila, Italy\\
\llap{$^{43}$} INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy\\
\llap{$^{44}$} INFN, Sezione di Catania, Catania, Italy\\
\llap{$^{45}$} INFN, Sezione di Lecce, Lecce, Italy\\
\llap{$^{46}$} INFN, Sezione di Milano, Milano, Italy\\
\llap{$^{47}$} INFN, Sezione di Napoli, Napoli, Italy\\
\llap{$^{48}$} INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy\\
\llap{$^{49}$} INFN, Sezione di Torino, Torino, Italy\\
\llap{$^{50}$} Osservatorio Astrofisico di Torino (INAF), Torino, Italy\\
\llap{$^{51}$} Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy\\
\llap{$^{52}$} Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy\\
\llap{$^{53}$} Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy\\
\llap{$^{54}$} Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy\\
\llap{$^{55}$} Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy\\
\llap{$^{56}$} Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy\\
\llap{$^{57}$} Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy\\
\llap{$^{58}$} Universit\`a Torino, Dipartimento di Fisica, Torino, Italy\\
\llap{$^{59}$} Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico\\
\llap{$^{60}$} Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico, D.F., M\'exico\\
\llap{$^{61}$} Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico\\
\llap{$^{62}$} Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico\\
\llap{$^{63}$} Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico\\
\llap{$^{64}$} Institute of Nuclear Physics PAN, Krakow, Poland\\
\llap{$^{65}$} University of \L{}\'od\'z, Faculty of Astrophysics, \L{}\'od\'z, Poland\\
\llap{$^{66}$} University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland\\
\llap{$^{67}$} Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal\\
\llap{$^{68}$} ``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
\llap{$^{69}$} Institute of Space Science, Bucharest-Magurele, Romania\\
\llap{$^{70}$} University Politehnica of Bucharest, Bucharest, Romania\\
\llap{$^{71}$} Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia\\
\llap{$^{72}$} Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia\\
\llap{$^{73}$} Universidad de Granada and C.A.F.P.E., Granada, Spain\\
\llap{$^{74}$} Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
\llap{$^{75}$} IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands\\
\llap{$^{76}$} KVI -- Center for Advanced Radiation Technology, University of Groningen, Groningen, The Netherlands\\
\llap{$^{77}$} Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands\\
\llap{$^{78}$} Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands\\
\llap{$^{79}$} Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands\\
\llap{$^{80}$} Case Western Reserve University, Cleveland, OH, USA\\
\llap{$^{81}$} Colorado School of Mines, Golden, CO, USA\\
\llap{$^{82}$} Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA\\
\llap{$^{83}$} Louisiana State University, Baton Rouge, LA, USA\\
\llap{$^{84}$} Michigan Technological University, Houghton, MI, USA\\
\llap{$^{85}$} New York University, New York, NY, USA\\
\llap{$^{86}$} Pennsylvania State University, University Park, PA, USA\\
\llap{$^{87}$} University of Chicago, Enrico Fermi Institute, Chicago, IL, USA\\
\llap{$^{88}$} University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA\\
\llap{$^{a}$} School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom\\
\llap{$^{b}$} Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany\\
\llap{$^{c}$} Fermi National Accelerator Laboratory, USA\\
\llap{$^{d}$} also at Universidade Federal de Alfenas, Po\c{c}os de Caldas, Brazil\\
\llap{$^{e}$} Colorado State University, Fort Collins, CO, USA\\
\llap{$^{f}$} now at Hakubi Center for Advanced Research and Graduate School of Science, Kyoto University, Kyoto, Japan\\
\llap{$^{g}$} also at Karlsruhe Institute of Technology, Karlsruhe, Germany\\
\llap{$^{h}$} also at Radboud Universtiy Nijmegen, Nijmegen, The Netherlands
}


==> 2020-04-author_list-ZIP/latex_authorlist_authors.tex <==
% created on 2020-04-02

A.~Aab$^{75}$,
P.~Abreu$^{67}$,
M.~Aglietta$^{50,49}$,
J.M.~Albury$^{12}$,
I.~Allekotte$^{1}$,
A.~Almela$^{8,11}$,
J.~Alvarez Castillo$^{63}$,
J.~Alvarez-Mu\~niz$^{74}$,
R.~Alves Batista$^{75}$,
G.A.~Anastasi$^{58,49}$,
L.~Anchordoqui$^{82}$,
B.~Andrada$^{8}$,
S.~Andringa$^{67}$,
C.~Aramo$^{47}$,
P.R.~Ara\'ujo Ferreira$^{39}$,
H.~Asorey$^{8}$,
P.~Assis$^{67}$,
G.~Avila$^{9,10}$,
A.M.~Badescu$^{70}$,
A.~Bakalova$^{30}$,
A.~Balaceanu$^{68}$,
F.~Barbato$^{56,47}$,
R.J.~Barreira Luz$^{67}$,
K.H.~Becker$^{35}$,
J.A.~Bellido$^{12}$,
C.~Berat$^{34}$,
M.E.~Bertaina$^{58,49}$,
X.~Bertou$^{1}$,
P.L.~Biermann$^{b}$,
T.~Bister$^{39}$,
J.~Biteau$^{32}$,
A.~Blanco$^{67}$,
J.~Blazek$^{30}$,
C.~Bleve$^{34}$,
M.~Boh\'a\v{c}ov\'a$^{30}$,
D.~Boncioli$^{53,43}$,
C.~Bonifazi$^{24}$,
L.~Bonneau Arbeletche$^{19}$,
N.~Borodai$^{64}$,
A.M.~Botti$^{8}$,
J.~Brack$^{e}$,
T.~Bretz$^{39}$,
F.L.~Briechle$^{39}$,
P.~Buchholz$^{41}$,
A.~Bueno$^{73}$,
S.~Buitink$^{14}$,
M.~Buscemi$^{54,44}$,
K.S.~Caballero-Mora$^{62}$,
L.~Caccianiga$^{55,46}$,
L.~Calcagni$^{4}$,
A.~Cancio$^{11,8}$,
F.~Canfora$^{75,77}$,
I.~Caracas$^{35}$,
J.M.~Carceller$^{73}$,
R.~Caruso$^{54,44}$,
A.~Castellina$^{50,49}$,
F.~Catalani$^{17}$,
G.~Cataldi$^{45}$,
L.~Cazon$^{67}$,
M.~Cerda$^{9}$,
J.A.~Chinellato$^{20}$,
K.~Choi$^{74}$,
J.~Chudoba$^{30}$,
L.~Chytka$^{31}$,
R.W.~Clay$^{12}$,
A.C.~Cobos Cerutti$^{7}$,
R.~Colalillo$^{56,47}$,
A.~Coleman$^{88}$,
M.R.~Coluccia$^{52,45}$,
R.~Concei\c{c}\~ao$^{67}$,
A.~Condorelli$^{42,43}$,
G.~Consolati$^{46,51}$,
F.~Contreras$^{9,10}$,
F.~Convenga$^{52,45}$,
C.E.~Covault$^{80,h}$,
S.~Dasso$^{5,3}$,
K.~Daumiller$^{37}$,
B.R.~Dawson$^{12}$,
J.A.~Day$^{12}$,
R.M.~de Almeida$^{26}$,
J.~de Jes\'us$^{8,37}$,
S.J.~de Jong$^{75,77}$,
G.~De Mauro$^{75,77}$,
J.R.T.~de Mello Neto$^{24,25}$,
I.~De Mitri$^{42,43}$,
J.~de Oliveira$^{26}$,
D.~de Oliveira Franco$^{20}$,
V.~de Souza$^{18}$,
J.~Debatin$^{36}$,
M.~del R\'\i{}o$^{10}$,
O.~Deligny$^{32}$,
N.~Dhital$^{64}$,
A.~Di Matteo$^{49}$,
M.L.~D\'\i{}az Castro$^{20}$,
C.~Dobrigkeit$^{20}$,
J.C.~D'Olivo$^{63}$,
Q.~Dorosti$^{41}$,
R.C.~dos Anjos$^{23}$,
M.T.~Dova$^{4}$,
J.~Ebr$^{30}$,
R.~Engel$^{36,37}$,
I.~Epicoco$^{52,45}$,
M.~Erdmann$^{39}$,
C.O.~Escobar$^{c}$,
A.~Etchegoyen$^{8,11}$,
H.~Falcke$^{75,78,77}$,
J.~Farmer$^{87}$,
G.~Farrar$^{85}$,
A.C.~Fauth$^{20}$,
N.~Fazzini$^{c}$,
F.~Feldbusch$^{38}$,
F.~Fenu$^{58,49}$,
B.~Fick$^{84}$,
J.M.~Figueira$^{8}$,
A.~Filip\v{c}i\v{c}$^{72,71}$,
T.~Fodran$^{75}$,
M.M.~Freire$^{6}$,
T.~Fujii$^{87,f}$,
A.~Fuster$^{8,11}$,
C.~Galea$^{75}$,
C.~Galelli$^{55,46}$,
B.~Garc\'\i{}a$^{7}$,
A.L.~Garcia Vegas$^{39}$,
H.~Gemmeke$^{38}$,
F.~Gesualdi$^{8,37}$,
A.~Gherghel-Lascu$^{68}$,
P.L.~Ghia$^{32}$,
U.~Giaccari$^{75}$,
M.~Giammarchi$^{46}$,
M.~Giller$^{65}$,
J.~Glombitza$^{39}$,
F.~Gobbi$^{9}$,
G.~Golup$^{1}$,
M.~G\'omez Berisso$^{1}$,
P.F.~G\'omez Vitale$^{9,10}$,
J.P.~Gongora$^{9}$,
N.~Gonz\'alez$^{8}$,
I.~Goos$^{1,37}$,
D.~G\'ora$^{64}$,
A.~Gorgi$^{50,49}$,
M.~Gottowik$^{35}$,
T.D.~Grubb$^{12}$,
F.~Guarino$^{56,47}$,
G.P.~Guedes$^{21}$,
E.~Guido$^{49,58}$,
S.~Hahn$^{37,8}$,
R.~Halliday$^{80}$,
M.R.~Hampel$^{8}$,
P.~Hansen$^{4}$,
D.~Harari$^{1}$,
V.M.~Harvey$^{12}$,
A.~Haungs$^{37}$,
T.~Hebbeker$^{39}$,
D.~Heck$^{37}$,
G.C.~Hill$^{12}$,
C.~Hojvat$^{c}$,
J.R.~H\"orandel$^{75,77}$,
P.~Horvath$^{31}$,
M.~Hrabovsk\'y$^{31}$,
T.~Huege$^{37,14}$,
J.~Hulsman$^{8,37}$,
A.~Insolia$^{54,44}$,
P.G.~Isar$^{69}$,
J.A.~Johnsen$^{81}$,
J.~Jurysek$^{30}$,
A.~K\"a\"ap\"a$^{35}$,
K.H.~Kampert$^{35}$,
B.~Keilhauer$^{37}$,
J.~Kemp$^{39}$,
H.O.~Klages$^{37}$,
M.~Kleifges$^{38}$,
J.~Kleinfeller$^{9}$,
M.~K\"opke$^{36}$,
G.~Kukec Mezek$^{71}$,
B.L.~Lago$^{16}$,
D.~LaHurd$^{80}$,
R.G.~Lang$^{18}$,
M.A.~Leigui de Oliveira$^{22}$,
V.~Lenok$^{37}$,
A.~Letessier-Selvon$^{33}$,
I.~Lhenry-Yvon$^{32}$,
D.~Lo Presti$^{54,44}$,
L.~Lopes$^{67}$,
R.~L\'opez$^{59}$,
R.~Lorek$^{80}$,
Q.~Luce$^{36}$,
A.~Lucero$^{8}$,
A.~Machado Payeras$^{20}$,
M.~Malacari$^{87}$,
G.~Mancarella$^{52,45}$,
D.~Mandat$^{30}$,
B.C.~Manning$^{12}$,
J.~Manshanden$^{40}$,
P.~Mantsch$^{c}$,
S.~Marafico$^{32}$,
A.G.~Mariazzi$^{4}$,
I.C.~Mari\c{s}$^{13}$,
G.~Marsella$^{52,45}$,
D.~Martello$^{52,45}$,
H.~Martinez$^{18}$,
O.~Mart\'\i{}nez Bravo$^{59}$,
M.~Mastrodicasa$^{53,43}$,
H.J.~Mathes$^{37}$,
J.~Matthews$^{83}$,
G.~Matthiae$^{57,48}$,
E.~Mayotte$^{35}$,
P.O.~Mazur$^{c}$,
G.~Medina-Tanco$^{63}$,
D.~Melo$^{8}$,
A.~Menshikov$^{38}$,
K.-D.~Merenda$^{81}$,
S.~Michal$^{31}$,
M.I.~Micheletti$^{6}$,
L.~Miramonti$^{55,46}$,
D.~Mockler$^{13}$,
S.~Mollerach$^{1}$,
F.~Montanet$^{34}$,
C.~Morello$^{50,49}$,
M.~Mostaf\'a$^{86}$,
A.L.~M\"uller$^{8,37}$,
M.A.~Muller$^{20,d,24}$,
K.~Mulrey$^{14}$,
R.~Mussa$^{49}$,
M.~Muzio$^{85}$,
W.M.~Namasaka$^{35}$,
L.~Nellen$^{63}$,
M.~Niculescu-Oglinzanu$^{68}$,
M.~Niechciol$^{41}$,
D.~Nitz$^{84,g}$,
D.~Nosek$^{29}$,
V.~Novotny$^{29}$,
L.~No\v{z}ka$^{31}$,
A Nucita$^{52,45}$,
L.A.~N\'u\~nez$^{28}$,
M.~Palatka$^{30}$,
J.~Pallotta$^{2}$,
M.P.~Panetta$^{52,45}$,
P.~Papenbreer$^{35}$,
G.~Parente$^{74}$,
A.~Parra$^{59}$,
M.~Pech$^{30}$,
F.~Pedreira$^{74}$,
J.~P\c{e}kala$^{64}$,
R.~Pelayo$^{61}$,
J.~Pe\~na-Rodriguez$^{28}$,
J.~Perez Armand$^{19}$,
M.~Perlin$^{8,37}$,
L.~Perrone$^{52,45}$,
C.~Peters$^{39}$,
S.~Petrera$^{42,43}$,
T.~Pierog$^{37}$,
M.~Pimenta$^{67}$,
V.~Pirronello$^{54,44}$,
M.~Platino$^{8}$,
B.~Pont$^{75}$,
M.~Pothast$^{77,75}$,
P.~Privitera$^{87}$,
M.~Prouza$^{30}$,
A.~Puyleart$^{84}$,
S.~Querchfeld$^{35}$,
J.~Rautenberg$^{35}$,
D.~Ravignani$^{8}$,
M.~Reininghaus$^{37,8}$,
J.~Ridky$^{30}$,
F.~Riehn$^{67}$,
M.~Risse$^{41}$,
P.~Ristori$^{2}$,
V.~Rizi$^{53,43}$,
W.~Rodrigues de Carvalho$^{19}$,
J.~Rodriguez Rojo$^{9}$,
M.J.~Roncoroni$^{8}$,
M.~Roth$^{37}$,
E.~Roulet$^{1}$,
A.C.~Rovero$^{5}$,
P.~Ruehl$^{41}$,
S.J.~Saffi$^{12}$,
A.~Saftoiu$^{68}$,
F.~Salamida$^{53,43}$,
H.~Salazar$^{59}$,
G.~Salina$^{48}$,
J.D.~Sanabria Gomez$^{28}$,
F.~S\'anchez$^{8}$,
E.M.~Santos$^{19}$,
E.~Santos$^{30}$,
F.~Sarazin$^{81}$,
R.~Sarmento$^{67}$,
C.~Sarmiento-Cano$^{8}$,
R.~Sato$^{9}$,
P.~Savina$^{52,45,32}$,
C.~Sch\"afer$^{37}$,
V.~Scherini$^{45}$,
H.~Schieler$^{37}$,
M.~Schimassek$^{36,8}$,
M.~Schimp$^{35}$,
F.~Schl\"uter$^{37,8}$,
D.~Schmidt$^{36}$,
O.~Scholten$^{76,14}$,
P.~Schov\'anek$^{30}$,
F.G.~Schr\"oder$^{88,37}$,
S.~Schr\"oder$^{35}$,
S.J.~Sciutto$^{4}$,
M.~Scornavacche$^{8,37}$,
R.C.~Shellard$^{15}$,
G.~Sigl$^{40}$,
G.~Silli$^{8,37}$,
O.~Sima$^{68,h}$,
R.~\v{S}m\'\i{}da$^{87}$,
P.~Sommers$^{86}$,
J.F.~Soriano$^{82}$,
J.~Souchard$^{34}$,
R.~Squartini$^{9}$,
M.~Stadelmaier$^{37,8}$,
D.~Stanca$^{68}$,
S.~Stani\v{c}$^{71}$,
J.~Stasielak$^{64}$,
P.~Stassi$^{34}$,
A.~Streich$^{36,8}$,
M.~Su\'arez-Dur\'an$^{28}$,
T.~Sudholz$^{12}$,
T.~Suomij\"arvi$^{32}$,
A.D.~Supanitsky$^{8}$,
J.~\v{S}up\'\i{}k$^{31}$,
Z.~Szadkowski$^{66}$,
A.~Taboada$^{36}$,
A.~Tapia$^{27}$,
C.~Timmermans$^{77,75}$,
P.~Tobiska$^{30}$,
C.J.~Todero Peixoto$^{17}$,
B.~Tom\'e$^{67}$,
G.~Torralba Elipe$^{74}$,
A.~Travaini$^{9}$,
P.~Travnicek$^{30}$,
C.~Trimarelli$^{53,43}$,
M.~Trini$^{71}$,
M.~Tueros$^{4}$,
R.~Ulrich$^{37}$,
M.~Unger$^{37}$,
M.~Urban$^{39}$,
L.~Vaclavek$^{31}$,
M.~Vacula$^{31}$,
J.F.~Vald\'es Galicia$^{63}$,
I.~Vali\~no$^{42,43}$,
L.~Valore$^{56,47}$,
A.~van Vliet$^{75}$,
E.~Varela$^{59}$,
B.~Vargas C\'ardenas$^{63}$,
A.~V\'asquez-Ram\'\i{}rez$^{28}$,
D.~Veberi\v{c}$^{37}$,
C.~Ventura$^{25}$,
I.D.~Vergara Quispe$^{4}$,
V.~Verzi$^{48}$,
J.~Vicha$^{30}$,
L.~Villase\~nor$^{59}$,
J.~Vink$^{79}$,
S.~Vorobiov$^{71}$,
H.~Wahlberg$^{4}$,
A.A.~Watson$^{a}$,
M.~Weber$^{38}$,
A.~Weindl$^{37}$,
L.~Wiencke$^{81}$,
H.~Wilczy\'nski$^{64}$,
T.~Winchen$^{14}$,
M.~Wirtz$^{39}$,
D.~Wittkowski$^{35}$,
B.~Wundheiler$^{8}$,
A.~Yushkov$^{30}$,
O.~Zapparrata$^{13}$,
E.~Zas$^{74}$,
D.~Zavrtanik$^{71,72}$,
M.~Zavrtanik$^{72,71}$,
L.~Zehrer$^{71}$,
A.~Zepeda$^{60}$,
M.~Ziolkowski$^{41}$,
F.~Zuccarello$^{54,44}$


==> 2020-04-author_list-ZIP/latex_authorlist_institutions.tex <==
% created on 2020-04-02

% needs \usepackage{enumitem}
\begin{description}[labelsep=0.2em,align=right,labelwidth=0.7em,labelindent=0em,leftmargin=2em,noitemsep]
\item[$^{1}$] Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina
\item[$^{2}$] Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina
\item[$^{3}$] Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina
\item[$^{4}$] IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina
\item[$^{5}$] Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina
\item[$^{6}$] Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina
\item[$^{7}$] Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina
\item[$^{8}$] Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina
\item[$^{9}$] Observatorio Pierre Auger, Malarg\"ue, Argentina
\item[$^{10}$] Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina
\item[$^{11}$] Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina
\item[$^{12}$] University of Adelaide, Adelaide, S.A., Australia
\item[$^{13}$] Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium
\item[$^{14}$] Vrije Universiteit Brussels, Brussels, Belgium
\item[$^{15}$] Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil
\item[$^{16}$] Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil
\item[$^{17}$] Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil
\item[$^{18}$] Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil
\item[$^{19}$] Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil
\item[$^{20}$] Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil
\item[$^{21}$] Universidade Estadual de Feira de Santana, Feira de Santana, Brazil
\item[$^{22}$] Universidade Federal do ABC, Santo Andr\'e, SP, Brazil
\item[$^{23}$] Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil
\item[$^{24}$] Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil
\item[$^{25}$] Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil
\item[$^{26}$] Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil
\item[$^{27}$] Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia
\item[$^{28}$] Universidad Industrial de Santander, Bucaramanga, Colombia
\item[$^{29}$] Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic
\item[$^{30}$] Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic
\item[$^{31}$] Palacky University, RCPTM, Olomouc, Czech Republic
\item[$^{32}$] Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France
\item[$^{33}$] Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Universit\'es Paris 6 et Paris 7, CNRS-IN2P3, Paris, France
\item[$^{34}$] Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France
\item[$^{35}$] Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany
\item[$^{36}$] Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany
\item[$^{37}$] Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany
\item[$^{38}$] Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany
\item[$^{39}$] RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany
\item[$^{40}$] Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany
\item[$^{41}$] Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany
\item[$^{42}$] Gran Sasso Science Institute, L'Aquila, Italy
\item[$^{43}$] INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy
\item[$^{44}$] INFN, Sezione di Catania, Catania, Italy
\item[$^{45}$] INFN, Sezione di Lecce, Lecce, Italy
\item[$^{46}$] INFN, Sezione di Milano, Milano, Italy
\item[$^{47}$] INFN, Sezione di Napoli, Napoli, Italy
\item[$^{48}$] INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy
\item[$^{49}$] INFN, Sezione di Torino, Torino, Italy
\item[$^{50}$] Osservatorio Astrofisico di Torino (INAF), Torino, Italy
\item[$^{51}$] Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy
\item[$^{52}$] Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy
\item[$^{53}$] Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy
\item[$^{54}$] Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy
\item[$^{55}$] Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy
\item[$^{56}$] Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy
\item[$^{57}$] Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy
\item[$^{58}$] Universit\`a Torino, Dipartimento di Fisica, Torino, Italy
\item[$^{59}$] Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico
\item[$^{60}$] Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico, D.F., M\'exico
\item[$^{61}$] Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico
\item[$^{62}$] Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico
\item[$^{63}$] Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico
\item[$^{64}$] Institute of Nuclear Physics PAN, Krakow, Poland
\item[$^{65}$] University of \L{}\'od\'z, Faculty of Astrophysics, \L{}\'od\'z, Poland
\item[$^{66}$] University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland
\item[$^{67}$] Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal
\item[$^{68}$] ``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania
\item[$^{69}$] Institute of Space Science, Bucharest-Magurele, Romania
\item[$^{70}$] University Politehnica of Bucharest, Bucharest, Romania
\item[$^{71}$] Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia
\item[$^{72}$] Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia
\item[$^{73}$] Universidad de Granada and C.A.F.P.E., Granada, Spain
\item[$^{74}$] Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain
\item[$^{75}$] IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands
\item[$^{76}$] KVI -- Center for Advanced Radiation Technology, University of Groningen, Groningen, The Netherlands
\item[$^{77}$] Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands
\item[$^{78}$] Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands
\item[$^{79}$] Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands
\item[$^{80}$] Case Western Reserve University, Cleveland, OH, USA
\item[$^{81}$] Colorado School of Mines, Golden, CO, USA
\item[$^{82}$] Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA
\item[$^{83}$] Louisiana State University, Baton Rouge, LA, USA
\item[$^{84}$] Michigan Technological University, Houghton, MI, USA
\item[$^{85}$] New York University, New York, NY, USA
\item[$^{86}$] Pennsylvania State University, University Park, PA, USA
\item[$^{87}$] University of Chicago, Enrico Fermi Institute, Chicago, IL, USA
\item[$^{88}$] University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA
\item[] -----
\item[$^{a}$] School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom
\item[$^{b}$] Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany
\item[$^{c}$] Fermi National Accelerator Laboratory, USA
\item[$^{d}$] also at Universidade Federal de Alfenas, Po\c{c}os de Caldas, Brazil
\item[$^{e}$] Colorado State University, Fort Collins, CO, USA
\item[$^{f}$] now at Hakubi Center for Advanced Research and Graduate School of Science, Kyoto University, Kyoto, Japan
\item[$^{g}$] also at Karlsruhe Institute of Technology, Karlsruhe, Germany
\item[$^{h}$] also at Radboud Universtiy Nijmegen, Nijmegen, The Netherlands
\end{description}


==> 2020-04-author_list-ZIP/revtex_authorlist.tex <==
% created on 2020-04-02

\author{A.~Aab}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{P.~Abreu}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{M.~Aglietta}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{J.M.~Albury}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{I.~Allekotte}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{A.~Almela}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}

\author{J.~Alvarez Castillo}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{J.~Alvarez-Mu\~niz}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{R.~Alves Batista}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{G.A.~Anastasi}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{L.~Anchordoqui}
\affiliation{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}

\author{B.~Andrada}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{S.~Andringa}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{C.~Aramo}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{P.R.~Ara\'ujo Ferreira}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{H.~Asorey}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{P.~Assis}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{G.~Avila}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{A.M.~Badescu}
\affiliation{University Politehnica of Bucharest, Bucharest, Romania}

\author{A.~Bakalova}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{A.~Balaceanu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{F.~Barbato}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{R.J.~Barreira Luz}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{K.H.~Becker}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{J.A.~Bellido}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{C.~Berat}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}

\author{M.E.~Bertaina}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{X.~Bertou}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{P.L.~Biermann}
\affiliation{Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany}

\author{T.~Bister}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{J.~Biteau}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}

\author{A.~Blanco}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{J.~Blazek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{C.~Bleve}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}

\author{M.~Boh\'a\v{c}ov\'a}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{D.~Boncioli}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{C.~Bonifazi}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}

\author{L.~Bonneau Arbeletche}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}

\author{N.~Borodai}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{A.M.~Botti}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{J.~Brack}
\affiliation{Colorado State University, Fort Collins, CO, USA}

\author{T.~Bretz}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{F.L.~Briechle}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{P.~Buchholz}
\affiliation{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{A.~Bueno}
\affiliation{Universidad de Granada and C.A.F.P.E., Granada, Spain}

\author{S.~Buitink}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{M.~Buscemi}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{K.S.~Caballero-Mora}
\affiliation{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}

\author{L.~Caccianiga}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{L.~Calcagni}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{A.~Cancio}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{F.~Canfora}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{I.~Caracas}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{J.M.~Carceller}
\affiliation{Universidad de Granada and C.A.F.P.E., Granada, Spain}

\author{R.~Caruso}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{A.~Castellina}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{F.~Catalani}
\affiliation{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}

\author{G.~Cataldi}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{L.~Cazon}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{M.~Cerda}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{J.A.~Chinellato}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{K.~Choi}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{J.~Chudoba}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{L.~Chytka}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{R.W.~Clay}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{A.C.~Cobos Cerutti}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}

\author{R.~Colalillo}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{A.~Coleman}
\affiliation{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}

\author{M.R.~Coluccia}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{R.~Concei\c{c}\~ao}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{A.~Condorelli}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{G.~Consolati}
\affiliation{INFN, Sezione di Milano, Milano, Italy}
\affiliation{Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy}

\author{F.~Contreras}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{F.~Convenga}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{C.E.~Covault}
\affiliation{Case Western Reserve University, Cleveland, OH, USA}
\affiliation{also at Radboud Universtiy Nijmegen, Nijmegen, The Netherlands}

\author{S.~Dasso}
\affiliation{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}
\affiliation{Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina}

\author{K.~Daumiller}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{B.R.~Dawson}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{J.A.~Day}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{R.M.~de Almeida}
\affiliation{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}

\author{J.~de Jes\'us}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{S.J.~de Jong}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{G.~De Mauro}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{J.R.T.~de Mello Neto}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}
\affiliation{Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil}

\author{I.~De Mitri}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{J.~de Oliveira}
\affiliation{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}

\author{D.~de Oliveira Franco}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{V.~de Souza}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}

\author{J.~Debatin}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}

\author{M.~del R\'\i{}o}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{O.~Deligny}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}

\author{N.~Dhital}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{A.~Di Matteo}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{M.L.~D\'\i{}az Castro}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{C.~Dobrigkeit}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{J.C.~D'Olivo}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{Q.~Dorosti}
\affiliation{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{R.C.~dos Anjos}
\affiliation{Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil}

\author{M.T.~Dova}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{J.~Ebr}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{R.~Engel}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{I.~Epicoco}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{M.~Erdmann}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{C.O.~Escobar}
\affiliation{Fermi National Accelerator Laboratory, USA}

\author{A.~Etchegoyen}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}

\author{H.~Falcke}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{J.~Farmer}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{G.~Farrar}
\affiliation{New York University, New York, NY, USA}

\author{A.C.~Fauth}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{N.~Fazzini}
\affiliation{Fermi National Accelerator Laboratory, USA}

\author{F.~Feldbusch}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{F.~Fenu}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{B.~Fick}
\affiliation{Michigan Technological University, Houghton, MI, USA}

\author{J.M.~Figueira}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Filip\v{c}i\v{c}}
\affiliation{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{T.~Fodran}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{M.M.~Freire}
\affiliation{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}

\author{T.~Fujii}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}
\affiliation{now at Hakubi Center for Advanced Research and Graduate School of Science, Kyoto University, Kyoto, Japan}

\author{A.~Fuster}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}

\author{C.~Galea}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{C.~Galelli}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{B.~Garc\'\i{}a}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}

\author{A.L.~Garcia Vegas}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{H.~Gemmeke}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{F.~Gesualdi}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{A.~Gherghel-Lascu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{P.L.~Ghia}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}

\author{U.~Giaccari}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{M.~Giammarchi}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{M.~Giller}
\affiliation{University of \L{}\'od\'z, Faculty of Astrophysics, \L{}\'od\'z, Poland}

\author{J.~Glombitza}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{F.~Gobbi}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{G.~Golup}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{M.~G\'omez Berisso}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{P.F.~G\'omez Vitale}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{J.P.~Gongora}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{N.~Gonz\'alez}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{I.~Goos}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{D.~G\'ora}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{A.~Gorgi}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{M.~Gottowik}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{T.D.~Grubb}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{F.~Guarino}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{G.P.~Guedes}
\affiliation{Universidade Estadual de Feira de Santana, Feira de Santana, Brazil}

\author{E.~Guido}
\affiliation{INFN, Sezione di Torino, Torino, Italy}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}

\author{S.~Hahn}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{R.~Halliday}
\affiliation{Case Western Reserve University, Cleveland, OH, USA}

\author{M.R.~Hampel}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{P.~Hansen}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{D.~Harari}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{V.M.~Harvey}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{A.~Haungs}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{T.~Hebbeker}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{D.~Heck}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{G.C.~Hill}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{C.~Hojvat}
\affiliation{Fermi National Accelerator Laboratory, USA}

\author{J.R.~H\"orandel}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{P.~Horvath}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{M.~Hrabovsk\'y}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{T.~Huege}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{J.~Hulsman}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{A.~Insolia}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{P.G.~Isar}
\affiliation{Institute of Space Science, Bucharest-Magurele, Romania}

\author{J.A.~Johnsen}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{J.~Jurysek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{A.~K\"a\"ap\"a}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{K.H.~Kampert}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{B.~Keilhauer}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{J.~Kemp}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{H.O.~Klages}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{M.~Kleifges}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{J.~Kleinfeller}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{M.~K\"opke}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}

\author{G.~Kukec Mezek}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{B.L.~Lago}
\affiliation{Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil}

\author{D.~LaHurd}
\affiliation{Case Western Reserve University, Cleveland, OH, USA}

\author{R.G.~Lang}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}

\author{M.A.~Leigui de Oliveira}
\affiliation{Universidade Federal do ABC, Santo Andr\'e, SP, Brazil}

\author{V.~Lenok}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{A.~Letessier-Selvon}
\affiliation{Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Universit\'es Paris 6 et Paris 7, CNRS-IN2P3, Paris, France}

\author{I.~Lhenry-Yvon}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}

\author{D.~Lo Presti}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{L.~Lopes}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{R.~L\'opez}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{R.~Lorek}
\affiliation{Case Western Reserve University, Cleveland, OH, USA}

\author{Q.~Luce}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}

\author{A.~Lucero}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Machado Payeras}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{M.~Malacari}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{G.~Mancarella}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{D.~Mandat}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{B.C.~Manning}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{J.~Manshanden}
\affiliation{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}

\author{P.~Mantsch}
\affiliation{Fermi National Accelerator Laboratory, USA}

\author{S.~Marafico}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}

\author{A.G.~Mariazzi}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{I.C.~Mari\c{s}}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{G.~Marsella}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{D.~Martello}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{H.~Martinez}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}

\author{O.~Mart\'\i{}nez Bravo}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{M.~Mastrodicasa}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{H.J.~Mathes}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{J.~Matthews}
\affiliation{Louisiana State University, Baton Rouge, LA, USA}

\author{G.~Matthiae}
\affiliation{Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy}
\affiliation{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}

\author{E.~Mayotte}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{P.O.~Mazur}
\affiliation{Fermi National Accelerator Laboratory, USA}

\author{G.~Medina-Tanco}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{D.~Melo}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Menshikov}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{K.-D.~Merenda}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{S.~Michal}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{M.I.~Micheletti}
\affiliation{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}

\author{L.~Miramonti}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{D.~Mockler}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{S.~Mollerach}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{F.~Montanet}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}

\author{C.~Morello}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{M.~Mostaf\'a}
\affiliation{Pennsylvania State University, University Park, PA, USA}

\author{A.L.~M\"uller}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{M.A.~Muller}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}
\affiliation{also at Universidade Federal de Alfenas, Po\c{c}os de Caldas, Brazil}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}

\author{K.~Mulrey}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{R.~Mussa}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{M.~Muzio}
\affiliation{New York University, New York, NY, USA}

\author{W.M.~Namasaka}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{L.~Nellen}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{M.~Niculescu-Oglinzanu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{M.~Niechciol}
\affiliation{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{D.~Nitz}
\affiliation{Michigan Technological University, Houghton, MI, USA}
\affiliation{also at Karlsruhe Institute of Technology, Karlsruhe, Germany}

\author{D.~Nosek}
\affiliation{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}

\author{V.~Novotny}
\affiliation{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}

\author{L.~No\v{z}ka}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{A Nucita}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{L.A.~N\'u\~nez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{M.~Palatka}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{J.~Pallotta}
\affiliation{Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina}

\author{M.P.~Panetta}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{P.~Papenbreer}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{G.~Parente}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{A.~Parra}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{M.~Pech}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.~Pedreira}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{J.~P\c{e}kala}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{R.~Pelayo}
\affiliation{Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico}

\author{J.~Pe\~na-Rodriguez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{J.~Perez Armand}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}

\author{M.~Perlin}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{L.~Perrone}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{C.~Peters}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{S.~Petrera}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{T.~Pierog}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{M.~Pimenta}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{V.~Pirronello}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{M.~Platino}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{B.~Pont}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{M.~Pothast}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{P.~Privitera}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{M.~Prouza}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{A.~Puyleart}
\affiliation{Michigan Technological University, Houghton, MI, USA}

\author{S.~Querchfeld}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{J.~Rautenberg}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{D.~Ravignani}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{M.~Reininghaus}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{J.~Ridky}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.~Riehn}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{M.~Risse}
\affiliation{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{P.~Ristori}
\affiliation{Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina}

\author{V.~Rizi}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{W.~Rodrigues de Carvalho}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}

\author{J.~Rodriguez Rojo}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{M.J.~Roncoroni}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{M.~Roth}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{E.~Roulet}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{A.C.~Rovero}
\affiliation{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}

\author{P.~Ruehl}
\affiliation{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{S.J.~Saffi}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{A.~Saftoiu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{F.~Salamida}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{H.~Salazar}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{G.~Salina}
\affiliation{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}

\author{J.D.~Sanabria Gomez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{F.~S\'anchez}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{E.M.~Santos}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}

\author{E.~Santos}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.~Sarazin}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{R.~Sarmento}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{C.~Sarmiento-Cano}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{R.~Sato}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{P.~Savina}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}

\author{C.~Sch\"afer}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{V.~Scherini}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{H.~Schieler}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{M.~Schimassek}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{M.~Schimp}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{F.~Schl\"uter}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{D.~Schmidt}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}

\author{O.~Scholten}
\affiliation{KVI -- Center for Advanced Radiation Technology, University of Groningen, Groningen, The Netherlands}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{P.~Schov\'anek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.G.~Schr\"oder}
\affiliation{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{S.~Schr\"oder}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{S.J.~Sciutto}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{M.~Scornavacche}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{R.C.~Shellard}
\affiliation{Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil}

\author{G.~Sigl}
\affiliation{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}

\author{G.~Silli}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{O.~Sima}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}
\affiliation{also at Radboud Universtiy Nijmegen, Nijmegen, The Netherlands}

\author{R.~\v{S}m\'\i{}da}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{P.~Sommers}
\affiliation{Pennsylvania State University, University Park, PA, USA}

\author{J.F.~Soriano}
\affiliation{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}

\author{J.~Souchard}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}

\author{R.~Squartini}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{M.~Stadelmaier}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{D.~Stanca}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{S.~Stani\v{c}}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{J.~Stasielak}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{P.~Stassi}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}

\author{A.~Streich}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{M.~Su\'arez-Dur\'an}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{T.~Sudholz}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{T.~Suomij\"arvi}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}

\author{A.D.~Supanitsky}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{J.~\v{S}up\'\i{}k}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{Z.~Szadkowski}
\affiliation{University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland}

\author{A.~Taboada}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}

\author{A.~Tapia}
\affiliation{Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia}

\author{C.~Timmermans}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{P.~Tobiska}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{C.J.~Todero Peixoto}
\affiliation{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}

\author{B.~Tom\'e}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{G.~Torralba Elipe}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{A.~Travaini}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{P.~Travnicek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{C.~Trimarelli}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{M.~Trini}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{M.~Tueros}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{R.~Ulrich}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{M.~Unger}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{M.~Urban}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{L.~Vaclavek}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{M.~Vacula}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{J.F.~Vald\'es Galicia}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{I.~Vali\~no}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{L.~Valore}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{A.~van Vliet}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{E.~Varela}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{B.~Vargas C\'ardenas}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{A.~V\'asquez-Ram\'\i{}rez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{D.~Veberi\v{c}}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{C.~Ventura}
\affiliation{Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil}

\author{I.D.~Vergara Quispe}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{V.~Verzi}
\affiliation{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}

\author{J.~Vicha}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{L.~Villase\~nor}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{J.~Vink}
\affiliation{Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands}

\author{S.~Vorobiov}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{H.~Wahlberg}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{A.A.~Watson}
\affiliation{School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom}

\author{M.~Weber}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{A.~Weindl}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{L.~Wiencke}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{H.~Wilczy\'nski}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{T.~Winchen}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{M.~Wirtz}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{D.~Wittkowski}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{B.~Wundheiler}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Yushkov}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{O.~Zapparrata}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{E.~Zas}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{D.~Zavrtanik}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}
\affiliation{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}

\author{M.~Zavrtanik}
\affiliation{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{L.~Zehrer}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{A.~Zepeda}
\affiliation{Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico, D.F., M\'exico}

\author{M.~Ziolkowski}
\affiliation{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{F.~Zuccarello}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\collaboration{The Pierre Auger Collaboration}
\email{auger_spokespersons@fnal.gov}
\homepage{http://www.auger.org}
\noaffiliation



==> 2020-04-author_list-ZIP/templates/aastex/Makefile <==
# Makefile for building latex documents (c) Darko Veberic
# $Id: Makefile 10301 2017-02-02 17:33:43Z darko $

USEPDFLATEX := 1
USEBIBTEX := 1

TEXFILES := $(shell grep -le '^\s*\\document\(class\|style\)' *.tex)
TARGETS := $(basename $(TEXFILES))
DEPENDENCIES := $(wildcard figs/* *.bib) $(filter-out $(TEXFILES), $(wildcard *.tex))

##########################################################
SHELL := bash
PDFS := $(addsuffix .pdf,$(TARGETS))
DEPENDENCIES += $(wildcard *.sty *.bib)

LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)

# 30=black 31=red 32=green 33=yellow 34=blue 35=magenta 36=cyan 37=white 0=cancel
COLORIZE := awk 'BEGIN{ec="\033[31;1m";wc="\033[34;1m";cc="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print ec""$$0""cc;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print wc""$$0""cc;next}{print}END{if(w||e)print "\n"ec"Warning/error summary:"cc"\n"wc""w""cc;if(e){print ec""e""cc;exit 1}}'

define basic_latex_rule
  for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && break ; done
endef

ifeq ($(USEBIBTEX), 1)
define latex_rule
  $(LATEX) $< ; bibtex $*
  $(call basic_latex_rule)
endef
else
define latex_rule
  $(call basic_latex_rule)
endef
endif

.PHONY: all clean

all: $(PDFS)

# dependencies
$(PDFS): $(DEPENDENCIES)

clean:
	- $(RM) *{.tex~,.dvi,.log,.aux,.toc,.nav,.out,.snm,.bbl,.blg,.spl,.lof,Notes.bib,.maf,.fff,.lot,.ttt}
	- for f in $(TARGETS) ; do $(RM) $$f{.ps,.pdf} ; done

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.dvi
	dvipdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<


==> 2020-04-author_list-ZIP/templates/aastex/aastex_authorlist.tex <==
% created on 2020-04-02

\author{
A.~Aab\altaffilmark{75},
P.~Abreu\altaffilmark{67},
M.~Aglietta\altaffilmark{50,49},
J.M.~Albury\altaffilmark{12},
I.~Allekotte\altaffilmark{1},
A.~Almela\altaffilmark{8,11},
J.~Alvarez Castillo\altaffilmark{63},
J.~Alvarez-Mu\~niz\altaffilmark{74},
R.~Alves Batista\altaffilmark{75},
G.A.~Anastasi\altaffilmark{58,49},
L.~Anchordoqui\altaffilmark{82},
B.~Andrada\altaffilmark{8},
S.~Andringa\altaffilmark{67},
C.~Aramo\altaffilmark{47},
P.R.~Ara\'ujo Ferreira\altaffilmark{39},
H.~Asorey\altaffilmark{8},
P.~Assis\altaffilmark{67},
G.~Avila\altaffilmark{9,10},
A.M.~Badescu\altaffilmark{70},
A.~Bakalova\altaffilmark{30},
A.~Balaceanu\altaffilmark{68},
F.~Barbato\altaffilmark{56,47},
R.J.~Barreira Luz\altaffilmark{67},
K.H.~Becker\altaffilmark{35},
J.A.~Bellido\altaffilmark{12},
C.~Berat\altaffilmark{34},
M.E.~Bertaina\altaffilmark{58,49},
X.~Bertou\altaffilmark{1},
P.L.~Biermann\altaffilmark{1001},
T.~Bister\altaffilmark{39},
J.~Biteau\altaffilmark{32},
A.~Blanco\altaffilmark{67},
J.~Blazek\altaffilmark{30},
C.~Bleve\altaffilmark{34},
M.~Boh\'a\v{c}ov\'a\altaffilmark{30},
D.~Boncioli\altaffilmark{53,43},
C.~Bonifazi\altaffilmark{24},
L.~Bonneau Arbeletche\altaffilmark{19},
N.~Borodai\altaffilmark{64},
A.M.~Botti\altaffilmark{8},
J.~Brack\altaffilmark{1004},
T.~Bretz\altaffilmark{39},
F.L.~Briechle\altaffilmark{39},
P.~Buchholz\altaffilmark{41},
A.~Bueno\altaffilmark{73},
S.~Buitink\altaffilmark{14},
M.~Buscemi\altaffilmark{54,44},
K.S.~Caballero-Mora\altaffilmark{62},
L.~Caccianiga\altaffilmark{55,46},
L.~Calcagni\altaffilmark{4},
A.~Cancio\altaffilmark{11,8},
F.~Canfora\altaffilmark{75,77},
I.~Caracas\altaffilmark{35},
J.M.~Carceller\altaffilmark{73},
R.~Caruso\altaffilmark{54,44},
A.~Castellina\altaffilmark{50,49},
F.~Catalani\altaffilmark{17},
G.~Cataldi\altaffilmark{45},
L.~Cazon\altaffilmark{67},
M.~Cerda\altaffilmark{9},
J.A.~Chinellato\altaffilmark{20},
K.~Choi\altaffilmark{74},
J.~Chudoba\altaffilmark{30},
L.~Chytka\altaffilmark{31},
R.W.~Clay\altaffilmark{12},
A.C.~Cobos Cerutti\altaffilmark{7},
R.~Colalillo\altaffilmark{56,47},
A.~Coleman\altaffilmark{88},
M.R.~Coluccia\altaffilmark{52,45},
R.~Concei\c{c}\~ao\altaffilmark{67},
A.~Condorelli\altaffilmark{42,43},
G.~Consolati\altaffilmark{46,51},
F.~Contreras\altaffilmark{9,10},
F.~Convenga\altaffilmark{52,45},
C.E.~Covault\altaffilmark{80,1007},
S.~Dasso\altaffilmark{5,3},
K.~Daumiller\altaffilmark{37},
B.R.~Dawson\altaffilmark{12},
J.A.~Day\altaffilmark{12},
R.M.~de Almeida\altaffilmark{26},
J.~de Jes\'us\altaffilmark{8,37},
S.J.~de Jong\altaffilmark{75,77},
G.~De Mauro\altaffilmark{75,77},
J.R.T.~de Mello Neto\altaffilmark{24,25},
I.~De Mitri\altaffilmark{42,43},
J.~de Oliveira\altaffilmark{26},
D.~de Oliveira Franco\altaffilmark{20},
V.~de Souza\altaffilmark{18},
J.~Debatin\altaffilmark{36},
M.~del R\'\i{}o\altaffilmark{10},
O.~Deligny\altaffilmark{32},
N.~Dhital\altaffilmark{64},
A.~Di Matteo\altaffilmark{49},
M.L.~D\'\i{}az Castro\altaffilmark{20},
C.~Dobrigkeit\altaffilmark{20},
J.C.~D'Olivo\altaffilmark{63},
Q.~Dorosti\altaffilmark{41},
R.C.~dos Anjos\altaffilmark{23},
M.T.~Dova\altaffilmark{4},
J.~Ebr\altaffilmark{30},
R.~Engel\altaffilmark{36,37},
I.~Epicoco\altaffilmark{52,45},
M.~Erdmann\altaffilmark{39},
C.O.~Escobar\altaffilmark{1002},
A.~Etchegoyen\altaffilmark{8,11},
H.~Falcke\altaffilmark{75,78,77},
J.~Farmer\altaffilmark{87},
G.~Farrar\altaffilmark{85},
A.C.~Fauth\altaffilmark{20},
N.~Fazzini\altaffilmark{1002},
F.~Feldbusch\altaffilmark{38},
F.~Fenu\altaffilmark{58,49},
B.~Fick\altaffilmark{84},
J.M.~Figueira\altaffilmark{8},
A.~Filip\v{c}i\v{c}\altaffilmark{72,71},
T.~Fodran\altaffilmark{75},
M.M.~Freire\altaffilmark{6},
T.~Fujii\altaffilmark{87,1005},
A.~Fuster\altaffilmark{8,11},
C.~Galea\altaffilmark{75},
C.~Galelli\altaffilmark{55,46},
B.~Garc\'\i{}a\altaffilmark{7},
A.L.~Garcia Vegas\altaffilmark{39},
H.~Gemmeke\altaffilmark{38},
F.~Gesualdi\altaffilmark{8,37},
A.~Gherghel-Lascu\altaffilmark{68},
P.L.~Ghia\altaffilmark{32},
U.~Giaccari\altaffilmark{75},
M.~Giammarchi\altaffilmark{46},
M.~Giller\altaffilmark{65},
J.~Glombitza\altaffilmark{39},
F.~Gobbi\altaffilmark{9},
G.~Golup\altaffilmark{1},
M.~G\'omez Berisso\altaffilmark{1},
P.F.~G\'omez Vitale\altaffilmark{9,10},
J.P.~Gongora\altaffilmark{9},
N.~Gonz\'alez\altaffilmark{8},
I.~Goos\altaffilmark{1,37},
D.~G\'ora\altaffilmark{64},
A.~Gorgi\altaffilmark{50,49},
M.~Gottowik\altaffilmark{35},
T.D.~Grubb\altaffilmark{12},
F.~Guarino\altaffilmark{56,47},
G.P.~Guedes\altaffilmark{21},
E.~Guido\altaffilmark{49,58},
S.~Hahn\altaffilmark{37,8},
R.~Halliday\altaffilmark{80},
M.R.~Hampel\altaffilmark{8},
P.~Hansen\altaffilmark{4},
D.~Harari\altaffilmark{1},
V.M.~Harvey\altaffilmark{12},
A.~Haungs\altaffilmark{37},
T.~Hebbeker\altaffilmark{39},
D.~Heck\altaffilmark{37},
G.C.~Hill\altaffilmark{12},
C.~Hojvat\altaffilmark{1002},
J.R.~H\"orandel\altaffilmark{75,77},
P.~Horvath\altaffilmark{31},
M.~Hrabovsk\'y\altaffilmark{31},
T.~Huege\altaffilmark{37,14},
J.~Hulsman\altaffilmark{8,37},
A.~Insolia\altaffilmark{54,44},
P.G.~Isar\altaffilmark{69},
J.A.~Johnsen\altaffilmark{81},
J.~Jurysek\altaffilmark{30},
A.~K\"a\"ap\"a\altaffilmark{35},
K.H.~Kampert\altaffilmark{35},
B.~Keilhauer\altaffilmark{37},
J.~Kemp\altaffilmark{39},
H.O.~Klages\altaffilmark{37},
M.~Kleifges\altaffilmark{38},
J.~Kleinfeller\altaffilmark{9},
M.~K\"opke\altaffilmark{36},
G.~Kukec Mezek\altaffilmark{71},
B.L.~Lago\altaffilmark{16},
D.~LaHurd\altaffilmark{80},
R.G.~Lang\altaffilmark{18},
M.A.~Leigui de Oliveira\altaffilmark{22},
V.~Lenok\altaffilmark{37},
A.~Letessier-Selvon\altaffilmark{33},
I.~Lhenry-Yvon\altaffilmark{32},
D.~Lo Presti\altaffilmark{54,44},
L.~Lopes\altaffilmark{67},
R.~L\'opez\altaffilmark{59},
R.~Lorek\altaffilmark{80},
Q.~Luce\altaffilmark{36},
A.~Lucero\altaffilmark{8},
A.~Machado Payeras\altaffilmark{20},
M.~Malacari\altaffilmark{87},
G.~Mancarella\altaffilmark{52,45},
D.~Mandat\altaffilmark{30},
B.C.~Manning\altaffilmark{12},
J.~Manshanden\altaffilmark{40},
P.~Mantsch\altaffilmark{1002},
S.~Marafico\altaffilmark{32},
A.G.~Mariazzi\altaffilmark{4},
I.C.~Mari\c{s}\altaffilmark{13},
G.~Marsella\altaffilmark{52,45},
D.~Martello\altaffilmark{52,45},
H.~Martinez\altaffilmark{18},
O.~Mart\'\i{}nez Bravo\altaffilmark{59},
M.~Mastrodicasa\altaffilmark{53,43},
H.J.~Mathes\altaffilmark{37},
J.~Matthews\altaffilmark{83},
G.~Matthiae\altaffilmark{57,48},
E.~Mayotte\altaffilmark{35},
P.O.~Mazur\altaffilmark{1002},
G.~Medina-Tanco\altaffilmark{63},
D.~Melo\altaffilmark{8},
A.~Menshikov\altaffilmark{38},
K.-D.~Merenda\altaffilmark{81},
S.~Michal\altaffilmark{31},
M.I.~Micheletti\altaffilmark{6},
L.~Miramonti\altaffilmark{55,46},
D.~Mockler\altaffilmark{13},
S.~Mollerach\altaffilmark{1},
F.~Montanet\altaffilmark{34},
C.~Morello\altaffilmark{50,49},
M.~Mostaf\'a\altaffilmark{86},
A.L.~M\"uller\altaffilmark{8,37},
M.A.~Muller\altaffilmark{20,1003,24},
K.~Mulrey\altaffilmark{14},
R.~Mussa\altaffilmark{49},
M.~Muzio\altaffilmark{85},
W.M.~Namasaka\altaffilmark{35},
L.~Nellen\altaffilmark{63},
M.~Niculescu-Oglinzanu\altaffilmark{68},
M.~Niechciol\altaffilmark{41},
D.~Nitz\altaffilmark{84,1006},
D.~Nosek\altaffilmark{29},
V.~Novotny\altaffilmark{29},
L.~No\v{z}ka\altaffilmark{31},
A Nucita\altaffilmark{52,45},
L.A.~N\'u\~nez\altaffilmark{28},
M.~Palatka\altaffilmark{30},
J.~Pallotta\altaffilmark{2},
M.P.~Panetta\altaffilmark{52,45},
P.~Papenbreer\altaffilmark{35},
G.~Parente\altaffilmark{74},
A.~Parra\altaffilmark{59},
M.~Pech\altaffilmark{30},
F.~Pedreira\altaffilmark{74},
J.~P\c{e}kala\altaffilmark{64},
R.~Pelayo\altaffilmark{61},
J.~Pe\~na-Rodriguez\altaffilmark{28},
J.~Perez Armand\altaffilmark{19},
M.~Perlin\altaffilmark{8,37},
L.~Perrone\altaffilmark{52,45},
C.~Peters\altaffilmark{39},
S.~Petrera\altaffilmark{42,43},
T.~Pierog\altaffilmark{37},
M.~Pimenta\altaffilmark{67},
V.~Pirronello\altaffilmark{54,44},
M.~Platino\altaffilmark{8},
B.~Pont\altaffilmark{75},
M.~Pothast\altaffilmark{77,75},
P.~Privitera\altaffilmark{87},
M.~Prouza\altaffilmark{30},
A.~Puyleart\altaffilmark{84},
S.~Querchfeld\altaffilmark{35},
J.~Rautenberg\altaffilmark{35},
D.~Ravignani\altaffilmark{8},
M.~Reininghaus\altaffilmark{37,8},
J.~Ridky\altaffilmark{30},
F.~Riehn\altaffilmark{67},
M.~Risse\altaffilmark{41},
P.~Ristori\altaffilmark{2},
V.~Rizi\altaffilmark{53,43},
W.~Rodrigues de Carvalho\altaffilmark{19},
J.~Rodriguez Rojo\altaffilmark{9},
M.J.~Roncoroni\altaffilmark{8},
M.~Roth\altaffilmark{37},
E.~Roulet\altaffilmark{1},
A.C.~Rovero\altaffilmark{5},
P.~Ruehl\altaffilmark{41},
S.J.~Saffi\altaffilmark{12},
A.~Saftoiu\altaffilmark{68},
F.~Salamida\altaffilmark{53,43},
H.~Salazar\altaffilmark{59},
G.~Salina\altaffilmark{48},
J.D.~Sanabria Gomez\altaffilmark{28},
F.~S\'anchez\altaffilmark{8},
E.M.~Santos\altaffilmark{19},
E.~Santos\altaffilmark{30},
F.~Sarazin\altaffilmark{81},
R.~Sarmento\altaffilmark{67},
C.~Sarmiento-Cano\altaffilmark{8},
R.~Sato\altaffilmark{9},
P.~Savina\altaffilmark{52,45,32},
C.~Sch\"afer\altaffilmark{37},
V.~Scherini\altaffilmark{45},
H.~Schieler\altaffilmark{37},
M.~Schimassek\altaffilmark{36,8},
M.~Schimp\altaffilmark{35},
F.~Schl\"uter\altaffilmark{37,8},
D.~Schmidt\altaffilmark{36},
O.~Scholten\altaffilmark{76,14},
P.~Schov\'anek\altaffilmark{30},
F.G.~Schr\"oder\altaffilmark{88,37},
S.~Schr\"oder\altaffilmark{35},
S.J.~Sciutto\altaffilmark{4},
M.~Scornavacche\altaffilmark{8,37},
R.C.~Shellard\altaffilmark{15},
G.~Sigl\altaffilmark{40},
G.~Silli\altaffilmark{8,37},
O.~Sima\altaffilmark{68,1007},
R.~\v{S}m\'\i{}da\altaffilmark{87},
P.~Sommers\altaffilmark{86},
J.F.~Soriano\altaffilmark{82},
J.~Souchard\altaffilmark{34},
R.~Squartini\altaffilmark{9},
M.~Stadelmaier\altaffilmark{37,8},
D.~Stanca\altaffilmark{68},
S.~Stani\v{c}\altaffilmark{71},
J.~Stasielak\altaffilmark{64},
P.~Stassi\altaffilmark{34},
A.~Streich\altaffilmark{36,8},
M.~Su\'arez-Dur\'an\altaffilmark{28},
T.~Sudholz\altaffilmark{12},
T.~Suomij\"arvi\altaffilmark{32},
A.D.~Supanitsky\altaffilmark{8},
J.~\v{S}up\'\i{}k\altaffilmark{31},
Z.~Szadkowski\altaffilmark{66},
A.~Taboada\altaffilmark{36},
A.~Tapia\altaffilmark{27},
C.~Timmermans\altaffilmark{77,75},
P.~Tobiska\altaffilmark{30},
C.J.~Todero Peixoto\altaffilmark{17},
B.~Tom\'e\altaffilmark{67},
G.~Torralba Elipe\altaffilmark{74},
A.~Travaini\altaffilmark{9},
P.~Travnicek\altaffilmark{30},
C.~Trimarelli\altaffilmark{53,43},
M.~Trini\altaffilmark{71},
M.~Tueros\altaffilmark{4},
R.~Ulrich\altaffilmark{37},
M.~Unger\altaffilmark{37},
M.~Urban\altaffilmark{39},
L.~Vaclavek\altaffilmark{31},
M.~Vacula\altaffilmark{31},
J.F.~Vald\'es Galicia\altaffilmark{63},
I.~Vali\~no\altaffilmark{42,43},
L.~Valore\altaffilmark{56,47},
A.~van Vliet\altaffilmark{75},
E.~Varela\altaffilmark{59},
B.~Vargas C\'ardenas\altaffilmark{63},
A.~V\'asquez-Ram\'\i{}rez\altaffilmark{28},
D.~Veberi\v{c}\altaffilmark{37},
C.~Ventura\altaffilmark{25},
I.D.~Vergara Quispe\altaffilmark{4},
V.~Verzi\altaffilmark{48},
J.~Vicha\altaffilmark{30},
L.~Villase\~nor\altaffilmark{59},
J.~Vink\altaffilmark{79},
S.~Vorobiov\altaffilmark{71},
H.~Wahlberg\altaffilmark{4},
A.A.~Watson\altaffilmark{1000},
M.~Weber\altaffilmark{38},
A.~Weindl\altaffilmark{37},
L.~Wiencke\altaffilmark{81},
H.~Wilczy\'nski\altaffilmark{64},
T.~Winchen\altaffilmark{14},
M.~Wirtz\altaffilmark{39},
D.~Wittkowski\altaffilmark{35},
B.~Wundheiler\altaffilmark{8},
A.~Yushkov\altaffilmark{30},
O.~Zapparrata\altaffilmark{13},
E.~Zas\altaffilmark{74},
D.~Zavrtanik\altaffilmark{71,72},
M.~Zavrtanik\altaffilmark{72,71},
L.~Zehrer\altaffilmark{71},
A.~Zepeda\altaffilmark{60},
M.~Ziolkowski\altaffilmark{41},
F.~Zuccarello\altaffilmark{54,44}
}

\fullcollaborationName{The Pierre Auger Collaboration}

\altaffiltext{1}{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}
\altaffiltext{2}{Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina}
\altaffiltext{3}{Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina}
\altaffiltext{4}{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}
\altaffiltext{5}{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}
\altaffiltext{6}{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}
\altaffiltext{7}{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}
\altaffiltext{8}{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\altaffiltext{9}{Observatorio Pierre Auger, Malarg\"ue, Argentina}
\altaffiltext{10}{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}
\altaffiltext{11}{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}
\altaffiltext{12}{University of Adelaide, Adelaide, S.A., Australia}
\altaffiltext{13}{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}
\altaffiltext{14}{Vrije Universiteit Brussels, Brussels, Belgium}
\altaffiltext{15}{Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil}
\altaffiltext{16}{Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil}
\altaffiltext{17}{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}
\altaffiltext{18}{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}
\altaffiltext{19}{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}
\altaffiltext{20}{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}
\altaffiltext{21}{Universidade Estadual de Feira de Santana, Feira de Santana, Brazil}
\altaffiltext{22}{Universidade Federal do ABC, Santo Andr\'e, SP, Brazil}
\altaffiltext{23}{Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil}
\altaffiltext{24}{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}
\altaffiltext{25}{Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil}
\altaffiltext{26}{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}
\altaffiltext{27}{Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia}
\altaffiltext{28}{Universidad Industrial de Santander, Bucaramanga, Colombia}
\altaffiltext{29}{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}
\altaffiltext{30}{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}
\altaffiltext{31}{Palacky University, RCPTM, Olomouc, Czech Republic}
\altaffiltext{32}{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}
\altaffiltext{33}{Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Universit\'es Paris 6 et Paris 7, CNRS-IN2P3, Paris, France}
\altaffiltext{34}{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}
\altaffiltext{35}{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}
\altaffiltext{36}{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}
\altaffiltext{37}{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\altaffiltext{38}{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}
\altaffiltext{39}{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}
\altaffiltext{40}{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}
\altaffiltext{41}{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}
\altaffiltext{42}{Gran Sasso Science Institute, L'Aquila, Italy}
\altaffiltext{43}{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}
\altaffiltext{44}{INFN, Sezione di Catania, Catania, Italy}
\altaffiltext{45}{INFN, Sezione di Lecce, Lecce, Italy}
\altaffiltext{46}{INFN, Sezione di Milano, Milano, Italy}
\altaffiltext{47}{INFN, Sezione di Napoli, Napoli, Italy}
\altaffiltext{48}{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}
\altaffiltext{49}{INFN, Sezione di Torino, Torino, Italy}
\altaffiltext{50}{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\altaffiltext{51}{Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy}
\altaffiltext{52}{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\altaffiltext{53}{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\altaffiltext{54}{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\altaffiltext{55}{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\altaffiltext{56}{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\altaffiltext{57}{Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy}
\altaffiltext{58}{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\altaffiltext{59}{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}
\altaffiltext{60}{Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico, D.F., M\'exico}
\altaffiltext{61}{Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico}
\altaffiltext{62}{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}
\altaffiltext{63}{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}
\altaffiltext{64}{Institute of Nuclear Physics PAN, Krakow, Poland}
\altaffiltext{65}{University of \L{}\'od\'z, Faculty of Astrophysics, \L{}\'od\'z, Poland}
\altaffiltext{66}{University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland}
\altaffiltext{67}{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}
\altaffiltext{68}{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}
\altaffiltext{69}{Institute of Space Science, Bucharest-Magurele, Romania}
\altaffiltext{70}{University Politehnica of Bucharest, Bucharest, Romania}
\altaffiltext{71}{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}
\altaffiltext{72}{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\altaffiltext{73}{Universidad de Granada and C.A.F.P.E., Granada, Spain}
\altaffiltext{74}{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}
\altaffiltext{75}{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\altaffiltext{76}{KVI -- Center for Advanced Radiation Technology, University of Groningen, Groningen, The Netherlands}
\altaffiltext{77}{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\altaffiltext{78}{Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands}
\altaffiltext{79}{Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands}
\altaffiltext{80}{Case Western Reserve University, Cleveland, OH, USA}
\altaffiltext{81}{Colorado School of Mines, Golden, CO, USA}
\altaffiltext{82}{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}
\altaffiltext{83}{Louisiana State University, Baton Rouge, LA, USA}
\altaffiltext{84}{Michigan Technological University, Houghton, MI, USA}
\altaffiltext{85}{New York University, New York, NY, USA}
\altaffiltext{86}{Pennsylvania State University, University Park, PA, USA}
\altaffiltext{87}{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}
\altaffiltext{88}{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}
\altaffiltext{}{-----}
\altaffiltext{1000}{School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom}
\altaffiltext{1001}{Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany}
\altaffiltext{1002}{Fermi National Accelerator Laboratory, USA}
\altaffiltext{1003}{also at Universidade Federal de Alfenas, Po\c{c}os de Caldas, Brazil}
\altaffiltext{1004}{Colorado State University, Fort Collins, CO, USA}
\altaffiltext{1005}{now at Hakubi Center for Advanced Research and Graduate School of Science, Kyoto University, Kyoto, Japan}
\altaffiltext{1006}{also at Karlsruhe Institute of Technology, Karlsruhe, Germany}
\altaffiltext{1007}{also at Radboud Universtiy Nijmegen, Nijmegen, The Netherlands}


==> 2020-04-author_list-ZIP/templates/aastex/acknowledgments.tex <==
% created on 2020-04-02

\section*{Acknowledgments}

\begin{sloppypar}
The successful installation, commissioning, and operation of the Pierre
Auger Observatory would not have been possible without the strong
commitment and effort from the technical and administrative staff in
Malarg\"ue. We are very grateful to the following agencies and
organizations for financial support:
\end{sloppypar}

\begin{sloppypar}
Argentina -- Comisi\'on Nacional de Energ\'\i{}a At\'omica; Agencia Nacional de
Promoci\'on Cient\'\i{}fica y Tecnol\'ogica (ANPCyT); Consejo Nacional de
Investigaciones Cient\'\i{}ficas y T\'ecnicas (CONICET); Gobierno de la
Provincia de Mendoza; Municipalidad de Malarg\"ue; NDM Holdings and Valle
Las Le\~nas; in gratitude for their continuing cooperation over land
access; Australia -- the Australian Research Council; Brazil -- Conselho
Nacional de Desenvolvimento Cient\'\i{}fico e Tecnol\'ogico (CNPq);
Financiadora de Estudos e Projetos (FINEP); Funda\c{c}\~ao de Amparo \`a
Pesquisa do Estado de Rio de Janeiro (FAPERJ); S\~ao Paulo Research
Foundation (FAPESP) Grants No.~2019/10151-2, No.~2010/07359-6 and
No.~1999/05404-3; Minist\'erio da Ci\^encia, Tecnologia, Inova\c{c}\~oes e
Comunica\c{c}\~oes (MCTIC); Czech Republic -- Grant No.~MSMT CR LTT18004,
LM2015038, LM2018102, CZ.02.1.01/0.0/0.0/16{\textunderscore}013/0001402,
CZ.02.1.01/0.0/0.0/18{\textunderscore}046/0016010 and
CZ.02.1.01/0.0/0.0/17{\textunderscore}049/0008422; France -- Centre de Calcul
IN2P3/CNRS; Centre National de la Recherche Scientifique (CNRS); Conseil
R\'egional Ile-de-France; D\'epartement Physique Nucl\'eaire et Corpusculaire
(PNC-IN2P3/CNRS); D\'epartement Sciences de l'Univers (SDU-INSU/CNRS);
Institut Lagrange de Paris (ILP) Grant No.~LABEX ANR-10-LABX-63 within
the Investissements d'Avenir Programme Grant No.~ANR-11-IDEX-0004-02;
Germany -- Bundesministerium f\"ur Bildung und Forschung (BMBF); Deutsche
Forschungsgemeinschaft (DFG); Finanzministerium Baden-W\"urttemberg;
Helmholtz Alliance for Astroparticle Physics (HAP);
Helmholtz-Gemeinschaft Deutscher Forschungszentren (HGF); Ministerium
f\"ur Innovation, Wissenschaft und Forschung des Landes
Nordrhein-Westfalen; Ministerium f\"ur Wissenschaft, Forschung und Kunst
des Landes Baden-W\"urttemberg; Italy -- Istituto Nazionale di Fisica
Nucleare (INFN); Istituto Nazionale di Astrofisica (INAF); Ministero
dell'Istruzione, dell'Universit\'a e della Ricerca (MIUR); CETEMPS Center
of Excellence; Ministero degli Affari Esteri (MAE); M\'exico -- Consejo
Nacional de Ciencia y Tecnolog\'\i{}a (CONACYT) No.~167733; Universidad
Nacional Aut\'onoma de M\'exico (UNAM); PAPIIT DGAPA-UNAM; The Netherlands
-- Ministry of Education, Culture and Science; Netherlands Organisation
for Scientific Research (NWO); Dutch national e-infrastructure with the
support of SURF Cooperative; Poland -Ministry of Science and Higher
Education, grant No.~DIR/WK/2018/11; National Science Centre, Grants
No.~2013/08/M/ST9/00322, No.~2016/23/B/ST9/01635 and No.~HARMONIA
5--2013/10/M/ST9/00062, UMO-2016/22/M/ST9/00198; Portugal -- Portuguese
national funds and FEDER funds within Programa Operacional Factores de
Competitividade through Funda\c{c}\~ao para a Ci\^encia e a Tecnologia
(COMPETE); Romania -- Romanian Ministry of Education and Research, the
Program Nucleu within MCI (PN19150201/16N/2019 and PN19060102) and
project PN-III-P1-1.2-PCCDI-2017-0839/19PCCDI/2018 within PNCDI III;
Slovenia -- Slovenian Research Agency, grants P1-0031, P1-0385, I0-0033,
N1-0111; Spain -- Ministerio de Econom\'\i{}a, Industria y Competitividad
(FPA2017-85114-P and FPA2017-85197-P), Xunta de Galicia (ED431C
2017/07), Junta de Andaluc\'\i{}a (SOMM17/6104/UGR), Feder Funds, RENATA Red
Nacional Tem\'atica de Astropart\'\i{}culas (FPA2015-68783-REDT) and Mar\'\i{}a de
Maeztu Unit of Excellence (MDM-2016-0692); USA -- Department of Energy,
Contracts No.~DE-AC02-07CH11359, No.~DE-FR02-04ER41300,
No.~DE-FG02-99ER41107 and No.~DE-SC0011689; National Science Foundation,
Grant No.~0450696; The Grainger Foundation; Marie Curie-IRSES/EPLANET;
European Particle Physics Latin American Network; and UNESCO.
\end{sloppypar}


==> 2020-04-author_list-ZIP/templates/jcappub/Makefile <==
# Makefile for building latex documents (c) Darko Veberic
# $Id: Makefile 10301 2017-02-02 17:33:43Z darko $

USEPDFLATEX := 1
USEBIBTEX := 0

TEXFILES := $(shell grep -le '^\s*\\document\(class\|style\)' *.tex)
TARGETS := $(basename $(TEXFILES))
DEPENDENCIES := $(wildcard figs/* *.bib) $(filter-out $(TEXFILES), $(wildcard *.tex))

##########################################################
SHELL := bash
PDFS := $(addsuffix .pdf, $(TARGETS))
DEPENDENCIES += $(wildcard *.sty *.bib)

LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)

# 30=black 31=red 32=green 33=yellow 34=blue 35=magenta 36=cyan 37=white 0=cancel
COLORIZE := awk 'BEGIN{ec="\033[31;1m";wc="\033[34;1m";cc="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print ec""$$0""cc;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print wc""$$0""cc;next}{print}END{if(w||e)print "\n"ec"Warning/error summary:"cc"\n"wc""w""cc;if(e){print ec""e""cc;exit 1}}'

define basic_latex_rule
  for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && break ; done
endef

ifeq ($(USEBIBTEX), 1)
define latex_rule
  $(LATEX) $< ; bibtex $*
  $(call basic_latex_rule)
endef
else
define latex_rule
  $(call basic_latex_rule)
endef
endif

.PHONY: all clean

all: $(PDFS)

# dependencies
$(PDFS): $(DEPENDENCIES)

clean:
	- $(RM) *{.tex~,.dvi,.log,.aux,.toc,.nav,.out,.snm,.bbl,.blg,.spl,.lof,Notes.bib,.maf,.fff,.lot,.ttt}
	- for f in $(TARGETS) ; do $(RM) $$f{.ps,.pdf} ; done

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.dvi
	dvipdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<


==> 2020-04-author_list-ZIP/templates/jcappub/acknowledgments.tex <==
% created on 2020-04-02

\section*{Acknowledgments}

\begin{sloppypar}
The successful installation, commissioning, and operation of the Pierre
Auger Observatory would not have been possible without the strong
commitment and effort from the technical and administrative staff in
Malarg\"ue. We are very grateful to the following agencies and
organizations for financial support:
\end{sloppypar}

\begin{sloppypar}
Argentina -- Comisi\'on Nacional de Energ\'\i{}a At\'omica; Agencia Nacional de
Promoci\'on Cient\'\i{}fica y Tecnol\'ogica (ANPCyT); Consejo Nacional de
Investigaciones Cient\'\i{}ficas y T\'ecnicas (CONICET); Gobierno de la
Provincia de Mendoza; Municipalidad de Malarg\"ue; NDM Holdings and Valle
Las Le\~nas; in gratitude for their continuing cooperation over land
access; Australia -- the Australian Research Council; Brazil -- Conselho
Nacional de Desenvolvimento Cient\'\i{}fico e Tecnol\'ogico (CNPq);
Financiadora de Estudos e Projetos (FINEP); Funda\c{c}\~ao de Amparo \`a
Pesquisa do Estado de Rio de Janeiro (FAPERJ); S\~ao Paulo Research
Foundation (FAPESP) Grants No.~2019/10151-2, No.~2010/07359-6 and
No.~1999/05404-3; Minist\'erio da Ci\^encia, Tecnologia, Inova\c{c}\~oes e
Comunica\c{c}\~oes (MCTIC); Czech Republic -- Grant No.~MSMT CR LTT18004,
LM2015038, LM2018102, CZ.02.1.01/0.0/0.0/16{\textunderscore}013/0001402,
CZ.02.1.01/0.0/0.0/18{\textunderscore}046/0016010 and
CZ.02.1.01/0.0/0.0/17{\textunderscore}049/0008422; France -- Centre de Calcul
IN2P3/CNRS; Centre National de la Recherche Scientifique (CNRS); Conseil
R\'egional Ile-de-France; D\'epartement Physique Nucl\'eaire et Corpusculaire
(PNC-IN2P3/CNRS); D\'epartement Sciences de l'Univers (SDU-INSU/CNRS);
Institut Lagrange de Paris (ILP) Grant No.~LABEX ANR-10-LABX-63 within
the Investissements d'Avenir Programme Grant No.~ANR-11-IDEX-0004-02;
Germany -- Bundesministerium f\"ur Bildung und Forschung (BMBF); Deutsche
Forschungsgemeinschaft (DFG); Finanzministerium Baden-W\"urttemberg;
Helmholtz Alliance for Astroparticle Physics (HAP);
Helmholtz-Gemeinschaft Deutscher Forschungszentren (HGF); Ministerium
f\"ur Innovation, Wissenschaft und Forschung des Landes
Nordrhein-Westfalen; Ministerium f\"ur Wissenschaft, Forschung und Kunst
des Landes Baden-W\"urttemberg; Italy -- Istituto Nazionale di Fisica
Nucleare (INFN); Istituto Nazionale di Astrofisica (INAF); Ministero
dell'Istruzione, dell'Universit\'a e della Ricerca (MIUR); CETEMPS Center
of Excellence; Ministero degli Affari Esteri (MAE); M\'exico -- Consejo
Nacional de Ciencia y Tecnolog\'\i{}a (CONACYT) No.~167733; Universidad
Nacional Aut\'onoma de M\'exico (UNAM); PAPIIT DGAPA-UNAM; The Netherlands
-- Ministry of Education, Culture and Science; Netherlands Organisation
for Scientific Research (NWO); Dutch national e-infrastructure with the
support of SURF Cooperative; Poland -Ministry of Science and Higher
Education, grant No.~DIR/WK/2018/11; National Science Centre, Grants
No.~2013/08/M/ST9/00322, No.~2016/23/B/ST9/01635 and No.~HARMONIA
5--2013/10/M/ST9/00062, UMO-2016/22/M/ST9/00198; Portugal -- Portuguese
national funds and FEDER funds within Programa Operacional Factores de
Competitividade through Funda\c{c}\~ao para a Ci\^encia e a Tecnologia
(COMPETE); Romania -- Romanian Ministry of Education and Research, the
Program Nucleu within MCI (PN19150201/16N/2019 and PN19060102) and
project PN-III-P1-1.2-PCCDI-2017-0839/19PCCDI/2018 within PNCDI III;
Slovenia -- Slovenian Research Agency, grants P1-0031, P1-0385, I0-0033,
N1-0111; Spain -- Ministerio de Econom\'\i{}a, Industria y Competitividad
(FPA2017-85114-P and FPA2017-85197-P), Xunta de Galicia (ED431C
2017/07), Junta de Andaluc\'\i{}a (SOMM17/6104/UGR), Feder Funds, RENATA Red
Nacional Tem\'atica de Astropart\'\i{}culas (FPA2015-68783-REDT) and Mar\'\i{}a de
Maeztu Unit of Excellence (MDM-2016-0692); USA -- Department of Energy,
Contracts No.~DE-AC02-07CH11359, No.~DE-FR02-04ER41300,
No.~DE-FG02-99ER41107 and No.~DE-SC0011689; National Science Foundation,
Grant No.~0450696; The Grainger Foundation; Marie Curie-IRSES/EPLANET;
European Particle Physics Latin American Network; and UNESCO.
\end{sloppypar}


==> 2020-04-author_list-ZIP/templates/jcappub/jcappub_authorlist.tex <==
% created on 2020-04-02

\author[75]{A.~Aab,}
\author[67]{P.~Abreu,}
\author[50,49]{M.~Aglietta,}
\author[12]{J.M.~Albury,}
\author[1]{I.~Allekotte,}
\author[8,11]{A.~Almela,}
\author[63]{J.~Alvarez Castillo,}
\author[74]{J.~Alvarez-Mu\~niz,}
\author[75]{R.~Alves Batista,}
\author[58,49]{G.A.~Anastasi,}
\author[82]{L.~Anchordoqui,}
\author[8]{B.~Andrada,}
\author[67]{S.~Andringa,}
\author[47]{C.~Aramo,}
\author[39]{P.R.~Ara\'ujo Ferreira,}
\author[8]{H.~Asorey,}
\author[67]{P.~Assis,}
\author[9,10]{G.~Avila,}
\author[70]{A.M.~Badescu,}
\author[30]{A.~Bakalova,}
\author[68]{A.~Balaceanu,}
\author[56,47]{F.~Barbato,}
\author[67]{R.J.~Barreira Luz,}
\author[35]{K.H.~Becker,}
\author[12]{J.A.~Bellido,}
\author[34]{C.~Berat,}
\author[58,49]{M.E.~Bertaina,}
\author[1]{X.~Bertou,}
\author[b]{P.L.~Biermann,}
\author[39]{T.~Bister,}
\author[32]{J.~Biteau,}
\author[67]{A.~Blanco,}
\author[30]{J.~Blazek,}
\author[34]{C.~Bleve,}
\author[30]{M.~Boh\'a\v{c}ov\'a,}
\author[53,43]{D.~Boncioli,}
\author[24]{C.~Bonifazi,}
\author[19]{L.~Bonneau Arbeletche,}
\author[64]{N.~Borodai,}
\author[8]{A.M.~Botti,}
\author[e]{J.~Brack,}
\author[39]{T.~Bretz,}
\author[39]{F.L.~Briechle,}
\author[41]{P.~Buchholz,}
\author[73]{A.~Bueno,}
\author[14]{S.~Buitink,}
\author[54,44]{M.~Buscemi,}
\author[62]{K.S.~Caballero-Mora,}
\author[55,46]{L.~Caccianiga,}
\author[4]{L.~Calcagni,}
\author[11,8]{A.~Cancio,}
\author[75,77]{F.~Canfora,}
\author[35]{I.~Caracas,}
\author[73]{J.M.~Carceller,}
\author[54,44]{R.~Caruso,}
\author[50,49]{A.~Castellina,}
\author[17]{F.~Catalani,}
\author[45]{G.~Cataldi,}
\author[67]{L.~Cazon,}
\author[9]{M.~Cerda,}
\author[20]{J.A.~Chinellato,}
\author[74]{K.~Choi,}
\author[30]{J.~Chudoba,}
\author[31]{L.~Chytka,}
\author[12]{R.W.~Clay,}
\author[7]{A.C.~Cobos Cerutti,}
\author[56,47]{R.~Colalillo,}
\author[88]{A.~Coleman,}
\author[52,45]{M.R.~Coluccia,}
\author[67]{R.~Concei\c{c}\~ao,}
\author[42,43]{A.~Condorelli,}
\author[46,51]{G.~Consolati,}
\author[9,10]{F.~Contreras,}
\author[52,45]{F.~Convenga,}
\author[80,h]{C.E.~Covault,}
\author[5,3]{S.~Dasso,}
\author[37]{K.~Daumiller,}
\author[12]{B.R.~Dawson,}
\author[12]{J.A.~Day,}
\author[26]{R.M.~de Almeida,}
\author[8,37]{J.~de Jes\'us,}
\author[75,77]{S.J.~de Jong,}
\author[75,77]{G.~De Mauro,}
\author[24,25]{J.R.T.~de Mello Neto,}
\author[42,43]{I.~De Mitri,}
\author[26]{J.~de Oliveira,}
\author[20]{D.~de Oliveira Franco,}
\author[18]{V.~de Souza,}
\author[36]{J.~Debatin,}
\author[10]{M.~del R\'\i{}o,}
\author[32]{O.~Deligny,}
\author[64]{N.~Dhital,}
\author[49]{A.~Di Matteo,}
\author[20]{M.L.~D\'\i{}az Castro,}
\author[20]{C.~Dobrigkeit,}
\author[63]{J.C.~D'Olivo,}
\author[41]{Q.~Dorosti,}
\author[23]{R.C.~dos Anjos,}
\author[4]{M.T.~Dova,}
\author[30]{J.~Ebr,}
\author[36,37]{R.~Engel,}
\author[52,45]{I.~Epicoco,}
\author[39]{M.~Erdmann,}
\author[c]{C.O.~Escobar,}
\author[8,11]{A.~Etchegoyen,}
\author[75,78,77]{H.~Falcke,}
\author[87]{J.~Farmer,}
\author[85]{G.~Farrar,}
\author[20]{A.C.~Fauth,}
\author[c]{N.~Fazzini,}
\author[38]{F.~Feldbusch,}
\author[58,49]{F.~Fenu,}
\author[84]{B.~Fick,}
\author[8]{J.M.~Figueira,}
\author[72,71]{A.~Filip\v{c}i\v{c},}
\author[75]{T.~Fodran,}
\author[6]{M.M.~Freire,}
\author[87,f]{T.~Fujii,}
\author[8,11]{A.~Fuster,}
\author[75]{C.~Galea,}
\author[55,46]{C.~Galelli,}
\author[7]{B.~Garc\'\i{}a,}
\author[39]{A.L.~Garcia Vegas,}
\author[38]{H.~Gemmeke,}
\author[8,37]{F.~Gesualdi,}
\author[68]{A.~Gherghel-Lascu,}
\author[32]{P.L.~Ghia,}
\author[75]{U.~Giaccari,}
\author[46]{M.~Giammarchi,}
\author[65]{M.~Giller,}
\author[39]{J.~Glombitza,}
\author[9]{F.~Gobbi,}
\author[1]{G.~Golup,}
\author[1]{M.~G\'omez Berisso,}
\author[9,10]{P.F.~G\'omez Vitale,}
\author[9]{J.P.~Gongora,}
\author[8]{N.~Gonz\'alez,}
\author[1,37]{I.~Goos,}
\author[64]{D.~G\'ora,}
\author[50,49]{A.~Gorgi,}
\author[35]{M.~Gottowik,}
\author[12]{T.D.~Grubb,}
\author[56,47]{F.~Guarino,}
\author[21]{G.P.~Guedes,}
\author[49,58]{E.~Guido,}
\author[37,8]{S.~Hahn,}
\author[80]{R.~Halliday,}
\author[8]{M.R.~Hampel,}
\author[4]{P.~Hansen,}
\author[1]{D.~Harari,}
\author[12]{V.M.~Harvey,}
\author[37]{A.~Haungs,}
\author[39]{T.~Hebbeker,}
\author[37]{D.~Heck,}
\author[12]{G.C.~Hill,}
\author[c]{C.~Hojvat,}
\author[75,77]{J.R.~H\"orandel,}
\author[31]{P.~Horvath,}
\author[31]{M.~Hrabovsk\'y,}
\author[37,14]{T.~Huege,}
\author[8,37]{J.~Hulsman,}
\author[54,44]{A.~Insolia,}
\author[69]{P.G.~Isar,}
\author[81]{J.A.~Johnsen,}
\author[30]{J.~Jurysek,}
\author[35]{A.~K\"a\"ap\"a,}
\author[35]{K.H.~Kampert,}
\author[37]{B.~Keilhauer,}
\author[39]{J.~Kemp,}
\author[37]{H.O.~Klages,}
\author[38]{M.~Kleifges,}
\author[9]{J.~Kleinfeller,}
\author[36]{M.~K\"opke,}
\author[71]{G.~Kukec Mezek,}
\author[16]{B.L.~Lago,}
\author[80]{D.~LaHurd,}
\author[18]{R.G.~Lang,}
\author[22]{M.A.~Leigui de Oliveira,}
\author[37]{V.~Lenok,}
\author[33]{A.~Letessier-Selvon,}
\author[32]{I.~Lhenry-Yvon,}
\author[54,44]{D.~Lo Presti,}
\author[67]{L.~Lopes,}
\author[59]{R.~L\'opez,}
\author[80]{R.~Lorek,}
\author[36]{Q.~Luce,}
\author[8]{A.~Lucero,}
\author[20]{A.~Machado Payeras,}
\author[87]{M.~Malacari,}
\author[52,45]{G.~Mancarella,}
\author[30]{D.~Mandat,}
\author[12]{B.C.~Manning,}
\author[40]{J.~Manshanden,}
\author[c]{P.~Mantsch,}
\author[32]{S.~Marafico,}
\author[4]{A.G.~Mariazzi,}
\author[13]{I.C.~Mari\c{s},}
\author[52,45]{G.~Marsella,}
\author[52,45]{D.~Martello,}
\author[18]{H.~Martinez,}
\author[59]{O.~Mart\'\i{}nez Bravo,}
\author[53,43]{M.~Mastrodicasa,}
\author[37]{H.J.~Mathes,}
\author[83]{J.~Matthews,}
\author[57,48]{G.~Matthiae,}
\author[35]{E.~Mayotte,}
\author[c]{P.O.~Mazur,}
\author[63]{G.~Medina-Tanco,}
\author[8]{D.~Melo,}
\author[38]{A.~Menshikov,}
\author[81]{K.-D.~Merenda,}
\author[31]{S.~Michal,}
\author[6]{M.I.~Micheletti,}
\author[55,46]{L.~Miramonti,}
\author[13]{D.~Mockler,}
\author[1]{S.~Mollerach,}
\author[34]{F.~Montanet,}
\author[50,49]{C.~Morello,}
\author[86]{M.~Mostaf\'a,}
\author[8,37]{A.L.~M\"uller,}
\author[20,d,24]{M.A.~Muller,}
\author[14]{K.~Mulrey,}
\author[49]{R.~Mussa,}
\author[85]{M.~Muzio,}
\author[35]{W.M.~Namasaka,}
\author[63]{L.~Nellen,}
\author[68]{M.~Niculescu-Oglinzanu,}
\author[41]{M.~Niechciol,}
\author[84,g]{D.~Nitz,}
\author[29]{D.~Nosek,}
\author[29]{V.~Novotny,}
\author[31]{L.~No\v{z}ka,}
\author[52,45]{A Nucita,}
\author[28]{L.A.~N\'u\~nez,}
\author[30]{M.~Palatka,}
\author[2]{J.~Pallotta,}
\author[52,45]{M.P.~Panetta,}
\author[35]{P.~Papenbreer,}
\author[74]{G.~Parente,}
\author[59]{A.~Parra,}
\author[30]{M.~Pech,}
\author[74]{F.~Pedreira,}
\author[64]{J.~P\c{e}kala,}
\author[61]{R.~Pelayo,}
\author[28]{J.~Pe\~na-Rodriguez,}
\author[19]{J.~Perez Armand,}
\author[8,37]{M.~Perlin,}
\author[52,45]{L.~Perrone,}
\author[39]{C.~Peters,}
\author[42,43]{S.~Petrera,}
\author[37]{T.~Pierog,}
\author[67]{M.~Pimenta,}
\author[54,44]{V.~Pirronello,}
\author[8]{M.~Platino,}
\author[75]{B.~Pont,}
\author[77,75]{M.~Pothast,}
\author[87]{P.~Privitera,}
\author[30]{M.~Prouza,}
\author[84]{A.~Puyleart,}
\author[35]{S.~Querchfeld,}
\author[35]{J.~Rautenberg,}
\author[8]{D.~Ravignani,}
\author[37,8]{M.~Reininghaus,}
\author[30]{J.~Ridky,}
\author[67]{F.~Riehn,}
\author[41]{M.~Risse,}
\author[2]{P.~Ristori,}
\author[53,43]{V.~Rizi,}
\author[19]{W.~Rodrigues de Carvalho,}
\author[9]{J.~Rodriguez Rojo,}
\author[8]{M.J.~Roncoroni,}
\author[37]{M.~Roth,}
\author[1]{E.~Roulet,}
\author[5]{A.C.~Rovero,}
\author[41]{P.~Ruehl,}
\author[12]{S.J.~Saffi,}
\author[68]{A.~Saftoiu,}
\author[53,43]{F.~Salamida,}
\author[59]{H.~Salazar,}
\author[48]{G.~Salina,}
\author[28]{J.D.~Sanabria Gomez,}
\author[8]{F.~S\'anchez,}
\author[19]{E.M.~Santos,}
\author[30]{E.~Santos,}
\author[81]{F.~Sarazin,}
\author[67]{R.~Sarmento,}
\author[8]{C.~Sarmiento-Cano,}
\author[9]{R.~Sato,}
\author[52,45,32]{P.~Savina,}
\author[37]{C.~Sch\"afer,}
\author[45]{V.~Scherini,}
\author[37]{H.~Schieler,}
\author[36,8]{M.~Schimassek,}
\author[35]{M.~Schimp,}
\author[37,8]{F.~Schl\"uter,}
\author[36]{D.~Schmidt,}
\author[76,14]{O.~Scholten,}
\author[30]{P.~Schov\'anek,}
\author[88,37]{F.G.~Schr\"oder,}
\author[35]{S.~Schr\"oder,}
\author[4]{S.J.~Sciutto,}
\author[8,37]{M.~Scornavacche,}
\author[15]{R.C.~Shellard,}
\author[40]{G.~Sigl,}
\author[8,37]{G.~Silli,}
\author[68,h]{O.~Sima,}
\author[87]{R.~\v{S}m\'\i{}da,}
\author[86]{P.~Sommers,}
\author[82]{J.F.~Soriano,}
\author[34]{J.~Souchard,}
\author[9]{R.~Squartini,}
\author[37,8]{M.~Stadelmaier,}
\author[68]{D.~Stanca,}
\author[71]{S.~Stani\v{c},}
\author[64]{J.~Stasielak,}
\author[34]{P.~Stassi,}
\author[36,8]{A.~Streich,}
\author[28]{M.~Su\'arez-Dur\'an,}
\author[12]{T.~Sudholz,}
\author[32]{T.~Suomij\"arvi,}
\author[8]{A.D.~Supanitsky,}
\author[31]{J.~\v{S}up\'\i{}k,}
\author[66]{Z.~Szadkowski,}
\author[36]{A.~Taboada,}
\author[27]{A.~Tapia,}
\author[77,75]{C.~Timmermans,}
\author[30]{P.~Tobiska,}
\author[17]{C.J.~Todero Peixoto,}
\author[67]{B.~Tom\'e,}
\author[74]{G.~Torralba Elipe,}
\author[9]{A.~Travaini,}
\author[30]{P.~Travnicek,}
\author[53,43]{C.~Trimarelli,}
\author[71]{M.~Trini,}
\author[4]{M.~Tueros,}
\author[37]{R.~Ulrich,}
\author[37]{M.~Unger,}
\author[39]{M.~Urban,}
\author[31]{L.~Vaclavek,}
\author[31]{M.~Vacula,}
\author[63]{J.F.~Vald\'es Galicia,}
\author[42,43]{I.~Vali\~no,}
\author[56,47]{L.~Valore,}
\author[75]{A.~van Vliet,}
\author[59]{E.~Varela,}
\author[63]{B.~Vargas C\'ardenas,}
\author[28]{A.~V\'asquez-Ram\'\i{}rez,}
\author[37]{D.~Veberi\v{c},}
\author[25]{C.~Ventura,}
\author[4]{I.D.~Vergara Quispe,}
\author[48]{V.~Verzi,}
\author[30]{J.~Vicha,}
\author[59]{L.~Villase\~nor,}
\author[79]{J.~Vink,}
\author[71]{S.~Vorobiov,}
\author[4]{H.~Wahlberg,}
\author[a]{A.A.~Watson,}
\author[38]{M.~Weber,}
\author[37]{A.~Weindl,}
\author[81]{L.~Wiencke,}
\author[64]{H.~Wilczy\'nski,}
\author[14]{T.~Winchen,}
\author[39]{M.~Wirtz,}
\author[35]{D.~Wittkowski,}
\author[8]{B.~Wundheiler,}
\author[30]{A.~Yushkov,}
\author[13]{O.~Zapparrata,}
\author[74]{E.~Zas,}
\author[71,72]{D.~Zavrtanik,}
\author[72,71]{M.~Zavrtanik,}
\author[71]{L.~Zehrer,}
\author[60]{A.~Zepeda,}
\author[41]{M.~Ziolkowski,}
\author[54,44]{and F.~Zuccarello}

\affiliation[1]{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}
\affiliation[2]{Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina}
\affiliation[3]{Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina}
\affiliation[4]{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}
\affiliation[5]{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}
\affiliation[6]{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}
\affiliation[7]{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}
\affiliation[8]{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation[9]{Observatorio Pierre Auger, Malarg\"ue, Argentina}
\affiliation[10]{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}
\affiliation[11]{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}
\affiliation[12]{University of Adelaide, Adelaide, S.A., Australia}
\affiliation[13]{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}
\affiliation[14]{Vrije Universiteit Brussels, Brussels, Belgium}
\affiliation[15]{Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil}
\affiliation[16]{Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil}
\affiliation[17]{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}
\affiliation[18]{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}
\affiliation[19]{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}
\affiliation[20]{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}
\affiliation[21]{Universidade Estadual de Feira de Santana, Feira de Santana, Brazil}
\affiliation[22]{Universidade Federal do ABC, Santo Andr\'e, SP, Brazil}
\affiliation[23]{Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil}
\affiliation[24]{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}
\affiliation[25]{Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil}
\affiliation[26]{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}
\affiliation[27]{Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia}
\affiliation[28]{Universidad Industrial de Santander, Bucaramanga, Colombia}
\affiliation[29]{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}
\affiliation[30]{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}
\affiliation[31]{Palacky University, RCPTM, Olomouc, Czech Republic}
\affiliation[32]{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}
\affiliation[33]{Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Universit\'es Paris 6 et Paris 7, CNRS-IN2P3, Paris, France}
\affiliation[34]{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}
\affiliation[35]{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}
\affiliation[36]{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}
\affiliation[37]{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\affiliation[38]{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}
\affiliation[39]{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}
\affiliation[40]{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}
\affiliation[41]{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}
\affiliation[42]{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation[43]{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}
\affiliation[44]{INFN, Sezione di Catania, Catania, Italy}
\affiliation[45]{INFN, Sezione di Lecce, Lecce, Italy}
\affiliation[46]{INFN, Sezione di Milano, Milano, Italy}
\affiliation[47]{INFN, Sezione di Napoli, Napoli, Italy}
\affiliation[48]{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}
\affiliation[49]{INFN, Sezione di Torino, Torino, Italy}
\affiliation[50]{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation[51]{Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy}
\affiliation[52]{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation[53]{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation[54]{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation[55]{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation[56]{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation[57]{Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy}
\affiliation[58]{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation[59]{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}
\affiliation[60]{Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico, D.F., M\'exico}
\affiliation[61]{Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico}
\affiliation[62]{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}
\affiliation[63]{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}
\affiliation[64]{Institute of Nuclear Physics PAN, Krakow, Poland}
\affiliation[65]{University of \L{}\'od\'z, Faculty of Astrophysics, \L{}\'od\'z, Poland}
\affiliation[66]{University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland}
\affiliation[67]{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}
\affiliation[68]{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}
\affiliation[69]{Institute of Space Science, Bucharest-Magurele, Romania}
\affiliation[70]{University Politehnica of Bucharest, Bucharest, Romania}
\affiliation[71]{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}
\affiliation[72]{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\affiliation[73]{Universidad de Granada and C.A.F.P.E., Granada, Spain}
\affiliation[74]{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}
\affiliation[75]{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation[76]{KVI -- Center for Advanced Radiation Technology, University of Groningen, Groningen, The Netherlands}
\affiliation[77]{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\affiliation[78]{Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands}
\affiliation[79]{Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands}
\affiliation[80]{Case Western Reserve University, Cleveland, OH, USA}
\affiliation[81]{Colorado School of Mines, Golden, CO, USA}
\affiliation[82]{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}
\affiliation[83]{Louisiana State University, Baton Rouge, LA, USA}
\affiliation[84]{Michigan Technological University, Houghton, MI, USA}
\affiliation[85]{New York University, New York, NY, USA}
\affiliation[86]{Pennsylvania State University, University Park, PA, USA}
\affiliation[87]{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}
\affiliation[88]{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}
\affiliation[]{-----}
\affiliation[a]{School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom}
\affiliation[b]{Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany}
\affiliation[c]{Fermi National Accelerator Laboratory, USA}
\affiliation[d]{also at Universidade Federal de Alfenas, Po\c{c}os de Caldas, Brazil}
\affiliation[e]{Colorado State University, Fort Collins, CO, USA}
\affiliation[f]{now at Hakubi Center for Advanced Research and Graduate School of Science, Kyoto University, Kyoto, Japan}
\affiliation[g]{also at Karlsruhe Institute of Technology, Karlsruhe, Germany}
\affiliation[h]{also at Radboud Universtiy Nijmegen, Nijmegen, The Netherlands}


==> 2020-04-author_list-ZIP/templates/plain_latex/Makefile <==
# Makefile for building latex documents (c) Darko Veberic
# $Id: Makefile 9325 2015-09-12 14:41:15Z darko $

USEPDFLATEX := 1
USEBIBTEX := 0

TEXFILES := $(shell grep -le '^\s*\\document\(class\|style\)' *.tex)
TARGETS := $(basename $(TEXFILES))
DEPENDENCIES := $(wildcard figs/* *.bib) $(filter-out $(TEXFILES), $(wildcard *.tex))

##########################################################
SHELL := bash
PDFS := $(addsuffix .pdf,$(TARGETS))
DEPENDENCIES += $(wildcard *.sty *.bib)

LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)

# 30=black 31=red 32=green 33=yellow 34=blue 35=magenta 36=cyan 37=white 0=cancel
COLORIZE := awk 'BEGIN{ec="\033[31;1m";wc="\033[34;1m";cc="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print ec""$$0""cc;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print wc""$$0""cc;next}{print}END{if(w||e)print "\n"ec"Warning/error summary:"cc"\n"wc""w""cc;if(e){print ec""e""cc;exit 1}}'

define basic_latex_rule
  for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && break ; done
endef

ifeq ($(USEBIBTEX), 1)
define latex_rule
  $(LATEX) $< ; bibtex $*
  $(call basic_latex_rule)
endef
else
define latex_rule
  $(call basic_latex_rule)
endef
endif

.PHONY: all clean

all: $(PDFS)

# dependencies
$(PDFS): $(DEPENDENCIES)

clean:
	- $(RM) *{.tex~,.dvi,.log,.aux,.toc,.nav,.out,.snm,.bbl,.blg,.spl,.lof,Notes.bib,.maf,.fff,.lot,.ttt}
	- for f in $(TARGETS) ; do $(RM) $$f{.ps,.pdf} ; done

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.dvi
	dvipdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<


==> 2020-04-author_list-ZIP/templates/plain_latex/acknowledgments.tex <==
% created on 2020-04-02

\section*{Acknowledgments}

\begin{sloppypar}
The successful installation, commissioning, and operation of the Pierre
Auger Observatory would not have been possible without the strong
commitment and effort from the technical and administrative staff in
Malarg\"ue. We are very grateful to the following agencies and
organizations for financial support:
\end{sloppypar}

\begin{sloppypar}
Argentina -- Comisi\'on Nacional de Energ\'\i{}a At\'omica; Agencia Nacional de
Promoci\'on Cient\'\i{}fica y Tecnol\'ogica (ANPCyT); Consejo Nacional de
Investigaciones Cient\'\i{}ficas y T\'ecnicas (CONICET); Gobierno de la
Provincia de Mendoza; Municipalidad de Malarg\"ue; NDM Holdings and Valle
Las Le\~nas; in gratitude for their continuing cooperation over land
access; Australia -- the Australian Research Council; Brazil -- Conselho
Nacional de Desenvolvimento Cient\'\i{}fico e Tecnol\'ogico (CNPq);
Financiadora de Estudos e Projetos (FINEP); Funda\c{c}\~ao de Amparo \`a
Pesquisa do Estado de Rio de Janeiro (FAPERJ); S\~ao Paulo Research
Foundation (FAPESP) Grants No.~2019/10151-2, No.~2010/07359-6 and
No.~1999/05404-3; Minist\'erio da Ci\^encia, Tecnologia, Inova\c{c}\~oes e
Comunica\c{c}\~oes (MCTIC); Czech Republic -- Grant No.~MSMT CR LTT18004,
LM2015038, LM2018102, CZ.02.1.01/0.0/0.0/16{\textunderscore}013/0001402,
CZ.02.1.01/0.0/0.0/18{\textunderscore}046/0016010 and
CZ.02.1.01/0.0/0.0/17{\textunderscore}049/0008422; France -- Centre de Calcul
IN2P3/CNRS; Centre National de la Recherche Scientifique (CNRS); Conseil
R\'egional Ile-de-France; D\'epartement Physique Nucl\'eaire et Corpusculaire
(PNC-IN2P3/CNRS); D\'epartement Sciences de l'Univers (SDU-INSU/CNRS);
Institut Lagrange de Paris (ILP) Grant No.~LABEX ANR-10-LABX-63 within
the Investissements d'Avenir Programme Grant No.~ANR-11-IDEX-0004-02;
Germany -- Bundesministerium f\"ur Bildung und Forschung (BMBF); Deutsche
Forschungsgemeinschaft (DFG); Finanzministerium Baden-W\"urttemberg;
Helmholtz Alliance for Astroparticle Physics (HAP);
Helmholtz-Gemeinschaft Deutscher Forschungszentren (HGF); Ministerium
f\"ur Innovation, Wissenschaft und Forschung des Landes
Nordrhein-Westfalen; Ministerium f\"ur Wissenschaft, Forschung und Kunst
des Landes Baden-W\"urttemberg; Italy -- Istituto Nazionale di Fisica
Nucleare (INFN); Istituto Nazionale di Astrofisica (INAF); Ministero
dell'Istruzione, dell'Universit\'a e della Ricerca (MIUR); CETEMPS Center
of Excellence; Ministero degli Affari Esteri (MAE); M\'exico -- Consejo
Nacional de Ciencia y Tecnolog\'\i{}a (CONACYT) No.~167733; Universidad
Nacional Aut\'onoma de M\'exico (UNAM); PAPIIT DGAPA-UNAM; The Netherlands
-- Ministry of Education, Culture and Science; Netherlands Organisation
for Scientific Research (NWO); Dutch national e-infrastructure with the
support of SURF Cooperative; Poland -Ministry of Science and Higher
Education, grant No.~DIR/WK/2018/11; National Science Centre, Grants
No.~2013/08/M/ST9/00322, No.~2016/23/B/ST9/01635 and No.~HARMONIA
5--2013/10/M/ST9/00062, UMO-2016/22/M/ST9/00198; Portugal -- Portuguese
national funds and FEDER funds within Programa Operacional Factores de
Competitividade through Funda\c{c}\~ao para a Ci\^encia e a Tecnologia
(COMPETE); Romania -- Romanian Ministry of Education and Research, the
Program Nucleu within MCI (PN19150201/16N/2019 and PN19060102) and
project PN-III-P1-1.2-PCCDI-2017-0839/19PCCDI/2018 within PNCDI III;
Slovenia -- Slovenian Research Agency, grants P1-0031, P1-0385, I0-0033,
N1-0111; Spain -- Ministerio de Econom\'\i{}a, Industria y Competitividad
(FPA2017-85114-P and FPA2017-85197-P), Xunta de Galicia (ED431C
2017/07), Junta de Andaluc\'\i{}a (SOMM17/6104/UGR), Feder Funds, RENATA Red
Nacional Tem\'atica de Astropart\'\i{}culas (FPA2015-68783-REDT) and Mar\'\i{}a de
Maeztu Unit of Excellence (MDM-2016-0692); USA -- Department of Energy,
Contracts No.~DE-AC02-07CH11359, No.~DE-FR02-04ER41300,
No.~DE-FG02-99ER41107 and No.~DE-SC0011689; National Science Foundation,
Grant No.~0450696; The Grainger Foundation; Marie Curie-IRSES/EPLANET;
European Particle Physics Latin American Network; and UNESCO.
\end{sloppypar}


==> 2020-04-author_list-ZIP/templates/plain_latex/latex_authorlist_authors.tex <==
% created on 2020-04-02

A.~Aab$^{75}$,
P.~Abreu$^{67}$,
M.~Aglietta$^{50,49}$,
J.M.~Albury$^{12}$,
I.~Allekotte$^{1}$,
A.~Almela$^{8,11}$,
J.~Alvarez Castillo$^{63}$,
J.~Alvarez-Mu\~niz$^{74}$,
R.~Alves Batista$^{75}$,
G.A.~Anastasi$^{58,49}$,
L.~Anchordoqui$^{82}$,
B.~Andrada$^{8}$,
S.~Andringa$^{67}$,
C.~Aramo$^{47}$,
P.R.~Ara\'ujo Ferreira$^{39}$,
H.~Asorey$^{8}$,
P.~Assis$^{67}$,
G.~Avila$^{9,10}$,
A.M.~Badescu$^{70}$,
A.~Bakalova$^{30}$,
A.~Balaceanu$^{68}$,
F.~Barbato$^{56,47}$,
R.J.~Barreira Luz$^{67}$,
K.H.~Becker$^{35}$,
J.A.~Bellido$^{12}$,
C.~Berat$^{34}$,
M.E.~Bertaina$^{58,49}$,
X.~Bertou$^{1}$,
P.L.~Biermann$^{b}$,
T.~Bister$^{39}$,
J.~Biteau$^{32}$,
A.~Blanco$^{67}$,
J.~Blazek$^{30}$,
C.~Bleve$^{34}$,
M.~Boh\'a\v{c}ov\'a$^{30}$,
D.~Boncioli$^{53,43}$,
C.~Bonifazi$^{24}$,
L.~Bonneau Arbeletche$^{19}$,
N.~Borodai$^{64}$,
A.M.~Botti$^{8}$,
J.~Brack$^{e}$,
T.~Bretz$^{39}$,
F.L.~Briechle$^{39}$,
P.~Buchholz$^{41}$,
A.~Bueno$^{73}$,
S.~Buitink$^{14}$,
M.~Buscemi$^{54,44}$,
K.S.~Caballero-Mora$^{62}$,
L.~Caccianiga$^{55,46}$,
L.~Calcagni$^{4}$,
A.~Cancio$^{11,8}$,
F.~Canfora$^{75,77}$,
I.~Caracas$^{35}$,
J.M.~Carceller$^{73}$,
R.~Caruso$^{54,44}$,
A.~Castellina$^{50,49}$,
F.~Catalani$^{17}$,
G.~Cataldi$^{45}$,
L.~Cazon$^{67}$,
M.~Cerda$^{9}$,
J.A.~Chinellato$^{20}$,
K.~Choi$^{74}$,
J.~Chudoba$^{30}$,
L.~Chytka$^{31}$,
R.W.~Clay$^{12}$,
A.C.~Cobos Cerutti$^{7}$,
R.~Colalillo$^{56,47}$,
A.~Coleman$^{88}$,
M.R.~Coluccia$^{52,45}$,
R.~Concei\c{c}\~ao$^{67}$,
A.~Condorelli$^{42,43}$,
G.~Consolati$^{46,51}$,
F.~Contreras$^{9,10}$,
F.~Convenga$^{52,45}$,
C.E.~Covault$^{80,h}$,
S.~Dasso$^{5,3}$,
K.~Daumiller$^{37}$,
B.R.~Dawson$^{12}$,
J.A.~Day$^{12}$,
R.M.~de Almeida$^{26}$,
J.~de Jes\'us$^{8,37}$,
S.J.~de Jong$^{75,77}$,
G.~De Mauro$^{75,77}$,
J.R.T.~de Mello Neto$^{24,25}$,
I.~De Mitri$^{42,43}$,
J.~de Oliveira$^{26}$,
D.~de Oliveira Franco$^{20}$,
V.~de Souza$^{18}$,
J.~Debatin$^{36}$,
M.~del R\'\i{}o$^{10}$,
O.~Deligny$^{32}$,
N.~Dhital$^{64}$,
A.~Di Matteo$^{49}$,
M.L.~D\'\i{}az Castro$^{20}$,
C.~Dobrigkeit$^{20}$,
J.C.~D'Olivo$^{63}$,
Q.~Dorosti$^{41}$,
R.C.~dos Anjos$^{23}$,
M.T.~Dova$^{4}$,
J.~Ebr$^{30}$,
R.~Engel$^{36,37}$,
I.~Epicoco$^{52,45}$,
M.~Erdmann$^{39}$,
C.O.~Escobar$^{c}$,
A.~Etchegoyen$^{8,11}$,
H.~Falcke$^{75,78,77}$,
J.~Farmer$^{87}$,
G.~Farrar$^{85}$,
A.C.~Fauth$^{20}$,
N.~Fazzini$^{c}$,
F.~Feldbusch$^{38}$,
F.~Fenu$^{58,49}$,
B.~Fick$^{84}$,
J.M.~Figueira$^{8}$,
A.~Filip\v{c}i\v{c}$^{72,71}$,
T.~Fodran$^{75}$,
M.M.~Freire$^{6}$,
T.~Fujii$^{87,f}$,
A.~Fuster$^{8,11}$,
C.~Galea$^{75}$,
C.~Galelli$^{55,46}$,
B.~Garc\'\i{}a$^{7}$,
A.L.~Garcia Vegas$^{39}$,
H.~Gemmeke$^{38}$,
F.~Gesualdi$^{8,37}$,
A.~Gherghel-Lascu$^{68}$,
P.L.~Ghia$^{32}$,
U.~Giaccari$^{75}$,
M.~Giammarchi$^{46}$,
M.~Giller$^{65}$,
J.~Glombitza$^{39}$,
F.~Gobbi$^{9}$,
G.~Golup$^{1}$,
M.~G\'omez Berisso$^{1}$,
P.F.~G\'omez Vitale$^{9,10}$,
J.P.~Gongora$^{9}$,
N.~Gonz\'alez$^{8}$,
I.~Goos$^{1,37}$,
D.~G\'ora$^{64}$,
A.~Gorgi$^{50,49}$,
M.~Gottowik$^{35}$,
T.D.~Grubb$^{12}$,
F.~Guarino$^{56,47}$,
G.P.~Guedes$^{21}$,
E.~Guido$^{49,58}$,
S.~Hahn$^{37,8}$,
R.~Halliday$^{80}$,
M.R.~Hampel$^{8}$,
P.~Hansen$^{4}$,
D.~Harari$^{1}$,
V.M.~Harvey$^{12}$,
A.~Haungs$^{37}$,
T.~Hebbeker$^{39}$,
D.~Heck$^{37}$,
G.C.~Hill$^{12}$,
C.~Hojvat$^{c}$,
J.R.~H\"orandel$^{75,77}$,
P.~Horvath$^{31}$,
M.~Hrabovsk\'y$^{31}$,
T.~Huege$^{37,14}$,
J.~Hulsman$^{8,37}$,
A.~Insolia$^{54,44}$,
P.G.~Isar$^{69}$,
J.A.~Johnsen$^{81}$,
J.~Jurysek$^{30}$,
A.~K\"a\"ap\"a$^{35}$,
K.H.~Kampert$^{35}$,
B.~Keilhauer$^{37}$,
J.~Kemp$^{39}$,
H.O.~Klages$^{37}$,
M.~Kleifges$^{38}$,
J.~Kleinfeller$^{9}$,
M.~K\"opke$^{36}$,
G.~Kukec Mezek$^{71}$,
B.L.~Lago$^{16}$,
D.~LaHurd$^{80}$,
R.G.~Lang$^{18}$,
M.A.~Leigui de Oliveira$^{22}$,
V.~Lenok$^{37}$,
A.~Letessier-Selvon$^{33}$,
I.~Lhenry-Yvon$^{32}$,
D.~Lo Presti$^{54,44}$,
L.~Lopes$^{67}$,
R.~L\'opez$^{59}$,
R.~Lorek$^{80}$,
Q.~Luce$^{36}$,
A.~Lucero$^{8}$,
A.~Machado Payeras$^{20}$,
M.~Malacari$^{87}$,
G.~Mancarella$^{52,45}$,
D.~Mandat$^{30}$,
B.C.~Manning$^{12}$,
J.~Manshanden$^{40}$,
P.~Mantsch$^{c}$,
S.~Marafico$^{32}$,
A.G.~Mariazzi$^{4}$,
I.C.~Mari\c{s}$^{13}$,
G.~Marsella$^{52,45}$,
D.~Martello$^{52,45}$,
H.~Martinez$^{18}$,
O.~Mart\'\i{}nez Bravo$^{59}$,
M.~Mastrodicasa$^{53,43}$,
H.J.~Mathes$^{37}$,
J.~Matthews$^{83}$,
G.~Matthiae$^{57,48}$,
E.~Mayotte$^{35}$,
P.O.~Mazur$^{c}$,
G.~Medina-Tanco$^{63}$,
D.~Melo$^{8}$,
A.~Menshikov$^{38}$,
K.-D.~Merenda$^{81}$,
S.~Michal$^{31}$,
M.I.~Micheletti$^{6}$,
L.~Miramonti$^{55,46}$,
D.~Mockler$^{13}$,
S.~Mollerach$^{1}$,
F.~Montanet$^{34}$,
C.~Morello$^{50,49}$,
M.~Mostaf\'a$^{86}$,
A.L.~M\"uller$^{8,37}$,
M.A.~Muller$^{20,d,24}$,
K.~Mulrey$^{14}$,
R.~Mussa$^{49}$,
M.~Muzio$^{85}$,
W.M.~Namasaka$^{35}$,
L.~Nellen$^{63}$,
M.~Niculescu-Oglinzanu$^{68}$,
M.~Niechciol$^{41}$,
D.~Nitz$^{84,g}$,
D.~Nosek$^{29}$,
V.~Novotny$^{29}$,
L.~No\v{z}ka$^{31}$,
A Nucita$^{52,45}$,
L.A.~N\'u\~nez$^{28}$,
M.~Palatka$^{30}$,
J.~Pallotta$^{2}$,
M.P.~Panetta$^{52,45}$,
P.~Papenbreer$^{35}$,
G.~Parente$^{74}$,
A.~Parra$^{59}$,
M.~Pech$^{30}$,
F.~Pedreira$^{74}$,
J.~P\c{e}kala$^{64}$,
R.~Pelayo$^{61}$,
J.~Pe\~na-Rodriguez$^{28}$,
J.~Perez Armand$^{19}$,
M.~Perlin$^{8,37}$,
L.~Perrone$^{52,45}$,
C.~Peters$^{39}$,
S.~Petrera$^{42,43}$,
T.~Pierog$^{37}$,
M.~Pimenta$^{67}$,
V.~Pirronello$^{54,44}$,
M.~Platino$^{8}$,
B.~Pont$^{75}$,
M.~Pothast$^{77,75}$,
P.~Privitera$^{87}$,
M.~Prouza$^{30}$,
A.~Puyleart$^{84}$,
S.~Querchfeld$^{35}$,
J.~Rautenberg$^{35}$,
D.~Ravignani$^{8}$,
M.~Reininghaus$^{37,8}$,
J.~Ridky$^{30}$,
F.~Riehn$^{67}$,
M.~Risse$^{41}$,
P.~Ristori$^{2}$,
V.~Rizi$^{53,43}$,
W.~Rodrigues de Carvalho$^{19}$,
J.~Rodriguez Rojo$^{9}$,
M.J.~Roncoroni$^{8}$,
M.~Roth$^{37}$,
E.~Roulet$^{1}$,
A.C.~Rovero$^{5}$,
P.~Ruehl$^{41}$,
S.J.~Saffi$^{12}$,
A.~Saftoiu$^{68}$,
F.~Salamida$^{53,43}$,
H.~Salazar$^{59}$,
G.~Salina$^{48}$,
J.D.~Sanabria Gomez$^{28}$,
F.~S\'anchez$^{8}$,
E.M.~Santos$^{19}$,
E.~Santos$^{30}$,
F.~Sarazin$^{81}$,
R.~Sarmento$^{67}$,
C.~Sarmiento-Cano$^{8}$,
R.~Sato$^{9}$,
P.~Savina$^{52,45,32}$,
C.~Sch\"afer$^{37}$,
V.~Scherini$^{45}$,
H.~Schieler$^{37}$,
M.~Schimassek$^{36,8}$,
M.~Schimp$^{35}$,
F.~Schl\"uter$^{37,8}$,
D.~Schmidt$^{36}$,
O.~Scholten$^{76,14}$,
P.~Schov\'anek$^{30}$,
F.G.~Schr\"oder$^{88,37}$,
S.~Schr\"oder$^{35}$,
S.J.~Sciutto$^{4}$,
M.~Scornavacche$^{8,37}$,
R.C.~Shellard$^{15}$,
G.~Sigl$^{40}$,
G.~Silli$^{8,37}$,
O.~Sima$^{68,h}$,
R.~\v{S}m\'\i{}da$^{87}$,
P.~Sommers$^{86}$,
J.F.~Soriano$^{82}$,
J.~Souchard$^{34}$,
R.~Squartini$^{9}$,
M.~Stadelmaier$^{37,8}$,
D.~Stanca$^{68}$,
S.~Stani\v{c}$^{71}$,
J.~Stasielak$^{64}$,
P.~Stassi$^{34}$,
A.~Streich$^{36,8}$,
M.~Su\'arez-Dur\'an$^{28}$,
T.~Sudholz$^{12}$,
T.~Suomij\"arvi$^{32}$,
A.D.~Supanitsky$^{8}$,
J.~\v{S}up\'\i{}k$^{31}$,
Z.~Szadkowski$^{66}$,
A.~Taboada$^{36}$,
A.~Tapia$^{27}$,
C.~Timmermans$^{77,75}$,
P.~Tobiska$^{30}$,
C.J.~Todero Peixoto$^{17}$,
B.~Tom\'e$^{67}$,
G.~Torralba Elipe$^{74}$,
A.~Travaini$^{9}$,
P.~Travnicek$^{30}$,
C.~Trimarelli$^{53,43}$,
M.~Trini$^{71}$,
M.~Tueros$^{4}$,
R.~Ulrich$^{37}$,
M.~Unger$^{37}$,
M.~Urban$^{39}$,
L.~Vaclavek$^{31}$,
M.~Vacula$^{31}$,
J.F.~Vald\'es Galicia$^{63}$,
I.~Vali\~no$^{42,43}$,
L.~Valore$^{56,47}$,
A.~van Vliet$^{75}$,
E.~Varela$^{59}$,
B.~Vargas C\'ardenas$^{63}$,
A.~V\'asquez-Ram\'\i{}rez$^{28}$,
D.~Veberi\v{c}$^{37}$,
C.~Ventura$^{25}$,
I.D.~Vergara Quispe$^{4}$,
V.~Verzi$^{48}$,
J.~Vicha$^{30}$,
L.~Villase\~nor$^{59}$,
J.~Vink$^{79}$,
S.~Vorobiov$^{71}$,
H.~Wahlberg$^{4}$,
A.A.~Watson$^{a}$,
M.~Weber$^{38}$,
A.~Weindl$^{37}$,
L.~Wiencke$^{81}$,
H.~Wilczy\'nski$^{64}$,
T.~Winchen$^{14}$,
M.~Wirtz$^{39}$,
D.~Wittkowski$^{35}$,
B.~Wundheiler$^{8}$,
A.~Yushkov$^{30}$,
O.~Zapparrata$^{13}$,
E.~Zas$^{74}$,
D.~Zavrtanik$^{71,72}$,
M.~Zavrtanik$^{72,71}$,
L.~Zehrer$^{71}$,
A.~Zepeda$^{60}$,
M.~Ziolkowski$^{41}$,
F.~Zuccarello$^{54,44}$


==> 2020-04-author_list-ZIP/templates/plain_latex/latex_authorlist_institutions.tex <==
% created on 2020-04-02

% needs \usepackage{enumitem}
\begin{description}[labelsep=0.2em,align=right,labelwidth=0.7em,labelindent=0em,leftmargin=2em,noitemsep]
\item[$^{1}$] Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina
\item[$^{2}$] Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina
\item[$^{3}$] Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina
\item[$^{4}$] IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina
\item[$^{5}$] Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina
\item[$^{6}$] Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina
\item[$^{7}$] Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina
\item[$^{8}$] Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina
\item[$^{9}$] Observatorio Pierre Auger, Malarg\"ue, Argentina
\item[$^{10}$] Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina
\item[$^{11}$] Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina
\item[$^{12}$] University of Adelaide, Adelaide, S.A., Australia
\item[$^{13}$] Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium
\item[$^{14}$] Vrije Universiteit Brussels, Brussels, Belgium
\item[$^{15}$] Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil
\item[$^{16}$] Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil
\item[$^{17}$] Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil
\item[$^{18}$] Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil
\item[$^{19}$] Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil
\item[$^{20}$] Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil
\item[$^{21}$] Universidade Estadual de Feira de Santana, Feira de Santana, Brazil
\item[$^{22}$] Universidade Federal do ABC, Santo Andr\'e, SP, Brazil
\item[$^{23}$] Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil
\item[$^{24}$] Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil
\item[$^{25}$] Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil
\item[$^{26}$] Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil
\item[$^{27}$] Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia
\item[$^{28}$] Universidad Industrial de Santander, Bucaramanga, Colombia
\item[$^{29}$] Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic
\item[$^{30}$] Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic
\item[$^{31}$] Palacky University, RCPTM, Olomouc, Czech Republic
\item[$^{32}$] Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France
\item[$^{33}$] Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Universit\'es Paris 6 et Paris 7, CNRS-IN2P3, Paris, France
\item[$^{34}$] Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France
\item[$^{35}$] Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany
\item[$^{36}$] Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany
\item[$^{37}$] Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany
\item[$^{38}$] Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany
\item[$^{39}$] RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany
\item[$^{40}$] Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany
\item[$^{41}$] Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany
\item[$^{42}$] Gran Sasso Science Institute, L'Aquila, Italy
\item[$^{43}$] INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy
\item[$^{44}$] INFN, Sezione di Catania, Catania, Italy
\item[$^{45}$] INFN, Sezione di Lecce, Lecce, Italy
\item[$^{46}$] INFN, Sezione di Milano, Milano, Italy
\item[$^{47}$] INFN, Sezione di Napoli, Napoli, Italy
\item[$^{48}$] INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy
\item[$^{49}$] INFN, Sezione di Torino, Torino, Italy
\item[$^{50}$] Osservatorio Astrofisico di Torino (INAF), Torino, Italy
\item[$^{51}$] Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy
\item[$^{52}$] Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy
\item[$^{53}$] Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy
\item[$^{54}$] Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy
\item[$^{55}$] Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy
\item[$^{56}$] Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy
\item[$^{57}$] Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy
\item[$^{58}$] Universit\`a Torino, Dipartimento di Fisica, Torino, Italy
\item[$^{59}$] Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico
\item[$^{60}$] Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico, D.F., M\'exico
\item[$^{61}$] Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico
\item[$^{62}$] Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico
\item[$^{63}$] Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico
\item[$^{64}$] Institute of Nuclear Physics PAN, Krakow, Poland
\item[$^{65}$] University of \L{}\'od\'z, Faculty of Astrophysics, \L{}\'od\'z, Poland
\item[$^{66}$] University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland
\item[$^{67}$] Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal
\item[$^{68}$] ``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania
\item[$^{69}$] Institute of Space Science, Bucharest-Magurele, Romania
\item[$^{70}$] University Politehnica of Bucharest, Bucharest, Romania
\item[$^{71}$] Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia
\item[$^{72}$] Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia
\item[$^{73}$] Universidad de Granada and C.A.F.P.E., Granada, Spain
\item[$^{74}$] Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain
\item[$^{75}$] IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands
\item[$^{76}$] KVI -- Center for Advanced Radiation Technology, University of Groningen, Groningen, The Netherlands
\item[$^{77}$] Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands
\item[$^{78}$] Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands
\item[$^{79}$] Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands
\item[$^{80}$] Case Western Reserve University, Cleveland, OH, USA
\item[$^{81}$] Colorado School of Mines, Golden, CO, USA
\item[$^{82}$] Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA
\item[$^{83}$] Louisiana State University, Baton Rouge, LA, USA
\item[$^{84}$] Michigan Technological University, Houghton, MI, USA
\item[$^{85}$] New York University, New York, NY, USA
\item[$^{86}$] Pennsylvania State University, University Park, PA, USA
\item[$^{87}$] University of Chicago, Enrico Fermi Institute, Chicago, IL, USA
\item[$^{88}$] University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA
\item[] -----
\item[$^{a}$] School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom
\item[$^{b}$] Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany
\item[$^{c}$] Fermi National Accelerator Laboratory, USA
\item[$^{d}$] also at Universidade Federal de Alfenas, Po\c{c}os de Caldas, Brazil
\item[$^{e}$] Colorado State University, Fort Collins, CO, USA
\item[$^{f}$] now at Hakubi Center for Advanced Research and Graduate School of Science, Kyoto University, Kyoto, Japan
\item[$^{g}$] also at Karlsruhe Institute of Technology, Karlsruhe, Germany
\item[$^{h}$] also at Radboud Universtiy Nijmegen, Nijmegen, The Netherlands
\end{description}

